HySIM: A Hybrid Spectrum and Information Market for TV White Space Networks

We propose a hybrid spectrum and information market for a database-assisted TV white space network, where the geo-location database serves as both a spectrum market platform and an information market platform. We study the inter- actions among the database operator, the spectrum licensee, and unlicensed users systematically, using a three-layer hierarchical model. In Layer I, the database and the licensee negotiate the commission fee that the licensee pays for using the spectrum market platform. In Layer II, the database and the licensee compete for selling information or channels to unlicensed users. In Layer III, unlicensed users determine whether they should buy the exclusive usage right of licensed channels from the licensee, or the information regarding unlicensed channels from the database. Analyzing such a three-layer model is challenging due to the co-existence of both positive and negative network externalities in the information market. We characterize how the network externalities affect the equilibrium behaviours of all parties involved. Our numerical results show that the proposed hybrid market can improve the network profit up to 87%, compared with a pure information market. Meanwhile, the achieved network profit is very close to the coordinated benchmark solution (the gap is less than 4% in our simulation).

==> Latex_ParticipateSensing_infocom_camera/Section0-Intro.tex <==
%!TEX root = main_hybrid_market.tex
%SourceDoc main_hybrid_market.tex


%\vspace{-2mm}
\section{Introduction}\label{sec:intro}


%http://venturebeat.com/2013/06/14/obama-orders-government-agencies-to-free-up-wireless-spectrum-for-the-people/
%http://en.wikipedia.org/wiki/Information_market

%\com{We need to avoid the introduction so that it does not closely resemble any of our existing papers in this area.
%In the time of "double-blind submission", people are likely to be more sensitive about the issue of "self-plagiarism", due to its possibility of revealing the authors' identities. }

\subsection{Background}

With the explosive growth of mobile smartphones and bandwidth-hunger wireless applications, radio spectrum has become increasingly scarce \cite{sen2013sdp}.
%Many countries have started to seek new spectrum opportunities for wireless broadband services.
The UHF/VHF frequency band originally assigned for broadcast television services (hereafter called TV channels) has been viewed as a promising spectrum opportunity for supporting new wireless broadband services.
First, in many places there are many unused TV channels (i.e., those unlicensed to any TV licensees),
%\footnote{For example, in the USA, we can obtain from the Google White Space Database \cite{Google} that among a total of $50$ TV channels (each with a bandwidth of $6$MHz), there are $12$ unused channels ($72$MHz) in Harvard University,
%% (Location: $42.377003, -71.116660$),
%$13$ unused  channels ($78$MHz) available in Yale University,
%% (Location: $41.316324, -72.922343$),
%$3$ unused channels ($18$MHz) available in Princeton University, etc.
%% (Location: $40.343989, -74.651448$), etc.
%}
often called \emph{TV white spaces} \cite{Microsoft2010report, Ofcom2012tvws, federal2012third}, which can be used for supporting unlicensed non-TV wireless services.
Second, even the licensed TV channels (i.e., allocated to certain TV licensees) may have a low utilization in most time \cite{cognitive}, and hence can be opportunistically reused by unlicensed non-TV wireless services with the permissions of licensees.
 
%\emph{TV White Space (TVWS)} has been recently recognized as one of the promising spectrum opportunities for wireless broadband services due to its low utilization and brilliant propagation performance \cite{Microsoft2010report, Ofcom2012tvws, Ofcom2010geo}.
%Specifically, TV white space refers to the unused broadcast television spectrum channels (also called TV channels) at a particular time and location.
%%TV white space can be utilized as super WiFi to provide a high transmission rate and a large single-cell coverage.
%By allowing unlicensed wireless devices (called white space devices, WSDs) use the TV white space in an opportunistic manner, we can effectively improve the spectrum efficiency and alleviate the global spectrum scarcity today.
%As a consequence, in the USA, the Federal Communications Commission (FCC) has unanimously approved the license-exempt use of TV white space to support new wireless applications \cite{federal2010second}.


%In the USA, the FCC has unanimously approved the {license-exempt} use of TV white space  (i.e., the unused/unlicensed TV channels)  for unlicensed wireless devices \cite{federal2010second}.
To effectively exploit the TV white spaces while not harming the interests of licensed devices (TVs),
%some spectrum regulators (such as the FCC in the USA and Ofcom in the UK), together with standards bodies and industrial organizations,
the industry has started to adopt a \emph{database-assisted} TV white space network architecture  \cite{Ofcom2010geo, Google, Microsoft, SpectrumBridge, SpectrumBridgeCommericial}.
In this architecture, unlicensed  devices obtain the list of available unlicensed TV channels via querying a certified white space \emph{geo-location} database, which periodically updates information based on a repository of licensees.
%To achieve this, the geo-location database needs to house and periodically updated the network infrastructures of TV licensees as well as their spectrum license information.
Meanwhile, the FCC also allows the spectrum licensees to temporarily   lease their licensed channels to unlicensed devices through, for example,  auction \cite{federal2004leasing}.
Such spectrum trading (leasing) requires a market platform, and the geo-location database can serve as such a platform (e.g., \emph{SpecEx} \cite{SpectrumBridgeCommericial2}) due to its proximity to both spectrum licensees and unlicensed devices.
This means that the geo-location database can facilitate the unlicensed spectrum access to both unlicensed and licensed TV channels.

%Note that the geo-location databases are usually operated by third-party companies, such as Google \cite{Google}, SpectrumBridge \cite{SpectrumBridge}, and Microsoft \cite{Microsoft}.
%%\footnote{These geo-location databases are certified by the FCC, and operate in the USA.
%%Based on these databases, several TV white space trial networks \cite{Microsoft2010report, SpectrumBridgeCommericial} have been developed in the USA.}
%Hence, the commercial deployment of such a database-assisted network or platform requires a proper business model that offers sufficient incentives to the database operators to cover their capital expense (CapEx) and operating expense (OpEx).
%%\rev{Based on these two kinds of TV \chs, recent works which are devoted to the business modeling of {\tvn} can be categorized into two classes.}
Recently, researchers have proposed several business and marketing models related to the database-assisted spectrum sharing, which can be categorized into two classes: \emph{Spectrum Market} and \emph{Information Market}.
The first class ({spectrum market}   \cite{luo2012,feng2013database,luo2013}) mainly deals with the trading of
%which has been extensively used in traditional dynamic spectrum sharing literature.
%Spectrum market is mainly designed for the licensed TV channels.
licensed TV channels.
The key idea is to let spectrum licensees temporarily lease their {under-utilized} licensed TV channels to unlicensed users for some additional revenue.
%\rev{The secondary spectrum market is mainly designed for the trading of those (non-free) TV channels registered to certain licensee already but under-utilized by the licensee, while not suitable for the unregistered TV channels due to the policy restraints \cite{federal2012third}.}
The database serves as a market platform facilitating this trading process.\footnote{For example, it acts as a spectrum broker or agent, purchases spectrum from licensees and then resells the purchased spectrum to unlicensed users.}
A commercial example of such a \emph{database-provided} spectrum market platform is \emph{SpecEx} \cite{SpectrumBridgeCommericial2}, operated by SpectrumBridge.\footnote{\rev{Note that there are also many existing work discussing the secondary spectrum markets using the auction mechanism such as \cite{zhou2008,zhou2009}. The auction mechanism is usually adopted when the seller has litre knowledge of buyers. Because in the TV white space market, {\eus} are required to report some information such as their location information, device type to the database in order to let the database calculate the available unlicensed channels to access to. Hence, we focus on pricing strategy in our paper.} }

%\com{Make it more specific regarding what
%kind of incentives we need to consider. }
%Today we are witnessing the spectrum scarcity and spectrum inefficient utilization.
%TV white space network is a novel and promising paradigm of dynamic spectrum sharing, and can effectively improve the spectrum efficiency and alleviate the spectrum scarcity \cite{federal2010second, Ofcom2012tvws}.
%In a TV white space network, unlicensed wireless devices (called white space devices, WSDs) explore and exploit the unused or under-utilized broadcast television spectrum (called TV white space, TVWS\footnotesc{For convenience, we will refer to TV white space as ``TV channel''.}) opportunistically, via a certified \emph{geo-location} white space database \cite{Ofcom2010geo}.
%%The successful deployment of a {\tvn} requires many technical innovations, among which an important one is to reliably detect the available {\tv} and accurately estimate the   channel quality  at different times and locations.~~~~~~~~
%The white space database is usually operated by a third-party company, and houses an up-to-date repository of TV licensees (e.g., the locations of TV stations and their channel occupancies).
%The WSD users, before accessing TV white spaces (i.e., TV channels), must query a white space database for the available (idle) channels at their current locations.
%%Figure \ref{fig:model} illustrates such a database-assistant TV white space network with 3 licensed TV stations and 8 unlicensed \eus, where \eus $1$ and $2$ query the available channel information from database 1, \eus $3$ and $4$ query the available channel information from database 2, and \eus $5$ to $8$ remain inactive.
%Such a database-assistant {\tvn} architecture
%has been widely supported by spectrum regulators, standards bodies, and industrial organizations \cite{IEEE80222, WSAlliance, Google, Microsoft, SpectrumBridge, Microsoft2010report, SpectrumBridgeCommericial}.\footnotesc{
%%\footnotesc{Supporters include the standards bodies (e.g., IEEE 802.22~Group~\cite{IEEE80222}), industrial organizations  (e.g., Whitespace Alliance \cite{WSAlliance}), and major IT companies (e.g., Google \cite{Google} and Microsoft \cite{Microsoft}).}
%%\footnotesc{For example, it has been approved by spectrum regulatory bodies (e.g., FCC in the USA [1] and Ofcom in the UK [2]), standards bodies (e.g., IEEE 802.22 Group [3]), industrial organizations (e.g., Whitespace Alliance [4]), and  major IT companies (e.g., Google and Microsoft).}
%%In 2010, FCC released a technical ruling \cite{federal2010second} for the use of TV {\tv s} for unlicensed \eus, which removes the mandatory sensing requirements on \eus. Instead, the ruling requires \eus to have the ability to learn the available TV {\tv} information at their respective locations via inquiring the geo-location database.
%In January 2011, FCC has conditionally designated 9 companies, including Google \cite{Google}, Spectrum Bridge \cite{SpectrumBridge}, and LS Telecom,  to serve as {white space} database operators in USA, developing trial white space database systems.
%%As of today, some of these databases (including those of Google \cite{Google} and Spectrum Bridge \cite{SpectrumBridge}) have been certified by FCC  and are operational.
%% and are available for \eus to inquire the available {\tv} at any time and any location in the USA.
%Based on these certified databases, several TV white space trial networks \cite{Microsoft2010report} and commercial networks \cite{SpectrumBridgeCommericial} have been developed.}
%%\footnotesc{After completing the FCC's 45-day testing phase, some of these companies including Spectrum Bridge and Google have been certificated by FCC as the  white spaces database providers.}
%Clearly, the long-term commercial deployment of such a database-assistant network requires a proper business model that offers sufficient economic incentives to the database operators.~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%Such an issue has not been extensively discussed in the existing literature.
%
%%\begin{figure}
%%%\vspace{-6mm}
%%  \centering
%%    \includegraphics[width=3in]{model-new}
%%\vspace{-5mm}
%%  \caption{Illustration of a database-assistant TV white space network. To access a TV channel, each \eu first reports its location to a white space database (request), and then the database returns the available channel list to the \eu. }
%%\label{fig:model}
%%\vspace{-5mm}
%%\end{figure}

%\com{explain two types of TV channels actually from here? }
%\rev{In practice, there are two kinds of TV \chs~co-exist in a particular location. One is registered TV \chs~which are owned by certain licensee. If this registered TV \chs~are under utilized, the licensee may lease/sell these TV \chs~to WSD users for exclusive usage. The other is unregistered TV channels which are not owned by any licensee. The database can provide WSD users with those unregistered TV channels information so that WSD users can freely those TV channels in shared based. Moreover, according to the FCC's rule \cite{federal2010second,federal2012third}, a WSD user can even access to the registered TV \chs~as long as this user is outside the protection contour around licensee. }


The second class ({information market}) has been recently introduced by Luo \emph{et al.} for the unlicensed TV channels (i.e., TV white spaces)\cite{luo2014wiopt, luo2014SDP}.
%Notice that based on the regulation policy (e.g., \cite{federal2012third}), this type of spectrum is often treated as the public resource (like water and air) for the free and shared usage among unlicensed devices, and is not allowed for trading.
%To this end, Luo \emph{et al.} proposed an information market, which lets the geo-location database sell the advanced information regarding the quality of unlicensed TV channels (instead of channels) to the unlicensed users for profit.
In their models, the geo-location database sells the advanced information regarding the quality of unlicensed TV channels, instead of channels, to the unlicensed users for profit.
The key motivation is that the database knows more information regarding TV white spaces than unlicensed users,\footnote{For example, based on the knowledge about the network infrastructures of TV licensees and their licensed channels, the database can predict the average interference (from licensed devices) on each TV channel at each location.} and hence it can provide information that helps unlicensed users improve their performances.
A commercial example of information market is \emph{White Space Plus} \cite{SpectrumBridgeCommericial}, again operated by SpectrumBridge.~~~~~~~~~~~~~~~~~~~~~~~~~~~~

%\rev{The information market is mainly designed for the trading of information regarding those (free) TV channels unregistered to any licensee (as these channels are freely shared among many users, hence their quality information may frequently change), while not efficient for the registered TV channels (as these channels are usually used by unlicensed users exclusively (under the grant of licensees), hence have fixed and guaranteed quality).}

% In practice, both spectrum market and information market have attracted growing interest among the real geo-location operators. Some database operators have tried to adopt one or both of these business models practically.
%Real-world examples of such  \emph{database-provided} spectrum market and information market are \emph{SpecEx} \cite{SpectrumBridgeCommericial2} and
%\emph{White Space Plus} \cite{SpectrumBridgeCommericial}, respectively, both provided by SpectrumBridge, the world first certified  database operator in the USA.
%Specifically, SpecEx is an online spectrum marketplace for the trading of (registered) TV channels between TV licensees and unlicensed users.
%It facilitates both the licensees to display their under-utilized spectrum information, and the unlicensed users to lease these licensed spectrum from the licensee.
%%In this process, the database may create revenue via acting as a spectrum agent or broker.
%White Space Plus is an online information market for the trading of information (mainly regarding the unregistered TV channels) between the database itself and unlicensed users.
%It offers advanced information regarding the quality of (unregistered) TV channels (e.g., the interference level) to unlicensed users.~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

% \subsection{Motivations}


% It is important to note that the secondary spectrum market is mainly designed for the trading of those (non-free) TV channels registered to certain licensee already but under-utilized by the licensee, while not suitable for the unregistered TV channels due to the policy restraints \cite{xa}.
% The information market is mainly designed for the trading of information regarding those (free) TV channels unregistered to any licensee (as these channels are freely shared among many users, hence their quality information may frequently change), while not efficient for the registered TV channels (as these channels are usually used by unlicensed users exclusively (under the grant of licensees), hence have fixed and guaranteed quality).~~~~~~~~~~~~~

In practice, \emph{both the licensed TV channels and unlicensed TV white spaces co-exist at a particular location}.
Some users may prefer to lease the licensed TV channels from licensees for the exclusive usage,
while other users may prefer to share the free unlicensed TV white spaces with others.
Hence, a joint formulation and optimization of both spectrum market and information market is highly desirable.
However, none of the existing work \cite{luo2012,feng2013database,luo2013,luo2014wiopt, luo2014SDP} looked at the interaction between spectrum market and information market.
This motivates our study of a \emph{hybrid} spectrum and information market for the database in TV white space networks.
%Clearly, the successful deployment of such a database-provided hybrid market requires a deep understanding of the market response and dynamics,
%which has not been completely studied in the existing literature.~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

%Note that these channels may be shared by many unlicensed users, hence users may suffer a high co-interference when using these channels.
%In this sense, the database can potentially make profit by selling his known information regarding these channels to unlicensed users.

%However, the TV spectrum market model may \emph{not} be suitable in practice due to some regulatory considerations.
%For example, TV white spaces (especially those not licensed to any licensee) are usually treated as the \emph{public} resources, and designated by regulators for the \emph{public and shared} usage by unlicensed devices.
%Therefore, TV white spaces may not be freely traded in a spectrum market like other licensed spectrum bands.
%Luo \emph{et. al} study the information market for the monopoly \db \cite{luo2014wiopt} and duopoly \dbs \cite{luo2014SDP}. In their models, the \db~makes the profit by selling the information of \tvn~instead of selling the spectrum. However, they only characterize the positive network effect in the information market without consider the congestion effect of the network. Note that all {\eus} have to share the TV \chs~together. The higher co-interference in TV \chs~may lead to the \db's advanced information not so valuable. To this end, a new business model without involving the trading of spectrum and taking both of the congestion and positive network effect is highly desirable.

%\com{Would be good to add a figure in page 1, illustrating the hybrid information market, and help readers understand both  the spectrum bridge model and our proposed model.}

%The world first white space database operator certified by FCC --
%Spectrum Bridge --
%proposed an alternative business model called ``White Space Plus" \cite{SpectrumBridgeCommericial}.
%The basic idea is to sell some advanced information (regarding the quality of TV channels) to \eus, such that the latter can choose and operate on the high quality {\tvs}.
%An example of such information is the degree of interference on every available \tv.
%This essentially leads to an \emph{information market}, where {\eus} purchase the information regarding the {\tv} quality from the database, instead of purchasing the channel itself.
%Besides selling the advance information of TV \chs, Spectrum Bridge also provides online marketplace called "SpecEx" \cite{SpectrumBridgeCommericial2} for licensed spectrum and unlicensed devices. The online marketplace displays the licensee information and help the unlicensed devices lease licensed spectrum from the \lh. Hence, the database creates value via information collection, aggregation, display, and information processing. These information includes unlicensed spectrum (e.g. TV white space) and licensed spectrum. Note that these two kinds of spectrum are substitutable and have different wireless transmission quality.
%Clearly, the successful deployment of such a hybrid information market requires a deep understanding
%of the market response and dynamics,
%which has not been considered in the existing literature.
%This motivates our study in this paper.



\begin{figure}
\centering
  \includegraphics[width=3.1in]{model}
  \caption{Illustration of Database-Provided Hybrid Spectrum and Informaiton Market (HySIM). Users 1 and 2 lease the licensed TV channels, and Users 3 and 4 share the free unlicensed TV white spaces with others. User 4 further purchases the advanced information to improve its performance.}\label{fig:model}
%  \com{should we also divide this into several channels? }
  \vspace{-6mm}
\end{figure}



\subsection{Contributions}

In this paper, we model and study a \underline{Hy}brid \underline{S}pectrum and \underline{I}nformation \underline{M}arket (HySIM) in a database-assisted TV white space network,
in which the geo-location database serves as (i) a \emph{spectrum market} platform for the trading of (under-utilized) licensed TV channels between spectrum licensees and unlicensed users,
and (ii) an \emph{information market} platform for the trading of information (regarding the unlicensed TV white spaces) between the database itself and unlicensed users.
Unlicensed users can choose to lease the licensed TV channels from licensees (via the database) for the exclusive usage,
or to share the free TV white spaces with others.
In the latter case, users can further decide whether to purchase the advanced information regarding these TV white spaces from the database to enhance the performance.
Figure \ref{fig:model} illustrates such a database-provided HySIM framework.
%In this example, users 1 and 2 choose to lease the registered channels from the TV licensee, while users 3 and 4 choose to use the shared unregistered channels. Moreover, user 4 chooses to purchase the advanced information from the database.

%Our focus in this work is to make a thorough and comprehensive understanding of the  behaviors and equilibrium in such a database-provided hybrid spectrum and information market, so as to offer meaningful insights to a real TV white space network system.
%To this end, we formulate the interactions among the geo-location database (operator), the spectrum licensee, and unlicensed users as a three-layer hierarchical model shown as follows.
%% illustrated in Figure \ref{fig:problem}. Specifically,

In order to thoroughly understand the user behaving, the market evolving, and the equilibrium in such a hybrid market, we formulate the interactions among the geo-location database (operator), the spectrum licensee, and unlicensed users as a three-layer hierarchical model:
% illustrated in Figure \ref{fig:problem}. Specifically,

\subsubsection{Layer I: Commission Negotiation (Section \ref{sec:layer1})}
In the first layer, the database and the   licensee negotiate regarding the commission for the licensee to use the spectrum market platform. 
Specifically, the database, as the spectrum market platform, helps the spectrum licensee to display, advertise, and sell the under-utilized TV channels to unlicensed users.
Accordingly, it takes some \emph{commission charge} from each successful transaction between the spectrum licensee and unlicensed users.
%We consider two different commission charging schemes: (i) \emph{revenue sharing} scheme  (RSS) and (ii) \emph{wholesale pricing} scheme (WPS).
%We study the commission charge under both schemes systematically, by using the Nash bargaining theory \cite{harsanyi1977bargaining}.
%In this work,
\rev{
The commission charging scheme we considered in this paper is \emph{revenue sharing} scheme  (RSS), where the licensee shares a fixed percentage of  revenue with the database.
We study such commission charge schemes using the  Nash bargaining theory \cite{harsanyi1977bargaining}.~~~~~~~
}
%We consider two different commission charging schemes: (i) \emph{revenue sharing} scheme  (RSS), where the licensee shares a fixed percentage of  revenue with the database, and (ii) \emph{wholesale pricing} scheme (WPS), where the database charges a fixed wholesale price from each successful transaction of the licensee.
%We study the commission charge under both schemes using the  Nash bargaining theory \cite{harsanyi1977bargaining}.~~~~~~~


\subsubsection{{Layer II: Price Competition Game} (Section \ref{sec:layer2})}
In the second layer, the database and the spectrum licensee compete with each other for selling information or channels to unlicensed users.
The spectrum licensee decides the price of the licensed TV channels,
and the database decides the price of the advanced information (regarding the unlicensed TV channels).
%This price competition game model is significantly different from traditional models \cite{Jia2008game,Niyato2009game,Duan2012game}, due to the commission charge on top of the game.\footnote{For example, a higher revenue sharing percentage under RSS will reduce the database's aggressivity in the pricing competition, since it can draw more revenue from the licensee's  transactions.}
We analyze the equilibrium of such a price competition game using the supermodular game theory \cite{topkis1998supermodular}.~~~~~~~~~
%study the game equilibrium systematically, by using the supermodular game theory \cite{topkis1998supermodular}.~~~~~~~~~~~~~~~~~~


\subsubsection{{Layer III: User Behaving and Market Dynamics (Section \ref{sec:user_subscript})}}
In the third layer, unlicensed users decide the best purchasing decisions, given the database's information price and the licensee's channel price.
%Each user has three different choices: (i) leasing the licensed TV channels for the exclusive usage, (ii) sharing the free unlicensed TV white space with others, (iii) sharing the free unlicensed TV white space with others and purchasing the advanced information to improve its performance.
Note that the users need to consider both the \emph{negative} and \emph{positive} network externality of the information market.
%On one hand, the information market has the \emph{negative} network externality, as more users purchasing the advanced information implies that more users share the TV white spaces, and hence increases the congestion level and degrades the user performance.
%On the other hand, the information market also has \emph{positive} network externality, as more users purchasing the advanced information increases the quality/value of the database's information and improves the user performance.
%Such a performance change further stimulates users to adjust their behaviors in the future, hence the users' behaviors dynamically involve.
We will show how the market dynamically evolves according to the users' best choices, and what the \emph{market equilibrium} point is.

%\begin{figure}
%\centering
%  \includegraphics[width=2.4in]{problem}
%  \caption{Three-layer Interaction Model.}\label{fig:problem}
%\end{figure}






%It is easy to see that in such a framework,
%the database operator serves as both the \emph{market platform} and the \emph{market component}.
%On one hand, as the market platform, the database operator helps the TV licensee to display its channel information (e.g., frequency band, idle time, price, etc),
%and helps the unlicensed WSD users to find out these information.
%Hence, it facilitates the spectrum trading between TV licensees and unlicensed users.
%Accordingly, the database operator takes certain \emph{commission charge} from each successful transaction between TV licensees and unlicensed users.
%\rev{In our work, we consider two different commission schemes-\emph{revenue sharing} scheme and \emph{wholesale pricing} scheme (WPS) and compare their performance.}
%\com{Yuan: As we will explain these two schemes detaildely in the next section, I think maybe we can delete the detail explanation here?}
%In our work, we consider two different commission schemes: (i) \emph{revenue sharing} scheme  (RSS), where the TV licensee shares a fixed portion of  revenue with the database operator, and (ii) \emph{wholesale pricing} scheme (WPS), where the database operator charges a fixed money from each successful transaction, regardless the detailed revenue that the TV licensee achieves from that transaction.~~~~~~~
%
%On the other hand, as the market component, the database operator competes directly with the TV licensee for unlicensed WSD users.
%Specifically, the TV licensee wants to sell its (under-utilized) registered channels to WSD users,
%while the database operator wants to sell its advanced information regarding the unregistered channels to WSD users.
%The TV licensee decides the price of the registered channels, and the database operator decides the price of its advanced information.
%In this sense, this is essentially a \emph{price competition} market.
%Note that the database operator is mandatorily required to provide the  unregistered TV channel list (which we call the basic information) to any legal WSD user \cite{federal2012third}, and the latter freely uses these channels in a   shared manner (hence there is co-interference).
%With the database's advanced information, the WSD users can potentially improve their performance when operating on the unregistered channels, e.g., choosing a channel with a low interference level.
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%Our focus in this work is to make a thorough and comprehensive understanding of the  behaviour and equilibrium in such a database-provided hybrid spectrum and information market, so as to offer meaningful insights to a real TV white space network system.
%To this end, we formulate  the interactions among the database operator, the TV licensee, and unlicensed WSD users as a three-layer hierarchical model.
%In the first layer, the database operator and the TV licensee negotiate the commission charge details regarding  the spectrum market platform.
%In the second layer, the database operator and the TV licensee make the pricing decisions.
%In the third layer, unlicensed WSD users make the purchasing decision.
%The key questions in such a three-layer model are following:~~~~~~~~~~~~~~~~~~
%\begin{itemize}
%\item
%\emph{Layer III:} How unlicensed WSD users determine  the best purchasing behaviour in the hybrid market, and what is the market equilibrium point, given the licensee's channel price and the database's information prices?
%\item
%\emph{Layer II:} How the licensee and the database make the best pricing decisions, and what is the equilibrium of this pricing competition game?
%\item
%\emph{Layer I:} How much commission charge should the database operator take from the TV licensee in order to operate the spectrum market platform?
%\end{itemize}

%These questions are challenging due to the following reason.
%On one hand, the information market has the property of {\emph{positive network externality}},
%i.e., the more users purchasing advanced information from the database, the higher value of the database's information for each buyer.
%On the other hand, more users purchasing information also increases the congestion among them (as they use the unregistered channels in a shared manner).
%This implies that the information market also has the property of \emph{negative network externality}.
% This makes our information market model significantly different from and more challenging than those in \cite{luo2014wiopt, luo2014SDP} which only considers the positive network effect.
%Hence, there is a tradeoff between the positive network externality and negative network externality.

%There are several challenges in the analysis of such a hybrid market.
%First, different from most of the traditional market models which are either negative effect only (e.g., spectrum market) or positive effect only (e.g., the information market in \cite{luo2014wiopt, luo2014SDP}), our proposed information exhibits both the negative effect and the positive effect.
%That is,  more WSD users purchasing the information from the database, on one hand, benefits the users in the information market due to the increase of information quality, and on the other hand, hurts the users operating on the unregistered TV channels (including the users in the information market) due to the increase of congestion.
%This makes our market model significantly different from those in \cite{luo2014wiopt, luo2014SDP}, which has only the positive effect.
%Second, the price competition game in our model is also very different from those traditional price competition game, due to the heterogeneity between two markets.

%In this paper, we model and study an online information platform provided by a \db, where
%the \db~not only sells the information about \emph{the interference level on every TV \chs} to \eus, but also list the licensed spectrum leasing information. The \lh~has to pay some certain listing fee to the \db.
%The {\eus} (buyers) decide whether to operate on the TV \chs~or lease licensed spectrum and whether to purchase the TV \chs' information if they operate on the TV \chs.
%The sequence of events is as follows. During the \emph{bargaining stage}, the \db~and the \lh~negotiate with each other in terms of the displaying fee for listing licensed spectrum leasing information on the \db's information platform. Given the bargaining result, both the \db~and the \lh~make \emph{pricing decisions} without observing each other's actions. In particular, the \db~choose subscription fee for {\eus} operating on the TV \chs~with advanced information, while the \lh~sets the leasing fee. Depending on the price pair, the utility provided by different service, and {\eus}' evaluation, each \eu~makes service choice.
%
%We want to understand the behavior of such an online information platform, in particular,
%%(i) what is the \eu's optimal purchasing behavior, (ii) how the market share of the \db~and the \lh (i.e., the percentage of \eus~purchasing TV \chs' information from the database and the percentage of \eus~leasing licensed spectrum from the \lh) dynamically evolves over time, and (iii) what is the stable market shares of both databases (also called \emph{market equilibrium})? All of these problems are challenging due to the following reasons.~~~~~~~~~~~~~~
%i) what is the optimal bargaining solution between the \db~and the \lh, ii) What is the Nash equilibrium of the pricing decisions game, and iii) how the market share of the \db~and the \lh~(i.e., the percentage of \eus~purchasing TV \chs' information from the database and the percentage of \eus~leasing licensed spectrum from the \lh) dynamically evolves over time, and what is the stable market shares of both the \db~and the \lh~(also called \emph{market equilibrium}).
%All of these problems are challenging due to the following reasons.~~~~~~~~~~~~~~
%
%First, there is lack of a unified framework to evaluate the value of information to \eus.
%Notice that the interference on a channel may come from the nearby TV stations operating on that channel or the nearby {\eus} using that channel.
%The {\db} can (relatively) precisely predict the interference from TV stations, as it maintains a repository of TV licensees.
%However, it may not be able to predict the precise interference from {\eus}, either because some users may not want to inform the \db~their choices of channels,
%or simply because some {\eus} may interact with another database in the same area.
%Therefore, the overall interference information that the {\db} provides may \emph{not} be accurate. Besides, what the value of TV \chs~information to {\eus} when the {\eus} can obtain the information of licensed spectrum? Note that the quality of licensed spectrum may be higher than that of TV \chs. If the price of leasing licensed spectrum is chosen appropriately, {\eus} are more willing to pay for leasing instead of purchasing the information.
%%In particular, one database's known information may not be the same as the other's, and neither database has the global information.
%%To this end, we propose a general framework to evaluate the value of information for \eus.
%The framework considers not only the potential error of the information provided by databases, but also the impact of listing licensed spectrum leasing information.
%
%Second, the information market has the property of {\emph{positive network externality}},
%i.e., the more \eus~purchasing information from the same database, the higher value of that database's information for each future buyer. Moreover, as the TV \chs~are shared basis spectrum, the information market also affected by the congestion effect, i.e., the more users operating on the TV \chs, the less value of TV \chs~quality information for each buyer due to the potential co-interference among users.
%This positive and negative correlation between the information value and  market share complicates the market behavior analysis, as a slight change of one \eu's purchasing behavior may affect the information evaluation and purchasing decisions of other \eus. We will analytically show how the market share of each database dynamically evolves over time, and eventually converges to a market equilibrium by taking these two network effect into consideration.

%In this work, we will study these three layer interactions systematically.
%As far as we know, this is the first work that proposes and studies a hybrid spectrum and information market for database-assisted TV white space networks.

In summary, we list the main contributions as follows. 
%\com{Yuan: According to the professor's suggestion, I do not mention [15][16].}

\begin{itemize}

\item
\emph{Novelty and Practical Significance:}
To the best of our knowledge, this is the first paper that proposes and studies a hybrid spectrum and information market for promoting the unlicensed spectrum access to both licensed and unlicensed TV channels.
%secondary utilization of both licensed and unlicensed TV channels.

\item
\emph{Modeling and Solution Techniques:}
We formulate the interactions as a three-layer hierarchical model, and analyze the model systematically by backward induction, using the market equilibrium theory, supermodular game theory, and Nash bargaining theory.~~~~~~~~~~~~

\item
\emph{Performance Evaluations:}
{Our numerical results show that the proposed hybrid market can bring up to $87\%$ network profit gain, compared with a pure information market.
Moreover, the gap between our achieved network profit and the coordinated benchmark is less than $4\%$.
}

%\item
%\emph{Observations and Insights:}
%Comparing the two commission charging schemes, we show that it is more profitable for the whole network to use the revenue sharing scheme when the information market is negative externality dominant, and use the wholesale pricing scheme when the information market is positive externality dominant. 
%\com{Not clean and too long. How to answer the readers' "So What" question? Is it really important for the readers to remember all these results? Or it is more importantly to emphasize a subset of the conclusions?}
%We show when the information market is negative externality dominant, (i) the database can always achieve a higher profit under the RSS scheme, (ii) the licensee can achieve a higher profits under the RSS scheme when the licensed channel quality is low, and (iii) the total network profit is higher under the RSS scheme.
%When the information market is positive externality dominant, (i) the licensee can always achieve a higher profit under the WPS scheme, (ii) the database can achieve a higher profits under the WPS scheme when the licensed channel quality is low, and (iii) the total network profit is higher under the WPS scheme.


%\item
%\emph{Market Equilibrium Analysis.}
%We first derive the WSD¡\UTF{00D8}s best purchasing behavior, and show how the market share of each database dynamically evolves over time.
%We first characterize the equilibrium market shares of databases ({market equilibrium}) systematically given the information prices of databases.
%Based on this, we further derive the
%equilibrium prices of two databases (game equilibrium) in the oligopoly price competition game.
%the optimal information pricing plan that maximizes the database operator's revenue.

%\item
%\emph{Layer-III (Market Equilibrium):}
%%We study the equilibrium of the proposed hybrid information market systematically.
%%We also find a sufficient condition which the positive network externality needs to satisfy in order to guarantee the
%%\db's and the \lh's market shares converge to a unique stable market equilibrium under.
%We analyze the WSD users' best purchasing behaviours, and show how the market dynamically evolves over time.
%We further characterize the market equilibrium, wherein no user has the incentive to change its behaviour.

%\item
%\emph{Layer-III (Market Equilibrium):}
%\rev{We study the impact of two network effects on the WSD users' best purchasing behaviors. We show that if the system is congestion effect dominates, the users purchasing dynamics converges to unique stable points. We also show that some incentive policy is needed to guarantee the convergence of the users purchasing dynamics in the positive network externality dominant system.}

%\item
%\emph{Layer-II (Price Competition Game Equilibrium):}
%%We formulate the competition between the \db~and the \lh~as a non-cooperative game, and analyze the Nash equilibrium of the competition game systemically using the supermodular game theory.
%We analyze the database operator's and the TV licensee's best pricing decisions, and characterize the Nash equilibrium of the pricing competition game.
%%To do this, we first transform the original price competition game into the market share competition as there is a one-to-one correspondence between the achieved market equilibrium and the information price. Then we analyze the Nash equilibrium of the market share competition game systemically using the supermodular game theory.

%\item
%\emph{Layer-II (Price Competition Game Equilibrium):}
%\rev{We analyze the pricing equilibrium in the database operator's and the TV licensee's pricing competition game, and characterize how the pricing equilibrium can be achieve in practical system.}
%%We analyze the database operator's and the TV licensee's best pricing decisions, and characterize the Nash equilibrium of the pricing competition game.


%\item
%\emph{Layer-I (Commission Bargaining Solution):}
%We adopt the Nash bargaining framework to achieve a fair and Pareto-efficient
%commission charge, under both revenue sharing scheme (RSS) and wholesale pricing scheme (WPS).

%\item
%\emph{Performance Analysis:}
%%We characterize the outcome of \db-to-\lh~bargaining under both revenue-sharing-market and wholesale-price-market.
%%We show how the \db~and the \lh~improve their respective profit using either a revenue sharing policy or wholesale price policy with bargaining. We study the impact of these two policy on the bargaining outcome comprehensively.
%%We quantify the impact of the databases' initial market shares and information prices on the market equilibrium.
%Numerical results show that using our proposed commission bargaining solution,
%(i) The database can achieve a higher revenue under the RSS scheme than the WPS scheme, while licensee can achieve a higher revenue under the WPS scheme than the RSS scheme;
%(ii) The social welfare under the RSS scheme is higher than that under the WPS scheme.
%
%\item
%\emph{Performance Analysis:}
%\rev{
%We provide a discussion on which scheme the database, the licensee, and the system regulator should consider implementing. Specially, the database and the system regulator are suggested to choose WPS system only when the positive network externality is the dominant network effect in the system. Otherwise, RSS scheme is a better choice for both of them. For the licensee, WPS is a better choice unless the negative network externality significantly dominates the positive network externality.
%%(i) It is better for the database to choose RSS in most cases except the positive network externality effect significantly dominates the negative network externality; (ii) WPS is a better choice for the licensee unless the negative network externality significantly dominates the positive network externality; (iii) It is better to choose WPS from the network regulator's perspective if the positive network externality is the dominant network effect. Otherwise, RSS would be a better choice.
%}


\end{itemize}

%The rest of the paper is organized as follows. ...


%The rest of the paper is organized as follows.
%In Section \ref{sec:model}, we present the system model.
%In Sections \ref{sec:user_subscript}-\ref{sec:layer1},
%we analyze the market equilibrium in layer III, the price competition game game in layer II, and the commission bargaining solution in layer I, respectively.
%In Section \ref{sec:simulation}, we provide the simulation results.
%Finally, we conclude in Section \ref{sec:con}.




==> Latex_ParticipateSensing_infocom_camera/Section_Bargaining.tex <==
%!TEX root = main_hybrid_market.tex
%SourceDoc main_hybrid_market.tex
\vspace{-2mm}
\section{Layer I -- Commission Bargaining Solution}\label{sec:layer1}


%\begin{figure*}
%  \centering
%  \vspace{-2mm}
%%  \includegraphics[width=2.2in]{fig_w_bar}
%  \includegraphics[width=2.2in]{fig_w_fixed_network_effect}
%  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%  \includegraphics[width=2.2in]{Fig_NE_price_fixed_network_effect}
%%  \includegraphics[width=2.2in]{Fig_NE_market_share_fixed_network_effect}
%\vspace{-2mm}
%  \caption{(a) Equivalent wholesale price, (b) the \db's and the \lh's retail price (where LH denotes Licensee and DB denotes database) vs $\RL$ under revenue sharing scheme(RSS) and wholesale price scheme(WPS)}.\label{fig:price-vs-diff-L}
%%  , and (c) the \db's and the \lh's market share vs $\RL$ under revenue-sharing-scheme(RSS) and wholesale-price-scheme(WPS).}
%  \vspace{-5mm}
%\end{figure*}


%In this section, we study the commission negotiation among the database and the spectrum licensee in Layer I, based on the predictions of the game equilibrium in Layer II and the market equilibrium in Layer III.
%Specifically, under the RSS scheme, the database and the spectrum licensee  negotiate the revenue sharing factor $\delta \in [0, 1]$, while under the WPS scheme, they negotiate the wholesale price $\w \geq 0$.

In this section, we study the commission negotiation among the database and the spectrum licensee in Layer I, based on their predictions of the price equilibrium in Layer II and the market equilibrium in Layer III.

\rev{
Specifically, we want to find a feasible revenue sharing percentage $\delta \in [0, 1]$ under RSS that is \emph{satisfactory} for both the database and the spectrum licensee.
}
%Specifically, we want to find a feasible revenue sharing percentage $\delta \in [0, 1]$ under RSS, or a feasible wholesale price $\w \geq 0$ under WPS, that is \emph{satisfactory} for both the database and the spectrum licensee.
We formulate the commission negotiation problem as a \emph{one-to-one bargaining}, and study the bargaining solution using the Nash bargaining theory \cite{harsanyi1977bargaining}.

%\vspace{-2mm}
%\subsection{Revenue Sharing Percentage $\delta$-Bargaining under RSS}\label{sec:layer1-rss}
%
%We first study the revenue sharing scheme, where we want to determine this revenue sharing percentage $\delta \in [0, 1]$ based on the Nash bargaining theory, which is expected to be satisfactory to both the database and the licensee.

Following the Nash bargaining framework, we first derive the database's and the licensee's payoffs when reaching an agreement and when \emph{not} reaching any agreement (hence reaching the disagreement).
%Notice that reaching an agreement
%(say $\delta$) implies that the database will provide the spectrum market platform for the licensee, and charge a fixed percentage $\delta$ of revenue from the licensee; while reaching the disagreement implies that the database will \emph{not} provide the spectrum market platform for the licensee, hence there will be no spectrum market and the hybrid market degenerates to a pure information market.\footnote{Here, we assume that there is no third-party spectrum market platform for the spectrum licensee.}
Specifically, when reaching an agreement $\delta$, the database's and the licensee's payoffs are  $\Udbrs (\delta)$ and $\Uslrs (\delta)$ derived in
Section \ref{sec:layer2}, respectively.
When not reaching any agreement (reaching the disagreement), the licensee's profit is $\Uslo = 0$, and the database's profit is $\Udbo = \pa^{\dag} \cdot \Proba^{\dag}(\pa^{\dag}) $, where $\pa^{\dag}$ and $\Proba^{\dag}(\pa^{\dag})  $ are the database's optimal price and the corresponding market share in the pure information market.\footnote{Note that such an optimal price and market share can be derived in the same way as in Section \ref{sec:layer2}, by simply setting $\RL = 0$.}
Then, the Nash bargaining solution is formally given by
\begin{equation}\label{eq:NBS-RS}
\begin{aligned}
\max_{\delta \in [0,1]}~ &\left( \Udbrs(\delta) - \Uslo \right) \cdot \left( \Uslrs(\delta) - \Udbo \right) \\
\text{s.~t.~} & \Udbrs(\delta) \geq \Uslo,~~ \Uslrs(\delta) \geq \Udbo.
\end{aligned}
\end{equation}

Note that analytically solving (\ref{eq:NBS-RS}) may be difficult, as it is hard to characterize the analytical forms of $\Udbrs(\delta)$  and $\Uslrs(\delta) $.
Nevertheless, we notice that the bargaining variable $\delta$ lies in closed and bounded range of $[0,1]$, and the objective function of (\ref{eq:NBS-RS}) is bounded.
Hence, there must exist an optimal solution for (\ref{eq:NBS-RS}), which can be found by using many one-dimensional search methods \rev{(e.g., \cite{bargai2001search})}.

%transform (\ref{eq:NBS-RS}) into an equivalent optimization problem on a closed and bounded feasible set. Thus, we can show the existence of the optimal solution of (\ref{eq:NBS-RS}) in the following proposition.

%The simulation results that the objective function in (\ref{eq:NBS-RS}) is a concave function. Thus, we have the following NBS for the \db~to~\lh~revenue sharing bargaining problem:
%
\vspace{-2mm}
\begin{proposition}[$\delta$-Bargaining Solution]\label{lemma:existence-NBS}
There must exist an optimal solution for the problem (\ref{eq:NBS-RS}). \rev{If the objective function of (\ref{eq:NBS-RS}) is monotonic, the optimal solution is unique.}
%\com{unique?}
%\com{unique under what conditions ... }
%In addition, the solution can be solved by numerical one-dimensional search.
\end{proposition}
\vspace{-2mm}

%
%
%For the basic revenue-sharing market, an agreement between the \db~and \lh~is as follows: If the \db~displays the \lh's information on the database's online trading platform, \lh~has to pay the database $\delta$, $0 < \delta < 1$, out of the total revenue. Hence, the utility pairs over this agreement are:
%\begin{equation}\label{eq:db-profit-dynamic-rv}
%\begin{aligned}
%\Udbars(\delta) &=  \pl^{*}(\delta) \cdot \Probl^{*}( \pl^{*}, \pa^{*}  ) \cdot (1 - \delta )
%\end{aligned}
%\end{equation}
%\begin{equation}\label{eq:sl-profit-dynamic-rv}
%\begin{aligned}
%\Uslars(\delta) &= \pa^{*}(\delta) \cdot \Proba^{*}(\pl^{*}, \pa^{*}) + \pl^{*}(\delta) \cdot \Probl^{*}(\pl^{*}, \pa^{*})\cdot \delta
%\end{aligned}
%\end{equation}
%
%
%If the \db~and the \lh~fail to reach such an agreement, the disagreement outcome is as follows: the \lh~cannot sell or lease its spectrum to \eus~and gain zero profit, while the \db~serves \eus~with TV channels only and gain profit from selling advanced TV channels information to \eus. In such case, the utilities of both the \db~and the \lh~can be written as:
%\begin{equation}\label{eq:sl-profit-dynamic-disagree}
%\begin{aligned}
%\Uslo &= 0
%\end{aligned}
%\end{equation}
%\begin{equation}\label{eq:db-profit-dynamic-rv}
%\begin{aligned}
%\Udbo &= \pa^{\ddag} \cdot \Proba^{\ddag}(\pa^{\ddag})
%\end{aligned}
%\end{equation}
%where $\pa^{\ddag}$ and $\Proba^{\ddag}$ are the optimal price and market share of the \db~under the information market\footnote{In such a information market, \eus~can only access to TV channels and choose to purchase the \db's advanced information or not. In such case, the \db's optimal market share and price satisfy: $ (1 - \Proba^{\ddag}) \cdot \gy(\Proba^{\ddag}) - \pa^{\ddag} = 0$. }.
%
%Then a bargaining game between the \db~and the \lh~can be written as $\mathcal{G}_{\textsc{(i)}} = ( \{ \lh, \db\}, A, D,  \{ \Usla, \Udba \} )$, where
%\begin{itemize}
%\item $\{ \lh,\db \}$ is the set of game players;
%\item  $A$ is a set of possible agreements and $D$ is the disagreement event;
%\item $\Udbars$ is the utility function of spectrum licensee and $\Uslars$ is the utility function of the database over the set $A \bigcup\{ D\}$.
%\end{itemize}
%
%
%The Nash Bargaining Solution (NBS) is an agreement $\delta^{*} \in A$ that solves the following problem:
%\begin{equation}\label{eq:NBS-RS}
%\begin{aligned}
%\max_{\delta \in A}~ &\bigg( \Udbars(\delta) - \Uslo \bigg) \cdot \bigg( \Uslars(\delta) - \Udbo \bigg) \\
%\text{s.~t.~} & \Udbars(\delta) \geq \Uslo,~~ \Uslars(\delta) \geq \Udbo.
%\end{aligned}
%\end{equation}

%We notice that the Nash Bargaining Solution $\delta$ is bounded in $[0,1]$. Hence, we can transform (\ref{eq:NBS-RS}) into an equivalent optimization problem on a closed and bounded feasible set. Thus, we can show the existence of the optimal solution of (\ref{eq:NBS-RS}) in the following proposition.
%
%%The simulation results that the objective function in (\ref{eq:NBS-RS}) is a concave function. Thus, we have the following NBS for the \db~to~\lh~revenue sharing bargaining problem:
%%
%\begin{proposition}\label{lemma:existence-NBS}
%There must exist at least one optimal solution for the optimization problem (\ref{eq:NBS-RS}). In addition, the optimal solution can be effectively found through numerical methods such as the exhaustive search.   \end{proposition}


%To find the optimal Nash Bargaining Solution, we perform a grid search over the revenue sharing value $\delta \in [0,1]$. We choose the agreement $\delta$ for which we find yields the highest bargaining gain for the \db~and the \lh.

%\begin{figure}
%  \centering
%  \includegraphics[width=3.2in]{fig_revenue_sharing_low_L}
%  \includegraphics[width=3.2in]{fig_revenue_sharing_large_L}
%\vspace{-5mm}
%  \caption{Profit under different bargaining agreements when (i) the expected data rate the licensed spectrum can provide is $L = 7$, (ii) the expected data rate the licensed spectrum can provide is $L = 10$ }\label{fig:profit-vs-delta}
%\vspace{-6mm}
%\end{figure}

%Figure \ref{fig:profit-vs-delta} shows that value of (\ref{eq:NBS-RS}) with different bargaining agreement, i.e.,$\delta$. The figure shows that there exist an unique Nash Bargaining Solution (NBS). The left figure of Figure \ref{fig:profit-vs-delta} shows that when the expected data rate of exclusive usage is small (i.e., $L = 7$), the NBS is $\delta = 0$, i.e., no revenue sharing between the database and the spectrum licensee. This is because the benefit of exclusive usage is small. Hence, more and more end-users are willing to access to the TV channels. In such case, reducing the congestion of TV channels brings more benefit to the database than collecting revenues from the spectrum licensee does. The database, therefore, are willing to display the licensee spectrum information for free. However, as the right figure of Figure \ref{fig:profit-vs-delta} shows that, the licensed spectrum attracts more end-users when the exclusive usage's benefit increases. In such case, the database requires the spectrum licensee to share certain revenue in order to compensate the database's own revenue loss.


%\vspace{-3mm}
%\subsection{Wholesale Price $\w$-Bargaining under WPS}\label{sec:layer1-wps}
%
%We now study the wholesale pricing scheme, where the database charges the spectrum licensee a fixed wholesale price $\w\geq 0$ for each successful transaction.
%Similarly, our focus is to determine this wholesale price $\w \geq 0$ based on the Nash bargaining theory.
%
%
%When reaching an agreement $\w$, the database's and the licensee's payoffs are  $\Udbwp (\w)$ and $\Uslwp (\w)$ derived in
%Section \ref{sec:layer2-wps}, respectively.
%When not reaching any agreement (reaching the disagreement), the licensee's profit is $\Uslo = 0$, and the database's profit is $\Udbo = \pa^{\dag} \cdot \Proba^{\dag}(\pa^{\dag}) $, which is the same as that under RSS (Section \ref{sec:layer1-rss}).
%The bargaining problem is
%\begin{equation}\label{eq:NBS-WP}
%\begin{aligned}
%\max_{\w \geq 0}~ &\left( \Udbwp (\w) - \Uslo \right) \cdot \left( \Uslwp (\w) - \Udbo \right) \\
%\text{s.~t.~} & \Udbwp (\w)  \geq \Uslo,~~ \Uslwp (\w) \geq \Udbo.
%\end{aligned}
%\end{equation}

%
%
%%
%%
%%
%%Using a similar approach in the revenues sharing market, we can also formulate the Nash Bargaining Problem in the Wholesale-Price-Based Market except the \lh's utility function $\Usla$ and the \db's utility function $\Udba$ are changed into:
%%\begin{equation}\label{eq:db-profit-dynamic-wp}
%%\begin{aligned}
%%\Udbawp(\w) &=  \big( \pl^{*}(\w) - \w \big) \cdot \Probl^{*}(\pl^{*}, \pa^{*})
%%\end{aligned}
%%\end{equation}
%%\begin{equation}\label{eq:sl-profit-dynamic-wp}
%%\begin{aligned}
%%\Uslawp(\w) &= \pa^{*} \cdot \Proba^{*}(\w) + \w \cdot \Probl^{*}(\pl^{*}, \pa^{*})
%%\end{aligned}
%%\end{equation}
%%
%%The Nash Bargaining Solution (NBS) is an agreement $\w^{*} \in A$ that solves the following problem:
%%\begin{equation}\label{eq:NBS-WP}
%%\begin{aligned}
%%\max_{\w \in A}~ &\bigg( \Udbawp(\w) - \Uslo \bigg) \cdot \bigg( \Uslawp(\w) - \Udbo \bigg) \\
%%\text{s.~t.~} & \Udbawp(\w) \geq \Uslo,~~ \Uslawp(\w) \geq \Udbo.
%%\end{aligned}
%%\end{equation}
%
%We further notice that we can restrict the bargaining variable $\w$ within a closed and bounded set, say $[0, \RL]$, while not affecting the optimality of the solution.
%This is because any $\w > \RL$ is meaningless, where no user will choose the leasing service.
%%We further notice that  the objective function of (\ref{eq:NBS-WP}) is bounded.
%Hence, there must exist an optimal solution for (\ref{eq:NBS-WP}), and which can be found effectively through numerical search.
%
%
%
%
%
%%
%%We can also notice that the Nash Bargaining Solution $\w$ is bounded in $[0, \pl^{*}]$. On one hand, if $\w < 0$, the \db~will achieve a negative profit by providing \lch~information to {\eus}, and thus it has no incentive to set a wholesale price $\w$ less than $0$. On the other hand, if $\w > \pl^{*}$, the \lh~will achieve a negative profit from leasing \lch, and thus it has no incentive to lease its \lch. Accordingly, the \db~will always get a zero profit form the \lh.
%%Hence, we can show the existence of the optimal solution of (\ref{eq:NBS-RS}) in the following proposition.
%%
%%The simulation results that the objective function in (\ref{eq:NBS-RS}) is a concave function. Thus, we have the following NBS for the \db~to~\lh~revenue sharing bargaining problem:
%%
%\vspace{-2mm}
%\begin{proposition}[$\w$-Bargaining Solution]\label{lemma:existence-NBS-wp}
%%There must exist at least one optimal solution for the optimization problem (\ref{eq:NBS-WP}). In addition, the optimal solution can be effectively found through numerical methods such as the exhaustive search.
%There must exist an optimal solution for the problem (\ref{eq:NBS-WP}). If the objective function of (\ref{eq:NBS-WP}) is monotonic, the optimal solution is unique.
%%In addition, the solution can be solved by numerical one-dimensional search.
%\end{proposition}
%
%
%%Figure \ref{fig:profit-vs-w} shows that corresponding results. The figure shows that there exist an unique Nash Bargaining Solution (NBS). The left figure of Figure \ref{fig:profit-vs-delta} shows that when the expected data rate of exclusive usage is small (i.e., $L = 7$), the NBS is $w = 0$. The reasons are the same as that in the revenue sharing market. Moreover, the left figure of Figure \ref{fig:profit-vs-w} shows that when the wholesale price is large (i.e., $w > 0.4$), the benefit of the agreement decreases. This is because the higher wholesale price drives the licensee to increase its price of leasing/selling spectrum. In such case, the amount of sold licensed spectrum decreases which in turns decreases the revenue of the database.
%
%%\begin{figure}
%%  \centering
%%  \includegraphics[width=3.2in]{fig_differ_w_small_L}
%%  \includegraphics[width=3.2in]{fig_differ_w_large_L}
%%\vspace{-5mm}
%%  \caption{Profit under different bargaining agreements when (i) the expected data rate the licensed spectrum can provide is $L = 7$, (ii) the expected data rate the licensed spectrum can provide is $L = 10$ }\label{fig:profit-vs-w}
%%\vspace{-6mm}
%%\end{figure}
%


==> Latex_ParticipateSensing_infocom_camera/Section_DB_pricing.tex <==
%!TEX root = main_hybrid_market.tex
%SourceDoc main_hybrid_market.tex

\vspace{-2mm}
\section{Layer II -- Price Competition Game Equilibrium}\label{sec:layer2}

In this section, we study the price competition between the database and the spectrum licensee in Layer II, given the commission negotiation solution in Layer I and based on the market equilibrium prediction in Layer III.
We will analyze the  game equilibrium under the revenue sharing scheme (RSS).
We first define the price competition game (PCG) explicitly.
\begin{itemize}
\item
\emph{Players:} The database and the spectrum licensee;
\item
\emph{Strategies:} The database's strategy is the price  $\pa$ of its advanced information, and the licensee's strategy is the price  $\pl$ of its licensed channels;
\item
\emph{Payoffs:} The payoffs of players are defined in (\ref{eq:u1}) under RSS.
\end{itemize}
For convenience, we write the (unique) market equilibrium $\BProb^{*} = \{ \Probl^{*}, \Proba^{*} \}$ in Layer III as functions of prices $(\pl, \pa)$, i.e., $\Probl^{*} (\pl, \pa)$ and $\Proba^{*} (\pl, \pa)$.
Intuitively, we can interpret $\Probl^{*} (\cdot)$ and $\Proba^{*} (\cdot)$ as the \emph{demand} functions of the licensee and the \db, respectively.

%%Then we consider two kinds of competitive settings, namely revenue-sharing market and wholesale-price-based market.
%%In what follows, we first consider the revenue-sharing market, followed by the wholesale-price-based market.
%\vspace{-3mm}
%\subsection{Revenue Sharing Scheme --- RSS}\label{sec:layer2-rss}

Assume that the licensee shares a fixed percentage $\delta \in [0, 1]$ of revenue with the database. Then, 
%We fist study the game equilibrium under the revenue sharing scheme, where the licensee shares a fixed percentage $\delta \in [0, 1]$ of revenue with the database.
by (\ref{eq:u1}), the payoffs of the \lh~and the \db~can be written as:
\begin{equation}\label{eq:sl-profit-dynamic-rv}
\left\{
\begin{aligned}
\Uslrs(\pl , \pa) & = \pl \cdot \Probl^{*}(\pl, \pa) \cdot (1 - \delta),
\\
%\end{aligned}
%\end{equation}
%\begin{equation}\label{eq:db-profit-dynamic-rv}
% \begin{aligned}
\Udbrs(\pl , \pa) &= \pa \cdot \Proba^{*}(\pl, \pa) + \pl \cdot \Probl^{*}(\pl, \pa) \cdot \delta.
\end{aligned}
\right.
\end{equation}

%Then, the price competition game between the database and the licensee can be written as $\Gamma_{\textsc{(i)}} = ( \mathcal{J}, \{\p_j\}_{j\in\mathcal{J}},  \{\U_j\}_{j \in \mathcal{J}} )$, where
%%$\Gamma_{\textsc{(i)}} = ( \{ \lh, \db \}, \{ \pl, \pa \}, \{ \Uslrs, \Udbrs \})$, where
%\begin{itemize}
%\item $\mathcal{J} = \{ \lh, \db \}$ is the set of game players;
%\item $\{\p_j\}_{j\in\mathcal{J}}$ is the strategy of player $j$: $\pl$ is the strategy of the \lh~while $\pa$ is the strategy of the \db;
%\item $\{\U_j\}_{j \in \mathcal{J}}$ is the payoff function of player $j$: $\Uslrs$ is the payoff of spectrum licensee defined in (\ref{eq:sl-profit-dynamic-rv}) and $\Udbrs$ is the payoff of the database defined in (\ref{eq:db-profit-dynamic-rv}).
%\end{itemize}
%%\com{Yuan: I am not quite sure about what does "Define in a Game environment."?}

\begin{definition}[Nash Equilibrium]\label{def:nash}
A pair of prices $( \pl^{*}, \pa^{*} )$ is called a Nash equilibrium, if
\begin{equation}\label{eq:db-price-dynamic}
\left\{
\begin{aligned}
\textstyle\pl^{*} & = \arg \max_{\pl \geq 0}\ \Uslrs(\pl , \pa^{*}),
\\
\textstyle\pa^{*} & = \arg \max_{\pa \geq 0}\ \Udbrs(\pl^{*} , \pa).
\end{aligned}
\right.
\end{equation}
\end{definition}

It is notable that directly solving the Nash equilibrium is very challenging, due to the difficulty in analytically characterizing the market equilibrium $\{\Probl^{*}(\pl, \pa),\Proba^{*} (\pl, \pa) \}$ under a particular price pair $\{\pl, \pa\}$.
%It is very challenging to solve the Nash equilibrium of the game $\Gamma$ directly, due to the difficulty in characterizing the equilibrium market share $\{\Probl^{*}(\pl, \pa),\Proba^{*} (\pl, \pa) \}$.
To this end, we transform the original price competition game (PCG) into an
equivalent \emph{market~share~competition game} (MSCG).
The key idea is to view the market share as the strategy of the database or the licensee, and the prices as functions of the market shares.

Specifically, we notice that under the uniqueness condition (\ref{eq:stable_condition}), there is a \emph{one-to-one} correspondence between the market equilibrium $\{\Probl^{*}, \Proba^* \}$ and the prices  $\{\pl, \pa\}$.
%\footnote{\rev{It can be shown that if the game $\Gamma$ has Nash Equilibrium, it must satisfy $ 1> \left.\thlb(\Probl)\right|_{\Probl = 0} > \left. \thab(\Proba) \right|_{\Proba = 0} > 0$. Hence, we can get the relationship between the market equilibrium and the price from from (\ref{eq:NE-pt-22}). According to Theorem \ref{thrm:stable-eq_pt}, there exist unique solution of (\ref{eq:NE-pt-22}) given any price pair. Hence, we can obtain the one-to-one correspondence between the market equilibrium and the price.}}.

In this sense, once the \lh~and the \db~choose the prices $\{\pl, \pa\}$, they have equivalently chosen the market shares $\{\Probl^{*}, \Proba^* \}$.
Hence, we obtain the equivalent {market share competition game}---MSCG, where the strategy of each player is its market share (i.e., $\Probl$ for the licensee and $\Proba$ for the database), and the prices $\{\pl, \pa\}$ are functions of the market shares $\{\Probl , \Proba  \}$.
{Substitute $\thla=\frac{\pl-\pa}{\RL - \RA}$ and $\thab=\frac{ \pa}{ \RA- \RB }$ into (\ref{eq:NE-pt-22}), we can derive the inverse function of (\ref{eq:NE-pt-22}), where prices are functions of market shares, i.e.,\footnote{We omit the trivial case in (\ref{eq:NE-pt-1}), where the database has a zero market share, as this will never the case at the pricing equilibrium of Layer II.}}
\begin{equation}\label{eq:price-market-share-rs}
\textstyle
\left\{
  \begin{aligned}
  \textstyle  \pl(\Probl , \Proba )   = & ( 1 - \Probl ) \cdot \left( \RL - \fx(1-\Probl) - \gy(\Proba) \right)   \\
&  + ( 1 - \Probl - \Proba )\cdot \gy(\Probl) , \\
 \textstyle  \pa (\Probl , \Proba ) =& ( 1 - \Probl - \Proba )\cdot \gy(\Proba).
   \end{aligned}
   \right.
\end{equation}
Accordingly, the payoffs of two players can be written as:
\begin{equation}\label{eq:sl-profit-dynamic-rv-xx}
\left\{
\begin{aligned}
\textstyle
\Urslrs(\Probl , \Proba) & = \pl (\Probl, \Proba) \cdot \Probl \cdot (1 - \delta),
\\
\textstyle
\Urdbrs(\Probl , \Proba) & = \pa (\Probl , \Proba) \cdot \Probl + \pl (\Probl , \Proba) \cdot \Probl \cdot \delta.
\end{aligned}
\right.
\end{equation}
Similarly, a pair of market shares $(\Probl^*, \Proba^*)$ is called a Nash equilibrium of MSCG, if $\Probl^* = \arg \max_{\Probl} \Uslrs(\Probl , \Proba^*) $ and $\Proba^* = \arg \max_{\Proba} \Udbrs(\Probl^*, \Proba) $.


%
%
%
%the Thus, we transform the original price competition game into the following market share competition game, where
%$$
%\textstyle
%\Urslrs(\Probl , \Proba) = \pl^*(\Probl, \Proba) \cdot \Probl \cdot (1 - \delta)
%$$
%and
%$$
%\textstyle
%\Urdbrs(\Probl , \Proba) = \pa^*(\Probl , \Proba) \cdot \Probl + \pl^*(\Probl , \Proba) \cdot \Probl \cdot \delta
%$$
%and $\pl^* (\Probl , \Proba)$ and $\pa^* (\Probl , \Proba)$ is given by the following equation.
%%\begin{proposition}
%%Suppose $\Prob^{0}_1 < \Prob^{0}_2$. The information prices that leads to a market equilibrium $\{\Prob_1, \Prob_2\}$ are
%\begin{equation}\label{eq:price-market-share-rs}
%\left\{
%  \begin{aligned}
%  &\textstyle  \pl^* = [1 - \Probl ]\cdot [ \RL - \fx(\Probl) - \gy(\Proba) ]  + ( 1 - \Probl - \Proba )\cdot \gy(\Probl) \\
%  &\textstyle  \pa^* = ( 1 - \Probl - \Proba )\cdot \gy(\Proba)
%   \end{aligned}
%\right.
%\end{equation}
%The solution in the case of $\Prob^{0}_1 > \Prob^{0}_2$ is symmetric.
%\end{proposition}
We first show that the equivalence between the original PCG and the above MSCG.
\vspace{-2mm}
\begin{proposition}[Equivalence]\label{lemma:game_tranform}
If $\{\Probl^{*}, \Proba^*\}$ is a Nash equilibrium of MSCG, then $ \{\pl^*, \pa^*\}$ given by (\ref{eq:price-market-share-rs}) is a Nash equilibrium of the original price competition game PCG.
%If $ \{\pl^*, \pa^*\}$ is a Nash equilibrium of PCG, then $\{\Probl^{*}, \Proba^*\}$ given by (\ref{eq:NE-pt-22}) is a Nash equilibrium of MSCG.
\end{proposition}
\vspace{-2mm}
We next show that the MSCG is a supermodular game (with minor strategy transformation), and then derive the Nash equilibrium using the supermodular game theory \cite{topkis1998supermodular}.

%Our key results about the existence of NE is below.

%\begin{proposition}
%The market share competition game is a supermodular game with respect to $\Proba$ and $-\Probl$.
%\end{proposition}

\vspace{-2mm}
\begin{proposition}[Existence]\label{thrm:NE-existence}
The MSCG is a supermodular game with respect to $\Proba$ and $-\Probl$. Hence, there exists at least one Nash equilibrium $(\Probl^*, \Proba^*)$.
\end{proposition}
\vspace{-2mm}
%In order to prove the above theorem, we only need to treat $-\Probl$ as the action of \lh, then the market share competition game becomes a supermodular game.
%As a supermodular game guarantees at least one Nash equilibrium \cite{topkis1998supermodular},
%%There are several appealing properties for a supermodular game \cite{topkis1998supermodular}.
%%First, it guarantees at least one Nash equilibrium.
%%Second, if the Nash equilibrium is unique, a simple best response based algorithm globally converges to the Nash equilibrium.
%there exists at least one Nash equilibrium for the game $\widetilde{\Gamma}_{\textsc{(i)}}$,
%and thus at least one Nash equilibrium for the original price competition game ${\Gamma}_{\textsc{(i)}}$.

The following proposition further gives the uniqueness condition of the Nash equilibrium in MSCG.
\vspace{-2mm}
\begin{proposition}[Uniqueness]\label{thrm:NE-uniquness}
%For any non-negative revenue sharing percentage $\delta$, the market share competition game $\widetilde{\Gamma}_{\textsc{(i)}}$ has a unique market share equilibrium if the following condition holds:
The MSCG has a unique Nash equilibrium $(\Probl^*, \Proba^*)$, if
$$
 \textstyle - \frac{  \partial^2{ \Urslrs({\Prob}_{\textsc{l}} , \Proba) } }{ \partial{ (-{\Prob}_{\textsc{l}}) }^2 } \geq \frac{  \partial^2{ \Urslrs( {\Prob}_{\textsc{l}} , \Proba)  } }{ \partial{ {(-{\Prob}_{\textsc{l}}) } }\partial{ \Proba  } },
~
 \textstyle - \frac{  \partial^2{ \Urdbrs( {\Prob}_{\textsc{l}} , \Proba) } }{ \partial{ (-{\Prob}_{\textsc{l}}) }^2 } \geq \frac{  \partial^2{ \Urdbrs( {\Prob}_{\textsc{l}} , \Proba)  } }{ \partial{ { \Proba } }\partial{ (-{\Prob}_{\textsc{l}})  } }.
$$
%where $\bar{\Prob}_{\textsc{l}} = - \Probl$.
%\rev{
%$$
% \textstyle - \frac{  \partial^2{ \Urslrs(- \Probl , \Proba) } }{ \partial{ (- \Probl) }^2 } \geq \frac{  \partial^2{ \Urslrs( - \Probl , \Proba)  } }{ \partial{ {(- \Probl) } }\partial{ \Proba  } },
%~
% \textstyle - \frac{  \partial^2{ \Urdbrs(- \Probl , \Proba) } }{ \partial{ (- \Probl) }^2 } \geq \frac{  \partial^2{ \Urdbrs(- \Probl , \Proba)  } }{ \partial{ { \Proba } }\partial{ (- \Probl)  } },
%$$
%}
\end{proposition}
%\vspace{-2mm}
%\com{Why not state the condition directly in terms of -$\eta_L$? The strategy transformation is useful in the proof, but should not be used in the expression of Prop 5?}
%\com{Yuan: Because only the MSCG are supermodular game and the condition is only for the supermodular game. hence, we need to use $-\eta_L$. I think maybe we can only state the condition directly in terms of $\eta_L$, but it will over the space }
The above uniqueness conditions are quite general, and follow the standard supermodular game theory.
Next we provide a specific example to illustrate these conditions more intuitively.
Consider the following example: $\fx(\Proba + \Probb) = \alpha_1 - \beta_1 \cdot ( \Proba + \Probb )$ and $\gy(\Proba) = \beta_2 \cdot \Proba$. That is, both positive and negative network effects change linearly with the respective market shares.  In this example, we can obtain the following uniqueness condition:
$\RL - \alpha_1 - \beta_1 > \beta_2 $.
Namely, if $\RL$ is large enough or $\beta_2$ is small enough, there is a unique Nash equilibrium in MSCG.

%This condition implies that the benefit difference between the leasing service and the basic service should be larger than that between the advanced service and the basic service.
%\com{Yuan: Actually, from the database's profit function we should add one condition that $\Proba + 2 \cdot \Probl - 1 > 0$. Because the second inequality of (\ref{eq:dominant-diagonal}) is independent of $\RL$, $\alpha_1$, $\beta_1$, $\beta_2$. But I omit this condition....}

%\begin{figure}
%  \centering
%  \includegraphics[width=3.2in]{fig_price_BR_RS}
%  \includegraphics[width=3.2in]{fig_eta_BR_RS}
%%\vspace{-5mm}
%  \caption{Equilibrium price and market share under revenue-sharing-market}\label{fig:NE-RS}
%\vspace{-6mm}
%\end{figure}

Once we obtain the Nash equilibrium $(\Probl^*, \Proba^*)$ of MSCG, we can immediately obtain the Nash equilibrium $(\pl^*, \pa^*)$ of the original PCG by (\ref{eq:price-market-share-rs}).
It is notable that we may not be able to derive the analytical Nash equilibrium of MSCG, as we use the generic functions $\fx(\cdot)$ and $\gy(\cdot)$.
Nevertheless, thanks to the nice property of supermodular game, we can easily numerically compute the Nash equilibrium of MSCG through, for example, the simple best response iteration in \cite{report}.


%
%\rev{
%For a supermodular game,  several commonly used updating rules are guaranteed to converged to
%the NE \cite{topkis1998supermodular}.
%%In case of multiple fixed points, there exist two extreme one $\{ \Proba^{L}, \Probl^{L} \}$ and $\{ \Proba^{H}, \Probl^{H} \}$
%In this work, we use the following best response algorithm as in \cite{topkis1998supermodular}:
%Starting with an arbitrary market share vector $\BProb^{0}$, where 0 is the round index.
%At every round $k+1$, both the \db~and the \lh~update their market share based on their best response to its competitor's market share in the previous round $k$. That is,
%\begin{equation}\label{eq:BR_updated_lh}
%\begin{aligned}
%\Probl^{(k+1)} = \arg \max_{  \Probl \in [0,1] } \Urslrs(\Probl , \Proba^{k})
%\end{aligned}
%\end{equation}
%\begin{equation}\label{eq:BR_updated_db}
%\begin{aligned}
%\Proba^{(k+1)} = \arg \max_{  \Proba \in [0,1] } \Urdbrs(\Probl^{k} , \Proba)
%\end{aligned}
%\end{equation}
%The above procedure continues until the market share equilibrium reached.
%Note that if both the \db~and the \lh~use best response algorithm update starting form their smallest (largest) element of their strategy set, then the strategies monotonically converge to the smallest (largest) NE market share. As the \db~owns the online platform and can put its advanced service as high priority, we always assume that the initial market share vector as $\BProb^{0} = \{ \Probl^{0} = 0, \Proba^{0} = 1 \}$.
%%Formally, we show this in Algorithm \ref{alg:round_robin}.
%%\footnote{\rev{Note that the updating in Algorithm \ref{alg:round_robin} can be asynchronous (i.e., not every one updates at each round). We provide the details in \cite{techrpt}.}}
%
%%\begin{algorithm}
%%\small
%%\DontPrintSemicolon
%%\textbf{Initialization}\;
%%~~Each operator $m \in \M$ selects an initial price $\p_{m}(0)$ as any feasible value;\;
%%%~~Record
%%%the initial price vector $\bp(0)= \big(\p_{1}(0),\p_{2}(0),...,\p_{M}(0)\big)$ at the initial round $k=0$;\;
%%%\textbf{end initialization}\;
%%\For{each round $k=1,...,K_{\mathrm{end}}$}
%%%{$|\bp(k) - \bp(k-1)| > \delta$}
%%{
%%\For{each operator $m = 1 ,...,M$}
%%{Operator  $m$ chooses the service price $\p_{m}(k )$ at round $k$ according to (\ref{eq:BR_updated}), i.e., the price maximizing his profit under $\bp_{-m}(k-1)$;}
%%% Record the price vector $\bp(k )=(\p_{m}(k ))_{m\in\M}$ at round $k$;\;
%%\textbf{if} {$\p_m(k) == \p_m(k-1),\forall m\in\M $} \textbf{then} break;	\qquad \emph{// convergence}
%%}
%%\caption{Best response update algorithm}\label{alg:round_robin}
%%\end{algorithm}
%
%%\vspace{-6mm}
%\begin{proposition}[Convergence]\label{pro:convergence}
%{The best response update converges to the unique NE.}
%\end{proposition}
%}

%Due to space limit, we keep the proof in \cite{techrpt}.
%For more clarity, we illustrate the convergence of the  best response update Algorithm \ref{alg:round_robin} by simulations in Figure \ref{fig:convergence}.

%Figure \ref{fig:NE-RS} illustrates the convergence of the best response update algorithm under revenue sharing market.
%The following settings are used in our simulations: $\N = 200$, $\K = 10$, and the aggregated interference follow the log-normal distribution. The transmission data rate is defined by the Shannon capacity: $
%\rt(\InfTot) = \log( 1 + \frac{P}{\InfTot} )
%$. The end-user utility is affine function and is simply defined as the expected data rate: $\ut(R) = R$.
%The spectrum licensee has to pay the database $\delta = 0.6$ out of the total revenue.
%Note that such parameter setting is just for an illustrative purpose, and similar results can be found in other parameter setting. Figure \ref{fig:NE-RS} shows that the prices and market share converge to the equilibrium.
%Moreover, it shows that the \lh~who can provide a higher expected data rate can specify a higher service price and obtain a much higher market share in the equilibrium.
%On the contrary, the \db~can only specify a lower service price. This is because the expected data rate between the advance service and basic service is small. Hence, the high-valuation users are willing to pay a higher fee for exclusive usage, and the low-valuation users are willing to use TV \ch~for free. The \db~can only charge a small price to attract limited median-valuation users.

%\vspace{-3mm}
%\subsection{Wholesale Pricing Scheme --- WPS}\label{sec:layer2-wps}
%
%We now study the game equilibrium under the wholesale pricing scheme, where the database charges a fixed wholesale price $w \geq 0$ from each successful transaction of the licensee.
%By (\ref{eq:u2}), the payoffs of the \lh~and the \db~can be written as:
%\begin{equation}\label{eq:sl-profit-dynamic-whole}
%\left\{
%\begin{aligned}
%\Uslwp(\pl , \pa) &= ( \pl - \w) \cdot \Probl^{*}(\pl , \pa),
%\\
%%\end{aligned}
%%\end{equation}
%%\begin{equation}\label{eq:db-profit-dynamic-whole}
%%\begin{aligned}
%\Udbwp(\pl , \pa) &= \pl \cdot \Probl^{*}(\pl , \pa) + \w \cdot \Proba^{*}(\pl , \pa).
%\end{aligned}
%\right.
%\end{equation}
%
%%\begin{definition}[Nash Equilibrium]\label{def:nash-ws}
%%A pair of prices $( \pl^{*}, \pa^{*} )$ is called a Nash equilibrium, if
%%\begin{equation}\label{eq:db-price-dynamic}
%%\left\{
%%\begin{aligned}
%%\pl^{*} & = \arg \max_{\pl \geq 0}\ \Uslwp(\pl , \pa^{*}),
%%\\
%%\pa^{*} & = \arg \max_{\pa \geq 0}\ \Udbwp(\pl^{*} , \pa).
%%\end{aligned}
%%\right.
%%\end{equation}
%%\end{definition}
%
%With the similar analysis used in Section \ref{sec:layer2-rss}, we can transform the original price competiton game (PCG) into an equivalent market share competition game (MSCG), and show that the MSCG is a supermodular game.
%Due to the space limit, we leave the detailed discussions in \cite{report}.
%
%Although we use the similar method to derive the Nash equilibrium of the PCG game under both RSS and WPS, these two equilibria are quite different.
%Intuitively, under RSS, the objective of the database is consistent with that of the licensee.
%This can be shown by the common term in both players' payoffs given in
%(\ref{eq:sl-profit-dynamic-rv}).
%Hence, the database becomes less aggressive in terms of market competition under RSS.
%
%We further notice that the database's and the licensee's equilibrium payoffs (under Nash equilibrium) are functions of $\delta$ under RSS, and functions of $\w$ under WPS.
%Hence, we will also write the equilibrium payoff of the database as $\Udbrs (\delta)$ under RSS and $\Udbwp(\w)$ under WPS. Similarly, we will
%write the equilibrium payoff of the licensee as $\Uslrs (\delta)$ under RSS and $\Uslwp(\w)$ under WPS.



==> Latex_ParticipateSensing_infocom_camera/Section_Information_Market.tex <==
%!TEX root = main_hybrid_market.tex
%SourceDoc main_hybrid_market.tex


\section{Information Value} 

%Before we solve the three-stage model discussed in the previous section with backwards induction. We first need to characterize the utility provided by different service so that we can analyze the subscription choice of {\eus}. Hence, in the next section, we will analyze the value of information to {\eus}.
%

Before analyzing the hybrid market, we first need to compute the value of advanced information for those WSD users using the unregistered channels. 
In this section, we first characterize the interference level on each unregistered channel for each \eu~(using the unregistered \chs), which essentially defines the advanced information. 
Then, we establish a framework to evaluate the value of advanced information for the WSD users using the unregistered channels.

%\subsection{Basic Service and Advanced Service}
%As mentioned in the previous section, the basic service is mainly consisted of the available TV \chs~list, while the advanced service is the interference level on every available \ch~for a particular \eu~and is denoted as $\{\InfTot_{\k}\}_{k\in\Kset}$.
%
%For convenience, we illustrate the basic service and advanced service by the example in the following table.
%In the basic service, the database provides the available channel set (i.e., \{CH1, CH3, CH4, CH6\}) to a particular \eu. In the advanced service, the database provides the interference levels on available channels (i.e., \{$\InfTot_1$, $\InfTot_3$, $\InfTot_4$, $\InfTot_6$\}) to the \eu, in addition to the available channel set.
%
%\begin{table}[h]
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\textbf{Channel ID} & \textbf{CH1}& \textbf{CH2}& \textbf{CH3} & \textbf{CH4} & \textbf{CH5} & \textbf{CH6}
%\\
%\hline
%Availability & Yes & No & Yes & Yes & No & Yes
%\\
%\hline
%Interference Level & $\InfTot_1$ &  - & $\InfTot_3$ & $\InfTot_4$ &  - & $\InfTot_6$
%\\
%\hline
%\end{tabular}
%\end{table}

\subsection{Interference Information}
\label{sec:interference_info}

\com{iid over time is easier to understand, assuming that the number of users on the channel does not change, but the channel gains change over time due to fading.
however, we need to better justify the iid assumption over frequency. This relies on the assumption that the number of users on each channel (which is a random variable) is iid.
We need to explain
- why this is a good assumption (possible answer: users with basic service will randomly choose, hence the number of such users per channel will follow the same distribution. Users with advanced service will go to the channel with the minimum "actual" interference. If the interference among each pair of users is iid over time, then statistically the number of such users in each channel will also follow the same distribution. )
-  why under such an assumption the information market still is useful (possible answer: the market provides the accurate interference information instead of the statistical information.)
Some of the above detailed discussions can be deferred to later part (the bottom part of the 2nd column on this page). However, it is important to make sure that readers understand (at this point) that the iid assumption is justified to certain extent, instead of just convenient assumption for analytical purpose.
Finally, important assumptions need to be put into the "Assumption" environment. So here which one is the fundamental assumption we make, and which ones are actually derived from the assumption (and hence are not assumption themselves)?
}

\rev{
For each {\eu} $n\in \Nset$ operating on the TV \ch, each channel $\k$ is associated with an \emph{interference level}, denoted by  $\InfTot_{\n,\k}$, which reflects the aggregate interference from all other nearby devices (including TV stations
and other {\eus}) operating on this channel.
Due to the fast changing of wireless channels and the uncertainty of {\eus}' mobilities and activities, the interference $\InfTot_{\n,\k}$ is a random variable. We impose assumptions on the interference $\InfTot_{\n,\k}$ as follows.
\begin{assumption}\label{assum:iid}
For each {\eu} $n\in \Nset$, each channel $\k$'s interference level $\InfTot_{\n,\k}$ is \emph{temporal-independence} and \emph{frequency-independence}.
\end{assumption}

This assumption shows that
(i) the interference $\InfTot_{\n,\k}$ on channel $\k$ is independent identically distributed (iid) at different times, and (ii)
the interferences on different channels, $\InfTot_{\n,\k}, \k\in\Kset$, are also iid at the same time.\footnotesc{\rev{Note that the iid assumption is a reasonable approximation of the practical scenario (e.g., \cite{chang2009channel,jiang2009channel,zhou2011channel}). This is because {\eus} with basic service will randomly choose one TV \ch, hence the number of such {\eus} per channel will follow the same distribution. For {\eus} with advanced service, they will go to the TV \ch~with the minimum realized interference. If the interference among each pair of users is iid over time, then statistically the number of such users in each channel will also follow the same distribution. Note that even though all channel quality distributions are the same, the realized instant qualities of different channels are different. Hence, the advanced information provided by the \db~is still valuable as such an advanced information is accurate interference information.} }
As we are talking about a general \eu~$n$, \textbf{we will omit the {\eu} index $n$ in the notations (e.g., write $\InfTot_{\n,\k}$ as $\InfTot_{\k}$), whenever there is no confusion caused.}
Let $F_{\InfTot}(\cdot)$ and $f_{\InfTot}(\cdot)$ denote the cumulative distribution function (CDF) and probability distribution function (PDF) of $\InfTot_{\k}$, $\forall \k\in\Kset$.\footnotesc{In this paper, we will conventionally  use $F_X(\cdot)$ and $f_X(\cdot)$ to denote the CDF and PDF of a random variable $X$, respectively.}~~~~
}

Usually, a particular {\eu}'s experienced interference $\InfTot_{\k}$ on a \ch~$\k$ consistss of the following three components:
\begin{enumerate}
\item
$\InfTV_{\k}$: the interference from licensed TV stations;
\item
$\InfEU_{\k,m}$: the interference from another {\eu} $m$ operating on the same channel $k$;
\item
$\InfOut_{\k}$: any other interference from outside systems.
\end{enumerate}
The total interference on channel $k$ is
$
\InfTot_{\k} = \InfTV_k + \InfEU_k + \InfOut_k
$, where  $\InfEU_k  \triangleq \sum_{m \in \Nkset} \InfEU_{\k,m}$ is the total interference from all other {\eus} operating on channel $k$ (denoted by $\Nkset$).
Similar to $\InfTot_{\k}$, we also assume that  $ \InfTV_k , \InfEU_k , \InfEU_{\k,m}$, and $ \InfOut_k$ are random variables with \emph{temporal-independence} (i.e., iid across time) and \emph{frequency-independence} (i.e., iid across frequency).
We further assume that $\InfEU_{\k,m}$ is \emph{user-independence}, i.e., $\InfEU_{\k,m}, m\in \Nkset$, are iid.
{It is important to note that \textbf{different {\eus} may experience different interferences $\InfTV_k$ (from TV stations), $ \InfEU_{\k,m} $ (from another \eu~operating on the same \ch), and $ \InfOut_k$ (from outside systems) on a channel $k$, as we have omitted the \eu~index $n$ for all these notations for clarity.}}
\com{Similarly, the iid assumption over space is ok for Lk, Ik, and even Wk,m, but not for Wk which depends on the number of users on each channel? Need to explain.}

Next we discuss these interferences in more details.

\begin{itemize}
\item
The \db~is able to compute the interference $\InfTV_k$ from TV stations to every {\eu} (on channel $k$), as it knows the locations and channel occupancies of all TV stations.~~~~

\item
The \db~cannot compute the interference
$\InfOut_k$ from outside systems, due to the lack of outside interference source information.
Thus, the interference $\InfOut_{\k}$ will \emph{not} be included in a database's advanced information sold to {\eus}.~~~~~~~~

\item
The \db~may or may not be able to compute the interference $\InfEU_{\k,m}$ from another {\eu} $m$, depending on whether {\eu} $m$ subscribes to the \db's advanced service.
Specifically, if {\eu} $m$ subscribes to the advanced service, the \db~can predict its channel selection (since the {\eu} is fully rational and will always choose the channel with the lowest interference level indicated by the \db~at the time of subscription), and thus can compute its interference to any other \eu.
However, if {\eu} $m$ only chooses the \db's basic service, the \db~cannot predict its channel selection, and thus cannot compute its interference to other \eus.~~~~
\end{itemize}

For convenience, we denote $\Nkset^{[\A]}$, as the set of {\eus} operating on \ch~$k$ and subscribing to the \db's advance service (i.e., those choosing the strategy $\l = \A$), and $\Nkset^{[\B]}$ as the set of {\eus} operating on channel $k$ and choosing the \db's basic service (i.e., those choosing the strategy $\l = \B$).
That is, $\Nkset^{[\A]} \bigcup \Nkset^{[\B]} = \Nkset $.
Then, for a particular {\eu}, its experienced interference (on channel $k$) \textbf{known by the \db} is
% (and thus will be included in the database $\dbb_i$'s advanced service to this WSD) is
\begin{equation}\label{eq:known_inf}
\begin{aligned}
\textstyle
\InfKnown_{\k} \triangleq \InfTV_{\k} + \sum_{m \in \Nkset^{[\A]}} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from TV licensees and all {\eus} (operating on channel $k$)  subscribing to the \db's advanced service.
The \eu's experienced interference (on channel $k$) \textbf{\emph{not} known by the \db} is
% (and thus will not be included in the database $\dbb_i$'s advanced information) is
\begin{equation}\label{eq:unknown_inf}
\begin{aligned}
\textstyle
\InfUnknown_{\k}  \triangleq \InfOut_{\k} + \sum_{m \in \Nkset^{[\B]}} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from outside systems and all {\eus} (operating on channel $k$) choosing the \db's basic service.
Obviously, both $\InfUnknown_{\k}$ and $\InfKnown_{\k}$ are also random variables with temporal- and frequency-independence.
Accordingly, the total interference on {\ch} $\k$ for a {\eu} can be written as
$\textstyle
\InfTot_{\k} = \InfKnown_{\k} + \InfUnknown_{\k}.$~~~~~~

\textbf{Since the \db~knows only $\InfKnown_{\k}$, it will provide this information (instead of the total interference $\InfTot_k$) as the {advanced service} to a subscribing {\eu}.}
It is easy to see that the more {\eus} subscribing to the \db's advanced service, the more information the \db~knows, and the more accurate the \db~information will be.


Next we can characterize the accuracy of a database's information explicitly. Note that $\Proba$ and $\Probl$ denote the fraction of {\eus} choosing the advanced service and leasing licensed spectrum, respectively. Moreover, $(1 - \Proba - \Probl)$ denotes the fraction of {\eus} choosing the basic service.
Hence, there are $(1 - \Probl) \cdot \N$ {\eus} in the network that we consider operating on the TV \chs.
Due to the Assumption \ref{assum:iid}, it is reasonable to assume that each channel $k\in\Kset$ will be occupied by an average of $\frac{\N}{\K} \cdot ( 1 - \Probl)$ {\eus}.\com{Yuan: Do we need to add more explanation on this?}
%Let $\Prob_l$ denote the percentage of {\eus} subscribing to the advanced service of database $\dbb_l$ (called the \emph{market share} of database $\dbb_l$).
Then, among all $\frac{\N}{\K} \cdot ( 1 - \Probl)$ {\eus} operating on channel $k$, there are, \emph{on average}, $\frac{\N}{\K}\cdot\Proba$ {\eus}  subscribing to the \db's advanced service, and $\frac{\N}{\K}\cdot ( 1 - \Proba - \Probl )$ {\eus} choosing the \db's basic service.
That is, $| \Nkset | = \frac{\N}{\K} \cdot ( 1 - \Probl)$, $| \Nkset^{[\A]} | = \frac{\N}{\K}\cdot\Proba$, and $|\Nkset^{[\B]} | = \frac{\N}{\K}\cdot(1-\Proba-\Probl)$.\footnotesc{{Note that the above discussion is from the aspect of expectation, and in a particular time period, the realized numbers of {\eus} in different channels may be different.}}
Finally, by the {user-independence} of $\InfEU_{\k,m}$, we can immediately calculate the distributions of $ \InfKnown_{\k}$ and $ \InfUnknown_{\k}$ under any given market share $\Proba$ and $\Probl$ via (\ref{eq:known_inf}) and (\ref{eq:unknown_inf}).

\rev{
\subsection{Information Value}
Now we evaluate the value of the \db's advanced information to {\eus}, which is
reflected by the {\eu}'s benefit (utility) that can be achieved from this information.

We first consider the expected  utility of a {\eu} when choosing the \db's basic service (i.e., $\l=\B$).
In this case, the {\eu} will randomly choosing a \tvch~based on the information provided in the free basic service,
and its expected data rate is
\begin{equation}\label{eq:rate-random-fixed}
\begin{aligned}
\textstyle
\R_0( 1 - \Probl)  \textstyle = \Ex_{Z} [\rt(\InfTot)] = \int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z), \\
%\RB   \textstyle \triangleq \fx = \ut(\R_0) = \ut\left(\int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z)\right),
\end{aligned}
\end{equation}
%where $\R_0$ is the expected data rate and is given as follows.
%\begin{equation}\label{eq:rkgs}
%\begin{aligned}
%& \R_0  \textstyle = \Ex_{Z} [\rt(\InfTot)] = \int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z),
%\end{aligned}
%\end{equation}
where $\rt(\cdot)$ is the transmission rate function (e.g.,
the Shannon capacity) under any given interference.
As shown in Section \ref{sec:interference_info}, each channel $k\in\Kset$ will be occupied by an average of $\frac{\N}{\K} \cdot ( 1 - \Probl)$ {\eus} based on the Assumption \ref{assum:iid}. Hence,
$\R_0( 1 - \Probl) $ depends only on the distribution of the total interference $\InfTot_k$, and thus depends on the fraction of {\eus} operating on TV \chs~(i.e., $1 - \Probl$). Then the expected utility provided by the basic service is:
\begin{equation}\label{eq:utility-random-fixed}
\begin{aligned}
\textstyle
\RB(1 - \Probl) = \textstyle \ut\bigg(\R_0( 1 - \Probl)\bigg),
% = \ut\left(\int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z)\right),
\end{aligned}
\end{equation}
where $\ut(\cdot)$ is the utility function of the \eu. We can easily check that
the more {\eus} operating on the TV \chs, the higher value of $\InfTot_k$ is, and thus the lower expected utility provided by the basic service. Hence, the basic service's expected utility reflects the congestion level of the TV \chs.
We use the function $\fx(\cdot)$ to characterize the congestion effect and have $\fx(1 - \Probl) = \RB( 1 - \Probl)$.
%while not on the specific distributions of $\InfKnown_k$ and $\InfUnknown_k$. This implies that the accuracy of the \db's information does not affect the utilities of those {\eus} choosing the basic service. However, as t

Then we consider the expected utility of a {\eu} when subscribing to the \db's advance service.
In this case, the {\db} returns the interference $\{\InfKnown_{k}\}_{k\in\Kset}$ to the {\eu} subscribing to the advanced service, together with the basic information such as the available channel list.
For a rational {\eu}, it will always choose the channel with the minimum $\InfKnown_{k}$ (since $\{\InfUnknown_{k}\}_{k\in\Kset}$ are iid).
Let $\InfKnownMin^{[l]} =  \min\{ \InfKnown_{1},  \ldots, \InfKnown_{K} \} $ denote the minimum interference indicated by the \db's advanced information.
Then, the actual interference experienced by a {\eu} (subscribing to the \db's advanced service) can be formulated as the sum of two random variables, denoted by $\InfTotA = \InfKnownMin + \InfUnknown$. Accordingly, the {\eu}'s expected data rate under the strategy $\l = \A$ can be computed by
\begin{equation}\label{eq:rate-pay-fixed}
\begin{aligned}
\Ra(\Proba, \Probl) & \textstyle = \Ex_{\InfTotA} \big[ \rt \left( \InfTotA \right) \big] = \int_z \rt(z)  \mathrm{d} F_{\InfTotA}(z),
%\\
%\RA & \textstyle  \triangleq \ut\left(\Ra\right) = \ut\left(\int_z \rt(z)  \mathrm{d} F_{\InfTotA}(z)	\right) ,
\end{aligned}
\end{equation}
where
$F_{\InfTotA}(z)$ is the CDF of $\InfTotA$. It is easy to see that $\Ra$ depends on the distributions of $\InfKnown_k$ and $\InfUnknown_k$, and thus depend on the market share $\Probl$ and $\Proba$.
Thus, we will write $\Ra$ as $\Ra(\Probl,\Proba)$. Accordingly, the advanced service's utility is:
 \begin{equation}\label{eq:utility-pay-fixed}
\begin{aligned}
%\Ra & \textstyle = \Ex_{\InfTotA} \big[ \rt \left( \InfTotA \right) \big] = \int_z \rt(z)  \mathrm{d} F_{\InfTotA}(z),
%\\
\RA(\Probl,\Proba) & \textstyle  \triangleq \ut\bigg( \Ra( \Probl,\Proba ) \bigg)
%= \ut\left(\int_z \rt(z)  \mathrm{d} F_{\InfTotA}(z)	\right) ,
\end{aligned}
\end{equation}

Note that the congestion effect also affects the value of $\RA$. However, compared with the utility of {\eu} choosing basic service, the benefit of a {\eu} subscribing to the \db's advanced information is coming from the $\InfKnownMin^{[l]}$, i.e., the minimum interference indicated by the \db's advanced information. As the value of $\InfKnownMin^{[l]}$ depends on the $\Proba$ only, we can get the approximation $\RA = \fx(1 - \Probl) + \gy(\Proba)$, where function $\gy(\cdot)$ characterize the benefit brought by $\InfKnownMin^{[l]}$ and denotes the positive network effect.
\com{This is a key assumption, by writing $\RA(\Probl,\Proba)$ as two separate terms. How to justify this? How to verify this? }


%We define $\RB$ and $\RA$ as follows:
%\begin{equation}\label{eq:utility-service-general}
%\begin{aligned}
%\RB & \textstyle \triangleq \fx(1 - \Probl),
%\\
%\RA & \textstyle \triangleq \fx( 1 - \Probl) + \gy(\Proba).
%\end{aligned}
%\end{equation}
%where the function $\fx(\cdot)$ denotes the \emph{congestion effect}, and the function $\gy(\cdot)$ denotes the \emph{positive network effect}.

%Note that the congestion effect depends on the total number of {\eus} in the TV \chs, because the more {\eus} are, the higher co-interference is. The positive network effect depends only on the number of {\eus} subscribing to the \db's advanced service. This is because the more {\eus} subscribing to the \db's advanced service, the more information such as the {\eus}' TV \ch~selection and the transmission power the \db~knows, and the more accurate the information about the best available \ch~will be.

By further checking the properties of $\RB(1 - \Probl)$ and $\RA(\Probl,\Proba)$, we have the following assumptions.

\begin{assumption}\label{assum:congestion}
The function $\fx(\cdot)$ is nonnegative, nonincreasing, convex, and continuously differentiable.
\end{assumption}

\begin{assumption}\label{assum:positive}
The function $\gy(\cdot)$ is nonnegative, nondecreasing, concave, and continuously differentiable.
\end{assumption}

The convexity requirement of $\fx$ due to the characteristic of interference in the expected data rate and is a common assumption in wireless networking (see e.g., \cite{shetty2010congestion,acemoglu2010congestion,johari2010congestion} and references therein). The concavity requirement of $\gy$ results form decelerating returns to increased the number of {\eus} subscribing to the advanced service. This is because in sharing the TV white space network, when the number of {\eus} is small, then each additional \eu~makes the network significantly more useful; but an additional \eu~may go unnoticed when added to a TV white space network.

Because function $\fx$ and $\gy$ can characterize the information value to the {\eus}, we begin to solve the three-stage model discussed in the previous section with backwards induction.
}

%\textbf{Problem Formulation.}
%Suppose that each {\eu} is rational, and will always choose the strategy that maximizes its payoff.
%We are interested in the following problems: given the information prices $\{\p_1, \p_2\}$ and initial market shares $\{\Prob^0_1, \Prob^0_2 \}$ of databases, how these market shares dynamically evolve and what is the market equilibrium?




==> Latex_ParticipateSensing_infocom_camera/Section_Model.tex <==
%!TEX root = main_hybrid_market.tex
%SourceDoc main_hybrid_market.tex


\vspace{-4mm}

\section{System Model}\label{sec:model}

We consider a database-assisted TV white space network with a \emph{geo-location {\db}} and a set of \emph{unlicensed users} (devices).
%Let $\Kset = \{ 1,\ldots, \K \}$ denote the $\Nset=\{1,...,\N\}$
There exist some unlicensed TV channels (TV white spaces), which can be  used by unlicensed users freely in a shared manner (e.g., using CDMA or CSMA).
%The database is mandatorily required to provide the unlicensed TV channel list (called \emph{basic information}) to any legal user requesting this information\cite{xx}.
Meanwhile, there is a \emph{spectrum licensee}, who owns some licensed channels and wants to lease the under-utilized channels to unlicensed users for additional revenue.\footnote{In case there are multiple spectrum licensees, we assume that they are coordinated by the single representative. We will leave the case of licensees competition to a future work.}
Different from the unlicensed TV white spaces, the licensed TV channels can be used by unlicensed users in an exclusive manner (with the permission of the licensee).
Therefore, users can enjoy a better performance (e.g., a higher data rate or a lower interference) on the licensed channels.
For convenience, let $\pl \geq 0$ denote the (licensed) {channel price} of the spectrum licensee.
%For convenience, we assume all licensed channels are identical, and
%denote $\pl$ as the (licensed) channel price.


% one \lh\footnote{We assume the homogeneous licensed spectrum for analytical simplicity. Hence, we consider all the licensed spectrum holders as a integrated party and called it as a \lh.}, and $\Nset=\{1,...,\N\}$ of unlicensed devices ({\eus}). We denotes $\Kset = \{ 1,\ldots, \K \}$ as the set of available TV channels in this area.
%The {\db} provides two kinds of TV \chs' information service-\emph{basic information service} and \emph{advance information service}-for \eus, while the {\lh} sells/leases licensed spectrum to \eus\footnote{For convenience, we consider the licensed spectrum as licensed \ch}. Each \eu~can choose either to purchase the information of the {\db} and access to \emph{one} of the available TV \chs~at a particular time on the shared basis (i.e., each TV {\ch} is can be used by multiple \eus~simultaneously using CDMA or CSMA techniques), or to buy/lease the licensed \ch for exclusive usage. We assume that the number of licensed spectrum for leasing is sufficient for analytical convenience.



%We consider a online spectrum information platform which lists the available TV \chs~list and the leasing spectrum information. We assume that a {\db} owns this online information platform and the licensed spectrum holders (called \lh) put their licensed spectrum information on this online platform\footnote{According to the regulators' ruling (e.g., FCC \cite{federal2010second}), only the {\db} can house the TV \chs availability information. Hence, only the {\db} can own this online information platform. We can interpret listing licensed spectrum information as the extra service provided by the \db as currently the Spectrum Bridge does. We assume the homogeneous licensed spectrum for analytical simplicity. Hence, we consider all the licensed spectrum holders as a integrated party and called it as a \lh.}.
%In a particular network service area, there are a set $\Nset=\{1,...,\N\}$ of unlicensed devices ({\eus}) access to this online information platform and make the choice between operating on the TV  \chs~and leasing the licensed spectrum.
%Let $\Kset = \{ 1,\ldots, \K \}$ denote the set of available TV channels in this area. Each \eu~can only operate on \emph{one} of the available \chs~at a particular time on the shared basis (i.e., each {\ch} is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques).
%We assume that the number of licensed spectrum for leasing is sufficient and each \eu~can use the leasing spectrum exclusively.

\vspace{-4mm}

\subsection{Geo-location Database}

\subsubsection{Basic Service}
According to the regulation policy (e.g., \cite{federal2012third}), it is mandatory for a geo-location white space {\db} to provide the following information for any unlicensed {\eu}: (i) the list of TV white spaces (i.e., unlicensed TV channels), (ii) the transmission constraint (e.g., maximum transmission power) on each channel in the list, and (iii) other optional requirements.
The database needs to provide this \emph{basic (information) service} free of charge for any unlicensed user.


\subsubsection{Advanced Service}
Beyond the basic information, the {\db} can also provide certain advanced information regarding the quality of TV channels (as SpectrumBridge did in \cite{SpectrumBridgeCommericial}), which we call the \emph{advanced (information) service}, as long as it does not conflict with the free basic service.
Such an advanced information can be rather general, and a typical example is ``the interference level on each channel'' used in \cite{luo2014wiopt, luo2014SDP}.
%Motivated by the practice of SpectrumBridge \cite{SpectrumBridgeCommericial} and the model proposed by Luo \emph{et al.} in \cite{luo2014wiopt, luo2014SDP}, we define the following advanced information:
%%consider such an advanced service, where the {\db} provides the following advanced information to every {\eu} $n$ subscribing to its advanced service (i.e., purchasing the advanced information):
%$$
%\boldsymbol{\InfTot} = \{\InfTot_{\k}\}_{k\in\Kset},
%$$
%where $\InfTot_{\k} $ is the interference level on TV {\ch} $k$ for a particular \eu.\footnote{Note that $\InfTot_{\k} $ may be different for different users. Here, we omit the user index for the writing convenience.}
%When subscribing to the advanced service of a \db,
With the advanced information, the {\eu} is able to choose a channel with the  highest quality (e.g., with the lowest interference level).
Hence, the {\db} can \emph{sell} this advanced information to users for profit.
This leads to an \emph{information market}.
For convenience, let $\pa \geq 0$ denote the (advanced) {information price} of the database.~~~~~~~~~~

\subsubsection{Leasing Service}
As mentioned previously, the geo-location database can also serve as a spectrum market \emph{platform} for the trading of licensed channels between the spectrum licensee and unlicensed users, which we call the \emph{leasing service}.
\rev{
We consider \emph{revenue sharing} scheme (RSS), where the licensee shares a fixed percentage  of  revenue with the database in this paper.
We further denote $\delta \in [0,1]$ as the revenue sharing percentage under RSS.
}
%We consider two different commission charging schemes: (i) \emph{revenue sharing} scheme (RSS), where the licensee shares a fixed percentage  of  revenue with the database, and (ii) \emph{wholesale pricing} scheme (WPS), where the database charges a fixed wholesale price from each successful transaction, regardless of the licensee's revenue from that transaction  (which depends on the licensee's leasing price $\pl$).
%We denote $\delta \in [0,1]$ as the revenue sharing percentage under RSS and $w \geq 0$ as the wholesale price under WPS.

%Figure  \ref{fig:model} illustrates such a  database-provided hybrid spectrum and information market framework.




%We next illustrate the basic and advanced services through an example in the following table (where the advanced information is defined as the interference level on each channel as in \cite{luo2014wiopt, luo2014SDP}).
%In the basic service, the database provides the TV white space list (i.e., \{CH1, CH3, CH4, CH6\}) to each \eu, with which the user may choose a channel randomly.
%In the advanced service, the database provides the TV white space list as well as the interference level on each channel in the list (i.e., \{$\InfTot_1$, $\InfTot_3$, $\InfTot_4$, $\InfTot_6$\}) to the \eu, with which the user can choose the channel with the lowest interference level.
%
%\begin{table}[h]
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\textbf{Channel ID} & \textbf{CH1}& \textbf{CH2}& \textbf{CH3} & \textbf{CH4} & \textbf{CH5} & \textbf{CH6}
%\\
%\hline
%Unlicensed & Yes & $\times$ & Yes & Yes & $\times$ & Yes
%\\
%\hline
%Interference Level & $\InfTot_1$ &  $\InfTot_2$ & $\InfTot_3$ & $\InfTot_4$ &  $\InfTot_5$ & $\InfTot_6$
%\\
%\hline
%\end{tabular}
%\end{table}

%\subsection{Spectrum Licensee}
%The spectrum licensee has the ownership of licensed channels, but may not fully utilize these channels.
%Hence, the {\lh} has an incentive to lease the under-utilized channels to unlicensed users for profit.
%Different from the unlicensed TV white space, licensed TV channels can be used in an exclusive manner (with the permission of the licensee).
%Thus, users can enjoy a better performance (e.g., a higher data rate or a lower interference) on the licensed channels.
%For convenience, we assume all licensed channels are identical, and
%denote $\pl$ as the (licensed) channel price.

%
%The licensee has the ownership of certain licensed TV channels, but these channels may not be fully utilized.
%Hence, the {\lh} has an incentive to lease the under-utilized channels to unlicensed users for profit.
%Different from the unlicensed TV channel, a licensed TV channel can be used by a user exclusively (with the grant of the licensee).
%Hence, users can enjoy a better performance (e.g., higher data rate or lower interference) on the licensed channels.
%For convenience, we assume all licensed channels are identical, and
% denote $\pl$ as the price of each channel.
%
%From the implementing perspective, however, it is difficult for the licensee to lease its channels to unlicensed users in an online and automatic manner, due to the lack of reliable and secure platforms to support this trading process.
%The white space database emerges as a promising candidate of such a spectrum trading platform.
%First, a legal white space databases must be certified by spectrum regulators, hence the security can (at least partly) be guaranteed.
%Second, a white space database can easily interact with both the licensees and the unlicensed users, hence it can potentially serve as an agent between the licensees and the unlicensed users.
%For these reasons, some real database operators have started to provide such a spectrum market platform, e.g., the SpecEx \cite{SpectrumBridgeCommericial2} provided by the database operator SpectrumBridge.

\vspace{-3mm}
\subsection{Unlicensed User}

Unlicensed users can choose either to purchase the licensed channel from the licensee for the exclusive usage, or to share the free unlicensed TV white spaces with others (with and without advanced information).
We assume that all licensed and unlicensed TV channels have the same bandwidth (e.g., 6MHz in the USA), and each user only needs one channel (either licensed or unlicensed) at a particular time.
Formally, we denote $\l \in \{\B, \A, \LS\}$ as the  \emph{strategy} of a user, where
%Each user can choose either to purchase the licensed channel from the spectrum licensee for the exclusive usage, or to request the free unlicensed channels from the database for the shared usage.
%We assume that one user requests one channel (either licensed or unlicensed).
%Let $\l$ denote the strategy of a unlicensed user.
%Then, each user {\eu} has the following 3 choices:
% in terms of channel selection under different services.
%After obtaining the available channel list through the free basic service, each {\eu} has 3 choices (denoted by $\l$) in terms of channel selection:
\begin{itemize}
\item[(i)] $\l = \B$:
Choose the basic service (i.e., share TV white spaces with others, without the advanced information);
%Hence, the user randomly chooses a unlicensed {\tvch} in the available channel list;
\item[(ii)] $\l = \A$:
Choose the advanced service (i.e., share TV white spaces with others, with the advanced information).
%Hence, the user picks the best {\ch} in the available channel list (e.g.,  with the lowest interference);
\item[(iii)] $\l = \LS$:
Choose the leasing service (i.e., lease the licensed channel from the licensee for the exclusive usage).
% in the available channel list.
%\footnotesc{We do not consider the sensing capability of users, which has been removed in the FCC ruling \cite{federal2010second}.}
\end{itemize}
We further denote $\RB$, $\RA$, and $\RL$ as the expected \emph{utility} that a user can achieve from choosing the basic service ($\l = \B$), the advanced service ($\l = \A$), and the leasing service ($\l = \LS$), respectively.
The \emph{payoff} of a {\eu} is defined as the difference between the achieved utility and the service cost (i.e., the  {information price} when choosing the advanced service, or the  {leasing price} if choosing the leasing service).
\rev{
Let $\th$ denote the \eu's evaluation for the achieved utility.
}
Then, the payoff of a user with an evaluation factor $\th$ can be written as 
\begin{equation}\label{eq:utility-basic}
\textstyle
\Ueu_{\th} = \left\{
  \begin{aligned}
  &\textstyle  \th \cdot \RB ,      &&  \ \text{if} ~ \l = \B, \\
  &\textstyle  \th \cdot \RA   -  \pa , &&  \  \text{if} ~ \l  = \A, \\
  &\textstyle  \th \cdot \RL - \pl ,      &&  \ \text{if} ~ \l = \LS.
   \end{aligned}
\right.
\end{equation}
%$\Rl$ is the expected data rate when the {\eu} chooses a strategy $\l\in \{ 0,1,2\}$, $\ut(\cdot)$ is the utility function (concave and increasing) of the \eu, and
Each user is rational and will choose a strategy $\l \in \{\B, \A, \LS\}$ that maximizes its payoff.
Note that different {\eus} may have different values of $\th$ (e.g., depending on application types), hence have different choices. That is, {\eus} are heterogeneous in term of $\th$.
For convenience, we assume that $\th$ is uniformly distributed in $[0,1]$ for all \eus\footnote{{This assumption is commonly used in the existing literature. Relaxing to more general distributions often does not change the main insights \cite{manshaei2008evolution,shetty2010congestion}.}}.

%Before we solve the three-stage model discussed in the previous section with backwards induction. We first need to characterize the utility provided by different service so that we can analyze the subscription choice of {\eus}. Hence, in the next section, we will analyze the value of information to {\eus}.

%\textbf{Problem Formulation}
%Based on this three-stage model we discussed in the previous section, we are interested in the following problems: i) what is the optimal bargaining solution between the {\db} and the \lh? ii) What is the Nash equilibrium of the pricing decisions game? iii) How these market share of the {\db} $\Proba$ and the {\lh} $\Probl$ dynamically evolve and what is the market equilibrium? Note that in order to answer these problems, we first need to characterize the utility provided by different service. Hence, in the next section, we will analyze the value of information to {\eus}.

Let $\Probb$, $\Proba$, and $\Probl$ denote the fraction of {\eus} choosing the basic service, the advanced service, and the leasing service, respectively.
For convenience, we refer to $\Probb$, $\Proba$, and $\Probl$ as the \emph{market shares} of the basic service, the advanced service, and the leasing service, respectively.
Obviously, $\Probb, \Proba, \Probl \geq 0$ and $\Probb + \Proba + \Probl = 1$.
Then, the {normalized} \emph{payoffs} (profits) of the spectrum licensee and the geo-location database are, respectively,
\begin{equation}\label{eq:u1}
\left\{
\begin{aligned}
\Usl \eq \Uslrs &= \pl   \Probl   (1 - \delta),
\\
\Udb \eq \Udbrs &= \pa   \Proba + \pl   \Probl   \delta,
\end{aligned}
\right.
\end{equation}
under the revenue sharing scheme.
% (Scheme I), and
%\begin{equation}\label{eq:u2}
%\left\{
%\begin{aligned}
%\Usl \eq \Uslwp &= (\pl -\w)  \Probl ,
%\\
% \Udb \eq \Udbwp &= \pa \Proba + \w   \Probl ,
%\end{aligned}
%\right.
%\end{equation}
%under the wholesale pricing scheme (Scheme II).
%\com{What is the impact of user population size N?
%If we are not using N, we should call the payoff "normalized".
%Actually, are we using "N" in the paper at all? }
%\com{Yuan: Since we only use N in the simulation part, I change it to the normalized payoff and I also change the simulation figures accordingly.}

\vspace{-2mm}
\subsection{Positive and Negative Network Externalities}
There are two types of network externalities coexisting in the information market: (i) \emph{negative network externality}, which corresponds to the increasing level of congestion and degradation of user performance due to more users sharing the same TV white space, and (ii) \emph{positive network externality}, which is due to the quality increase of the (advanced) information as more users purchasing the information.
Next we analytically quantify these two network externalities.

We first have the following observations for a user's expected utilities of three strategy choices:
\begin{itemize}
\item
\emph{$\RL$ is a constant independent of $\Proba $, $\Probb$, and $ \Probl $.}
This is because the licensed channels are used in an exclusive manner, hence the performance of a user on such a channel does not depend on the choices of others.
\item
\emph{$\RB$ is non-increasing in $\Proba + \Probb$} (the total fraction of users using TV white space) due to the congestion effect.
This is because the unlicensed TV white space must be used in a shared manner, hence more users using these channels increases the level of congestion and reduces the performance of each user.~~~~~~~
 \item
\emph{$\RA$ is non-increasing in $\Proba + \Probb$, due to the congestion effect} similar as $\RB$.
This is the \textbf{negative network externality}.
 \item
\emph{$\RA$ is non-decreasing in $\Proba$, given a fixed value of $\Proba + \Probb $}.
This is because more users purchasing the advanced information increases the quality of the information.
This is  the \textbf{positive network externality}.~~~~~~~~~~~~~~~~
% and meanwhile non-decreasing with the fraction of users purchasing the advanced information, i.e., $\Proba$, given the $(\Proba + \Probb)$, due to the positive network externality of the information market.
\end{itemize}
For convenience, we write $\RB$ as a non-increasing function of  $ \Proba + \Probb $, i.e.,\footnote{Later we will also write $\Proba + \Probb $ as $1- \Probl$, since $\Proba + \Probb  + \Probl  = 1$.}
$$
\textstyle
\RB \triangleq \fx(\Proba + \Probb),
$$
and write $\RA$ as the combination of a
non-increasing function of $ \Proba + \Probb $ and a non-decreasing function of $\Proba $, i.e.,
$$
\RA \triangleq \fx(\Proba + \Probb) + \gy(\Proba) ,
$$
%where $\fx(\cdot)$ is a non-increasing function, and $\gy(\cdot)$ is a non-decreasing function.
Note that function $\fx (\cdot)$ reflects the congestion effect, and is identical for $\RB $ and  $\RA$ (as users experience the same congestion effect in both basic and advanced services).
Function $\gy(\cdot)$ in $\RA$ reflects the performance gain induced by the advanced information, i.e., the (advanced) information value.

Since there is no congestion on the licensed channels, it is reasonable to assume that $\RL$ is always larger than $\RA $ and $\RB $.
We can further assume that $\RA$ is larger than $\RB$ due to additional advanced information\footnote{{Note that if we set $\RL < \RB$, then users will never choose the leasing service even with a zero channel price $\pl$.
In this case, our model degenerates to the pure information market, similar as that in \cite{luo2014wiopt}.
Moreover, if we set $\RA = \RB$, then users will never choose the advanced service even with a zero information price $\pa$.
In this case, our model degenerates to a monopoly spectrum market (where the licensee is the monopolist).
In this sense, our hybrid market model generalizes both the pure spectrum market and pure information market.}}.
To facilitate the later analysis, we further introduce the following assumptions on functions $\fx (\cdot)$ and $\gy (\cdot)$.
\vspace{-1mm}
\begin{assumption}\label{assum:congestion}
Function $\fx(\cdot)$ is non-negative, non-increasing, convex, and continuously differentiable.
\end{assumption}
\vspace{-4mm}
\begin{assumption}\label{assum:positive}
Function $\gy(\cdot)$ is non-negative, non-decreasing, concave, and continuously differentiable.
\end{assumption}
\vspace{-2mm}
\rev{
The non-increasing and convexity assumption of $\fx(\cdot)$ is due to the increasing of marginal performance degradation under congestion, and is widely used to model the network congestion effect in wireless networks (see, e.g., \cite{shetty2010congestion,johari2010congestion} and references therein).
The non-decreasing and concavity assumption of $\gy(\cdot)$ results form the diminishing of marginal performance improvement induced by the advanced information.
Note that the above generic functions $\fx(\cdot)$ and $\gy(\cdot)$ can be used to generalize a lot of scenarios with the explicit advanced information definition, e.g., those proposed by Luo \emph{et al.} in \cite{luo2014wiopt, luo2014SDP} (where the advanced information is the interference level on each channel). We provide the detailed discussion in the Appendix.
}

\begin{figure}[t]
\centering
\footnotesize
\begin{tabular}{|m{3in}|}
\hline
\textbf{\revh{Layer I}: Commission Negotiation}
\\
\hline
The database and the spectrum licensee negotiate the commission charge details (i.e.,
$\delta $ under RSS).
\\
\hline
\multicolumn{1}{c}{$\Downarrow$} \\
\hline
\textbf{\revh{Layer II}: Price Competition Game}
\\
\hline
The database determines the information price $\pa$;
\\
The spectrum licensee determines the channel price $\pl$.
\\
\hline
\multicolumn{1}{c}{$\Downarrow$} \\
\hline
\textbf{\revh{Layer III}: User Behaving and Market Dynamics}
\\
\hline
The unlicensed users determine and update their best choices;
\\
The market dynamically evolves to the equilibrium point.
\\
\hline
\end{tabular}
\caption{Three-layer Interaction Model}
\label{fig:layer}
\vspace{-4mm}
\end{figure}


\vspace{-3mm}
\subsection{Three-Layer Interaction Model}

%
%Our focus in this work is to make a thorough and comprehensive understanding of the  behaviour and equilibrium in such a database-provided hybrid spectrum and information market, so as to offer meaningful insights to a real TV white space network system.
%To this end, we formulate the interactions among the geo-location database (operator), the spectrum licensee, and unlicensed users as a three-layer hierarchical model illustrated in Figure \ref{fig:problem}.
%Specifically,

Based on the above discussion, a hybrid spectrum and information market involves the interactions among the geo-location database, the spectrum licensee, and the unlicensed users.
Hence, we formulate the interactions as a three-layer hierarchical model illustrated in Figure \ref{fig:layer}.
%To make a thorough and comprehensive understanding of the behaviour and equilibrium in such a market, we formulate the interactions as a three-layer hierarchical model illustrated in Figure \ref{fig:layer}.

Specifically, in Layer I, the database and the spectrum  licensee negotiate the commission charge details (regarding the spectrum market platform), i.e., the revenue sharing factor $\delta $ under RSS, or the wholesale price $\w$ under WPS.
In Layer II, the database and the spectrum licensee compete with each other to attract unlicensed users. The database determines the price $\pa$ of the advanced information, and the spectrum licensee determines the price $\pl$ of the licensed channel.
In Layer III, the unlicensed users determine their best choices, and dynamically update their choices based on the current market shares. Accordingly, the market dynamically involves and finally reaches the equilibrium point.


In the following sections, we will analyze this three-layer interaction model systematically using backward induction.





%\subsection{Market Platform}

%We propose a database-provided hybrid market framework shown in Figure  \ref{fig:model}, wherre the database operator provides (i) a \emph{spectrum market} platform for the trading of (licensed) TV channels between the TV licensee and unlicensed users, and (ii) an \emph{information market} platform for the trading of information (regarding the unlicensed TV channels) between the database itself and unlicensed users.
%In this example, users 1 and 2 lease the licensed channels from the TV licensee via the database-provided spectrum market, while users 3 and 4 use the shared unlicensed channels, and moreover, user 4 purchases the advanced information from the database vis the information market.
%
%By offering the spectrum market platform for the licensee, the database operator also takes certain \emph{commission charge} from each successful transaction between TV licensees and unlicensed users.
%We consider two different commission schemes in this work: (i) \emph{revenue sharing} scheme  (RSS), where the TV licensee shares a fixed portion of  revenue with the database operator, and (ii) \emph{wholesale pricing} scheme (WPS), where the database operator charges a fixed money from each successful transaction, regardless the detailed revenue that the TV licensee achieves from that transaction.
%
%
%Based on the above, we formulate the interactions among the database operator, the TV licensee, and unlicensed users as a three-layer hierarchical model.
%In the first layer, the database operator and the TV licensee negotiate the commission charge details regarding  the spectrum market platform.
%In the second layer, the database operator and the TV licensee make the pricing decisions.
%In the third layer, unlicensed users make the purchasing decision.
%

%Because the {\lh} has difficulty in identifying the potential buyers and the {\eus} who enquire the {\db} for accessing to the {\tvch} usually are unlicensed device, it is a good way for the {\lh} to lease its \lch~via the \db. Hence, the {\lh} pays the displaying fee to the {\db} so that the {\db} can provide each {\eu} with the \lch~information freely. If a {\eu} want to lease the \lch, this {\eu} has to pay the leasing price $\pl$ to {\lh} in order to enjoy the exclusively usage.


%Because a {\eu} has to share the TV {\ch} with other {\eus} who operate on the same \ch, the quality of TV {\ch} degrades with the number of {\eus} operating on the same TV \ch. Hence, the {\db} will to display some licensed spectrum information for {\eus} to lease in order to alleviate the congestion of the TV \chs. As Spectrum Bridge does \cite{SpectrumBridgeCommericial2}, each {\eu} can obtain the licensed spectrum information from the \db freely. However, it has to pay the leasing price $\pl$ to {\lh} in order to enjoy the exclusively usage. The {\db} will charge certain fee from the \lhs~for displaying the licensed information. The \lhs, on the other hand, are willing to pay the displaying fee as long as joining the online information platform can make revenue.

%\subsection{Market Property}
%
%The licensed channels are used by users in an exclusive manner, hence one user in the spectrum market (i.e., using the licensed channel) does not affect the performance of other users in the spectrum market.
%The unlicensed channels, however, are used by users in a shared manner. Hence, the more users using the unlicensed channels, the higher potential congestion among these users.
%This implies that the information market has the property of \emph{negative network externality}.
%On the other hand, similar as in \cite{luo2014wiopt, luo2014SDP}, more users purchasing the advanced information will improve the value of the information, hence benefit all users in the information market.
%That is, the information market also has the property of \emph{positive network externality}.
%
%Next we characterize these positive and negative network effects explicitly.
%Let $\Probb$ denote the fraction of {\eus} choosing the basic service (i.e.,   using the unlicensed channels without advanced information),  $\Proba$ denote the fraction of users choosing the advanced service (i.e.,   using the unlicensed channels with advanced information), and $\Probl$ denote the fraction of users leasing the licensed channels from the licensee.
%Obviously, $\Probb, \Proba, \Probl \geq 0$ and $\Probb + \Proba + \Probl = 1$\footnote{Because the basic service is provided for free, all {\eus} can obtain at least a non-negative profit by choosing the basic service.
%Hence, all \eus~must choose one of these three services.}.
%%For writing  convenience, we will use $( 1 - \Proba - \Probl) $ to represent $\Probb$.
%% Let $\RB$ denote the expected utility that an user can obtain from the basic service (i.e., using a unlicensed channel without advanced information), $\RA$ denote the expected utility that an user can obtain from the advanced service (i.e., using a unlicensed channel with advanced information), and $\RL$ denote the expected utility that an user can obtain from using a licensed channel. Then, we can easily find that:
%
%\rev{We further define the expected utility that an user can obtain from choosing different services as follows.
%\begin{itemize}
%\item
%$\RB$ is the expected utility that an user can obtain from the basic service (i.e., using a unlicensed channel without advanced information);
%\item
%$\RA$ is the expected utility that an user can obtain from the advanced service (i.e., using a unlicensed channel with advanced information);
% \item
%$\RL$ is the expected utility that an user can obtain from using a licensed channel.
%\end{itemize}
%}
%%Let $\RB$ denote the expected utility that an user can obtain from the basic service (i.e., using a unlicensed channel without advanced information), $\RA$ denote the expected utility that an user can obtain from the advanced service (i.e., using a unlicensed channel with advanced information), and $\RL$ denote the expected utility that an user can obtain from using a licensed channel.
%Then, we can easily find that:
%\begin{itemize}
%\item
%$\RL$ is constant and independent of $\Proba $, $\Probb$, and $ \Probl $;
%\item
% $\RB$ is non-increasing with the total fraction of users using the unlicensed channels, i.e., $(\Proba + \Probb)$, due to the congestion effect;
% \item
% $\RA$ is non-increasing with  the total fraction of users using the unlicensed channels, i.e., $(\Proba + \Probb)$, due to the congestion effect; and meanwhile non-decreasing with the fraction of users purchasing the advanced information, i.e., $\Proba$, given the $(\Proba + \Probb)$, due to the positive network externality of the information market.
%\end{itemize}
%For convenience, we will write $\RB$ as a function of  $(\Proba + \Probb)$:
%$$
%\RB \triangleq \fx(\Proba + \Probb),
%$$
%and $\RA$ as a function of  $(\Proba + \Probb)$ and $\Proba $:
%$$
%\RA \triangleq \fx(\Proba + \Probb) + \gy(\Proba) ,
%$$
%where $\fx(\cdot)$ is a non-increasing function, and $\gy(\cdot)$ is a non-decreasing function. Note that we can also write $\Proba + \Probb $ as $1- \Probl$.
%To facilitate the later analysis, we further introduce the following assumptions on these functions.
%
%\begin{assumption}\label{assum:congestion}
%The function $\fx(\cdot)$ is non-negative, non-increasing, convex, and continuously differentiable.
%\end{assumption}
%
%\begin{assumption}\label{assum:positive}
%The function $\gy(\cdot)$ is non-negative, non-decreasing, concave, and continuously differentiable.
%\end{assumption}
%
%\rev{
%The non-increasing and convexity assumption of $\fx(\cdot)$ is due to the increasing of marginal performance degradation under congestion, and is widely used to model the network congestion effect in wireless networks (see, e.g., \cite{shetty2010congestion,acemoglu2010congestion,johari2010congestion} and references therein).
%The non-decreasing and concavity assumption of $\gy(\cdot)$ results form the diminishing of marginal performance improvement induced by the advanced information.
%}
%Note that the above generic functions $\fx(\cdot)$ and $\gy(\cdot)$ can be used to generalize a lot of scenarios with the explicit advanced information definition, including that in \cite{luo2014wiopt, luo2014SDP} (where the advanced information is the interference level on each TV channel). Due to space limit, we leave the detailed discussion in \cite{report}.

%\com{Lin: We use the general functions to denote the positive and negative effects, rather than using the detailed functions derived by the interference. The reasons are follows. First, to make this work more different from our previous work; Second, to better present our model (the interference model is a bit complicated); Third, to generalize other models. }
%
%
%\com{Lin: We are still polishing the following Sections, and will finish in one or two days. The structure of the following content follows the backward induction. Namely, we will solve the three layers one by one in a backward sequence.}

%returns to increased the number of {\eus} subscribing to the advanced service.
%This is because in sharing the TV white space network, when the number of {\eus} is small, then each additional \eu~makes the network significantly more useful; but an additional \eu~may go unnoticed when added to a TV white space network.

%Because function $\fx$ and $\gy$ can characterize the information value to the {\eus}, we begin to solve the three-stage model discussed in the previous section with backwards induction.


%As mentioned previously,
%, while $\RB$ and $\RA$ are functions of $\RB$ and $\RA$, hence can be rewritten as $\RB(\Proba, \Probl)$ and $\RA(\Proba, \Probl)$, respectively.
%More details about $\RB(\Proba, \Probl)$ and $\RA(\Proba, \Probl)$ will be discussed in the next section.

%We also denote $\RB$, $\RA$, and $\RL$ as the expected utility provided by the basic service, the advanced service, and the leasing service, respectively. Because {\eus} can use the leasing spectrum exclusively, we assume that $\RL$ is a constant for simplicity. Note that the quality of TV \chs~depends on the number of {\eus} who operator on the TV \chs. Hence, $\RB$ and $\RA$ are the function of $\Proba$ and $\Probl$ and are rewritten as $\RB(\Proba, \Probl)$ and $\RA(\Proba, \Probl)$, respectively.
%We will study the characteristic of $\RB(\Proba, \Probl)$ and $\RA(\Proba, \Probl)$ detailedly in the next section.


%the Also, let $\RB = \fx(\Probb + \Proba)$ and $\RA = \fx(\Probb + \Proba) + \gy(\Proba)$ be the expected utility provided by the basic service and the advanced service, respectively, where  Because TV \chs~are shared basic spectrum, the quality of TV \chs~
%
%
%Intuitively, we have $\RA > \RB$ because the {\eu} can operate on the best available channel.

%\begin{table}[t]
%\centering
%\caption{Key Notations in This Paper}
%\label{table:key-notations}
%\footnotesize
%\begin{tabular}{|c|p{6.8cm}|}
%\hline
%$\N$ & The number of \eus
%\\
%\hline
%$\K$ & The number of available \tvch
%\\
%\hline
%$\pa$ & The \db's subscription fee
%\\
%\hline
%$\pl$ & The \lh's leasing fee
%\\
%\hline
%$\Proba$ & The fraction of {\eus} choosing the advanced service
%\\
%\hline
%$\Probl$ & The fraction of {\eus} choosing the leasing service
%\\
%\hline
%$\RB(\Proba, \Probl)$ & The expected utility provided by the basic service
%\\
%\hline
%$\RA(\Proba, \Probl)$ & The expected utility provided by the advanced service
%\\
%\hline
%$\RL$ & The expected utility provided by the leasing service
%\\
%\hline
%\centering $\l$ & The service choice of {\eu}, $\l = \B$: the basic service; $\l = \A$: the advanced service; and $\l = \LS$: the leasing service
%\\
%\hline
%\centering $\th$ & the \eu's evaluation for the achieved utility provided by the three kinds of service
%\\
%\hline
%\end{tabular}
%\end{table}

%\subsection{user}


==> Latex_ParticipateSensing_infocom_camera/Section_Model_new.tex <==
%!TEX root = main_inform_compe.tex
%SourceDoc main_inform_compe.tex

\section{System Model}\label{sec:model}
\subsection{TV White Space Information Market}
In this section, we first consider a monopoly TV white space network, where a set $\Nset=\{1,...,\N\}$ of unlicensed white space devices ({\eus}) can only operating on idle TV channels requested from a white space database.
Let $\Kset = \{ 1,\ldots, \K \}$ denote the set of available TV channels in the area of the network.
Each \eu~queries a database for the available TV channel set, and  can only operate on \emph{one} of the available \chs~at a particular time.

According to the regulator's ruling (e.g., FCC \cite{federal2010second}), a certified white space {\db} provides the following information for {\eus}: (i) the list of available TV channels, (ii) the transmission constraints (e.g., maximum transmission power) on each available channel, and (iii) some other optional requirements.
This is the basic information (\emph{basic service}) that every {\db} is mandatory to provide for any {\eu} free of charge.

Beyond the basic service, the white space {\db} can also provide certain advanced information (\emph{advanced service}) to make a profit, under the constraint that it does not conflict with the basic service.
Motivated by the practice of Spectrum Bridge \cite{SpectrumBridgeCommericial}, we consider such an advanced service, where each {\db} provides the following advanced information to every WSD $n$ subscribing to its advanced service\footnotesc{{``Subscribe to a \db'' means that the \eu purchases the advanced information from the \db.}}:
$\{\InfTot_{\k}\}_{k\in\Kset}$ (i.e., the interference level on every available channel for this particular \eu).
%When subscribing to the advanced service of a \db,
With this advanced information,
the {\eu} is able to operate on the best available channel (with the lowest interference level).
Accordingly, the {\db} can charge a \emph{subscription fee} (denoted by $\pa$) to every {\eu} subscribing to its advanced service.
This essentially constitutes an \emph{information market}.~~~~~~~~

For convenience, we illustrate the basic service and advanced service by the example in the following table.
In the basic service, the database provides the available channel set (i.e., \{CH1, CH3, CH4, CH6\}) to a particular \eu. In the advanced service, the database provides the interference levels on available channels (i.e., \{$\InfTot_1$, $\InfTot_3$, $\InfTot_4$, $\InfTot_6$\}) to the \eu, in addition to the available channel set.

\begin{table}[h]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Channel ID} & \textbf{CH1}& \textbf{CH2}& \textbf{CH3} & \textbf{CH4} & \textbf{CH5} & \textbf{CH6}
\\
\hline
Availability & Yes & No & Yes & Yes & No & Yes
\\
\hline
Interference Level & $\InfTot_1$ &  - & $\InfTot_3$ & $\InfTot_4$ &  - & $\InfTot_6$
\\
\hline
\end{tabular}
\end{table}


%======================
Assume that \eus are heterogeneous in the valuation of the achieved utility by choosing different services. We denote the \eu's valuation for the achieved utility by $\th$, and for analytic simplicity, assume that is it uniformly distributed in $[0,1]$.


After obtaining the available channel list through the free basic service, each {\eu} has 2 choices (denoted by $\l$) in terms of channel selection:
\begin{itemize}
\item[(i)] $\l = \A$: subscribing to the \db's advanced service, and picking the channel with the lowest interference indicated by the \db;
\item[(ii)] $\l = \B$: choosing an available channel randomly;
\end{itemize}
The \emph{payoff} of {\eu} equals (i) the benefit (\emph{utility}) from the achieved data rate on the selected channel minus (ii) the \emph{subscription fee} if subscribing to  an advanced service.
Formally, the payoff of {\eu} can be defined as:~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\begin{equation}\label{eq:utility-basic}
\Ueu  = \left\{
  \begin{aligned}
  &\textstyle  \th \cdot \ut(\R_l)  -  \p_l , &&  \  \text{if} ~ \l \in\{1,2\}, \\
%  &\textstyle  \th \cdot \ut(\Rkab)  -  \p_2 , &&  \quad  \text{if} ~ \l = \A_2, \\
  &\textstyle  \th \cdot \ut(\R_0) ,      &&  \ \text{if} ~ \l = 0,
%  \\
%  &\textstyle  \th \cdot \ut(\Rkgb) ,      &&  \quad  \text{if} ~ \l = \G_2, \\
   \end{aligned}
\right.
\end{equation}
where $\Rl$ is the expected data rate when the {\eu} chooses a strategy $\l\in \{ 0,1,2\}$, $\ut(\cdot)$ is the utility function (concave and increasing) of the \eu, and $\th$ is the \eu's evaluation for the achieved utility.
Note that different {\eus} may have the different utility evaluation factor $\th$ (e.g., for different applications), that is, {\eus} are heterogeneous in term of $\th$.
For the analytical convenience, we assume that $\th$ is uniformly distributed in $[0,1]$ for all \eus.
%We consider heterogeneous \eus, where different {\eus} value the same data transmission rate or utility differently (due to different wireless applications).
%, and $\kl$, $\l \in \{ \G, \S, \A \}$ is the \ch~index chosen by the type-$\th$ \eu~based on the \ch~state information provided by different service scheme.
%$\Ra$, $\Rs$, and $\Rr$ is expected data rate corresponding to different \eu's choice.
%Note that in our model, the \db~is not allowed to engage in either QoS discrimination nor price discrimination.
%Here assume that all \eus~are charged by the same price $\p_i$ if $\l=\A_i$.
%In other words, the \db~is not allowed to engage in price discrimination for the simplicity of practical implementation.




%We consider a online spectrum information platform which lists the available TV \chs~list and the leasing spectrum information. We assume that a \db~owns this online information platform and the licensed spectrum holders (called \lh) put their licensed spectrum information on this online platform \footnote{According to the regulators' ruling (e.g., FCC \cite{federal2010second}), only the \db~can house the TV \chs availability information. Hence, only the \db~can own this online information platform. We can interpret listing licensed spectrum information as the extra service provided by the \db as currently the Spectrum Bridge does.}.
%In a particular network service area, there are a set $\Nset=\{1,...,\N\}$ of unlicensed white space devices ({\eus}) access to this online information platform and make the choice between operating on the TV  \chs~and leasing the licensed spectrum.
%Let $\Kset = \{ 1,\ldots, \K \}$ denote the set of available TV channels in this area. Each \eu~can only operate on \emph{one} of the available \chs~at a particular time on the shared basis (i.e., each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques).
%We assume that the number of licensed spectrum for leasing is sufficient and each \eu~can use the leasing spectrum exclusively.
%
%\textbf{White Space Database.}
%According to the regulator's ruling (e.g., FCC \cite{federal2010second}), a certified white space {\db} provides the following information for {\eus}: (i) the list of available TV channels, (ii) the transmission constraints (e.g., maximum transmission power) on each available channel, and (iii) some other optional requirements.
%This is the basic information (\emph{basic service}) that every {\db} is mandatory to provide for any {\eu} free of charge.
%
%Beyond the basic service, the white space {\db} can also provide certain advanced information (\emph{advanced service}) to make a profit, under the constraint that it does not conflict with the basic service.
%Motivated by the practice of Spectrum Bridge \cite{SpectrumBridgeCommericial}, we consider such an advanced service, where each {\db} provides the following advanced information to every WSD $n$ subscribing to its advanced service\footnotesc{{``Subscribe to a \db'' means that the \eu purchases the advanced information from the \db.}}:
%$\{\InfTot_{\k}\}_{k\in\Kset}$ (i.e., the interference level on every available channel for this particular \eu).
%%When subscribing to the advanced service of a \db,
%With this advanced information,
%the {\eu} is able to operate on the best available channel (with the lowest interference level).
%Accordingly, each {\db} $\dbb_i $ can charge a \emph{subscription fee} (denoted by $\p_i$) to every {\eu} subscribing to its advanced service.
%%Notice that providing such interference information is not enforced by the regulator, and it is based on the bilateral agreement between a {\eu} and a database.
%%For example, each database can choose whether to offer this advanced service and at what price, and each {\eu} can choose whether and from which database it is going to subscribe to this service.
%This essentially constitutes an \emph{information market}.~~~~~~~~
%
%For convenience, we illustrate the basic service and advanced service by the example in the following table.
%In the basic service, the database provides the available channel set (i.e., \{CH1, CH3, CH4, CH6\}) to a particular \eu. In the advanced service, the database provides the interference levels on available channels (i.e., \{$\InfTot_1$, $\InfTot_3$, $\InfTot_4$, $\InfTot_6$\}) to the \eu, in addition to the available channel set.
%
%\begin{table}[h]
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\textbf{Channel ID} & \textbf{CH1}& \textbf{CH2}& \textbf{CH3} & \textbf{CH4} & \textbf{CH5} & \textbf{CH6}
%\\
%\hline
%Availability & Yes & No & Yes & Yes & No & Yes
%\\
%\hline
%Interference Level & $\InfTot_1$ &  - & $\InfTot_3$ & $\InfTot_4$ &  - & $\InfTot_6$
%\\
%\hline
%\end{tabular}
%\end{table}

%
%\textbf{White Space Devices ({\eus}).}
After obtaining the available channel list through the free basic service, each {\eu} has 3 choices (denoted by $\l$) in terms of channel selection:
\begin{itemize}
\item[(i)] $\l \in\{1,2\}$: subscribing to the database $\dbb_l$'s advanced service, and picking the channel with the lowest interference indicated by database $\dbb_l$;
\item[(ii)] $\l = 0$: choosing an available channel randomly;
% in the available channel list.
%\footnotesc{We do not consider the sensing capability of WSDs, which has been removed in the FCC ruling \cite{federal2010second}.}
\end{itemize}
The \emph{payoff} of {\eu} equals (i) the benefit (\emph{utility}) from the achieved data rate on the selected channel minus (ii) the \emph{subscription fee} if subscribing to  an advanced service.
%We assume that each {\eu} is rational, and will always choose the strategy that maximizes its payoff.
Formally, the payoff of {\eu} can be defined as:~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%We assume the \eus~valuation of expected data rate follows a probability distribution. For analysis tractability, we assume that $\th$ is uniformly distributed in $[0,1]$.
%We use $\a_{\n}$ denote the service scheme selected by \eu~$\n$. $\a_{\n} = 0$ represents the subscription scheme, $\a_{\n} = 1$ represents the sensing scheme, and $\a_{\n}=2$ is the random choosing scheme.
%Let us denote an \eu's choice as $\l$, with $\l = \A_1$ denoting subscribing to the $\dbb_1$'s advanced service, $\l = \A_2$ denoting subscribing to the $\dbb_2$'s advanced service, $\l = \G_1$
%denoting  randomly selecting a channel (under the $\dbb_1$'s basic service), and $\l = \G_2$
%denoting  randomly selecting a channel (under the $\dbb_2$'s basic service).
%Formally, the payoff of a type-$\th$ \eu~is:
\begin{equation}\label{eq:utility-basic}
\Ueu  = \left\{
  \begin{aligned}
  &\textstyle  \th \cdot \ut(\R_l)  -  \p_l , &&  \  \text{if} ~ \l \in\{1,2\}, \\
%  &\textstyle  \th \cdot \ut(\Rkab)  -  \p_2 , &&  \quad  \text{if} ~ \l = \A_2, \\
  &\textstyle  \th \cdot \ut(\R_0) ,      &&  \ \text{if} ~ \l = 0,
%  \\
%  &\textstyle  \th \cdot \ut(\Rkgb) ,      &&  \quad  \text{if} ~ \l = \G_2, \\
   \end{aligned}
\right.
\end{equation}
where $\Rl$ is the expected data rate when the {\eu} chooses a strategy $\l\in \{ 0,1,2\}$, $\ut(\cdot)$ is the utility function (concave and increasing) of the \eu, and $\th$ is the \eu's evaluation for the achieved utility.
Note that different {\eus} may have the different utility evaluation factor $\th$ (e.g., for different applications), that is, {\eus} are heterogeneous in term of $\th$.
For the analytical convenience, we assume that $\th$ is uniformly distributed in $[0,1]$ for all \eus.
%We consider heterogeneous \eus, where different {\eus} value the same data transmission rate or utility differently (due to different wireless applications).
%, and $\kl$, $\l \in \{ \G, \S, \A \}$ is the \ch~index chosen by the type-$\th$ \eu~based on the \ch~state information provided by different service scheme.
%$\Ra$, $\Rs$, and $\Rr$ is expected data rate corresponding to different \eu's choice.
%Note that in our model, the \db~is not allowed to engage in either QoS discrimination nor price discrimination.
%Here assume that all \eus~are charged by the same price $\p_i$ if $\l=\A_i$.
%In other words, the \db~is not allowed to engage in price discrimination for the simplicity of practical implementation.

Next we compute the \eu's expected data rate $\Rl$ under different strategies $\l\in\{0,1,2\}$.
Specifically, when $\l=0$ (choosing channel randomly), the {\eu}'s expected
data rate~is
\begin{equation}\label{eq:rkgs}
\begin{aligned}
& \R_0  \textstyle = \Ex_{Z} [\rt(\InfTot)] = \int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z),
%\\
%& \Rkaa = \Rkab \textstyle = \Ex_{Z_{(1)}} [\rt(Z_{(1)})] = \int_{Z} \rt(z) \mathrm{d} F_{Z_{(1)}}(z),
%\\
%& \Rkaa = \Rkab \textstyle = \Ex_{Z^{1}_{(1)}} [\rt(Z^{1}_{(1)})] = \int_{Z} \rt(z) \mathrm{d} F_{Z^{1}_{(1)}}(z),
%\\
%& \Rkab \textstyle = \Ex_{Z^{2}_{(1)}} [\rt(Z^{2}_{(1)})] = \int_{Z} \rt(z) \mathrm{d} F_{Z^{2}_{(1)}}(z),
\end{aligned}
\end{equation}
where $\rt(\cdot)$ is the transmission rate function (e.g.,
the Shannon capacity) under any given interference.
%$Z_{(1)} \triangleq \min\{Z_1,Z_2,...,Z_K\}$ is the minimum interference on all channels, and $\rt(\cdot)$ is a function that maps \ch~$\k$'s interference level $\InfTot_{\k}$ to the data rate.
%Notice the above formula assumes that the database knows precisely the state of every channel, and thus the \eus~subscribing to any \db's advanced service can always find the best channel (with the minimum interference) for transmission. Soon later we will show that $\Rkaa $ and $ \Rkab $ may not be the same when different databases do not have the precise interference information. {We will also show how the accuracy of the interference information changes with the {\eus}' subscription choices.

It is notable that under the strategy $\l\in \{1,2\}$ (subscribing to the database $\dbb_l$'s advanced service), the {\eu}'s expected data rate $\Rl$ cannot be directly computed, as it depends on the accuracy of the database $\dbb_l$'s information.
{We will provide more details regarding the computation of $\Rl$ in (\ref{eq:rate-pay-fixed}).}




%If a \eu~chooses operating on TV \ch, it can only operate on one of the available TV \chs from the \ch~set $\Kset = \{ 1,\ldots, \K \}$ at a particular time on the shared basis (i.e., each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques).
%Let $\Kset = \{ 1,\ldots, \K \}$ denote the set of available TV channels in this area. One \eu~can only operate on \emph{one} of the available \chs~at a particular time on the shared basis (i.e., each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques).
%
%Each \eu~makes its choice through the online platform provided by a \db. We assume that a \db~has the available TV \chs~information and provides such information to each querying \eu~in order to let the \eu~operate on \emph{one} of the available \chs~at a particular time. Note that each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques.
%We also assume that the licensed spectrum holders display their licensed spectrum

For each {\eu} $n\in \Nset$, each channel $\k$ is associated with an \emph{interference level}, denoted by  $\InfTot_{\n,\k}$, which reflects the aggregate interference from all other nearby devices (including TV stations
%\footnotesc{{Notice each TV station has the right to transmit on a particular channel within certain coverage area centered around the TV station, and unlicensed users may be allowed to transmit in this coverage \emph{with a strictly constrained power}. Hence, the TV station might generate interference to unlicensed users (whereas the reverse is not allowed).}}
and other {\eus}) operating on this channel.
%For convenience, we also refer to $\InfTot_{\k}$ as the \emph{quality} of channel $k$.
Due to the fast changing of wireless channels and the uncertainty of {\eus}' mobilities and activities, the interference $\InfTot_{\n,\k}$ is a random variable.
For convenience, we assume that
$$
\InfTot_{\n,\k} \mbox{ is \emph{temporal-independence} and \emph{frequency-independence}}.
$$
That is,
(i) the interference $\InfTot_{\n,\k}$ on channel $\k$ is independent identically distributed (iid) at different times, and (ii)
the interferences on different channels, $\InfTot_{\n,\k}, \k\in\Kset$, are also iid at the same time.\footnotesc{Note that the iid assumption is a reasonable approximation of the practical scenario, where all channel quality distributions are the same but the realized instant qualities of different channels are different (e.g., \cite{chang2009channel,jiang2009channel,zhou2011channel}).}
%Under the i.i.d. assumption, we assume that all channel states $\{ \InfTot_{\k} \}_{\k \in \Kset}$ have the same cumulative distribution function (CDF)
As we are talking about a general WSD $n$, \textbf{we will omit the WSD index $n$ in the notations (e.g., write $\InfTot_{\n,\k}$ as $\InfTot_{\k}$), whenever there is no confusion caused.}
Let $F_{\InfTot}(\cdot)$ and $f_{\InfTot}(\cdot)$ denote the cumulative distribution function (CDF) and probability distribution function (PDF) of $\InfTot_{\k}$, $\forall \k\in\Kset$.\footnotesc{In this paper, we will conventionally  use $F_X(\cdot)$ and $f_X(\cdot)$ to denote the CDF and PDF of a random variable $X$, respectively.}~~~~



\textbf{Interference Level (Information).}
{For a particular {\eu}}, its experienced interference $\InfTot_{\k}$ on a channel $k$ is the aggregate interference from all other (nearby) devices operating on channel $k$,
and usually consists of the following three components:
\begin{enumerate}
\item
$\InfTV_{\k}$: the interference from licensed TV stations;
\item
$\InfEU_{\k,m}$: the interference from another {\eu} $m$ operating on the same channel $k$;
\item
$\InfOut_{\k}$: any other interference from outside systems.
\end{enumerate}
%Here $\InfEU_{\n,\k}$ denotes the interference from an {\eu} $\n$ operating on channel $\k$, and
The total interference on channel $k$ is
$
\InfTot_{\k} = \InfTV_k + \InfEU_k + \InfOut_k
$, where  $\InfEU_k  \triangleq \sum_{m \in \Nkset} \InfEU_{\k,m}$ is the total interference from all other {\eus} operating on channel $k$ (denoted by $\Nkset$).
Similar to $\InfTot_{\k}$, we assume that  $ \InfTV_k , \InfEU_k , \InfEU_{\k,m}$, and $ \InfOut_k$ are random variables with \emph{temporal-independence} (i.e., iid across time) and \emph{frequency-independence} (i.e., iid across frequency).
We further assume that $\InfEU_{\k,m}$ is \emph{user-independence}, i.e., $\InfEU_{\k,m}, m\in \Nkset$, are iid.
%Similarly, we assume that $\{ \InfTV_k \}_{\k \in \Kset}$ are i.i.d., with the CDF $F_{\InfTV}(\cdot)$, and
%$\{ \InfOut_k \}_{\k \in \Kset}$, are i.i.d., with the CDF $F_{\InfOut}(\cdot)$.
%Let $F_{\InfTV}(\cdot)$, $F_{\InfEU}(\cdot)$, and $F_{\InfOut}(\cdot)$ denote the CDFs of $ \InfTV_k , \InfEU_{\n,\k}$, and $\InfOut_k $, respectively.
{It is important to note that \textbf{different {\eus} may experience different interferences $\InfTV_k$ (from TV stations), $ \InfEU_{\k,m} $ (from another WSD), and $ \InfOut_k$ (from outside systems) on a channel $k$, as we have omitted the \eu~index $n$ for all these notations for clarity.}}

Next we discuss these interferences in more details.

\begin{itemize}
\item
Each database is able to compute the interference $\InfTV_k$ from TV stations to every {\eu} (on channel $k$), as it knows the locations and channel occupancies of all TV stations.~~~~
%\footnotesc{Here we consider the long-term average interference, not the instantaneous interference. The same applies to {\eu} and outside interference.}

\item
Each database cannot compute the interference
$\InfOut_k$ from outside systems, due to the lack of outside interference source information.
%\footnotesc{Such outside interference may come from WSDs interacting with other databases, different wireless systems operating on the same or nearby frequency bands, etc.}
Thus, the interference $\InfOut_{\k}$ will \emph{not} be included in a database's information sold to {\eus}.~~~~~~~~
%This reduces the accuracy of information.

\item
Each database may or may not be able to compute the interference $\InfEU_{\k,m}$ from another {\eu} $m$, depending on whether {\eu} $m$ subscribes to the database's advanced service.
Specifically, if {\eu} $m$ subscribes to the advanced service, the database can predict its channel selection (since the {\eu} is fully rational and will always choose the channel with the lowest interference level indicated by the database at the time of subscription), and thus can compute its interference to any other \eu.
However, if {\eu} $m$ does not subscribe to the advanced service, the database cannot predict its channel selection, and thus cannot compute its interference to other \eus.~~~~
\end{itemize}


For convenience, we denote $\Nkset^{[l]},l\in\{1,2\}$, as the set of {\eus} operating on channel $k$ and subscribing to the database $\dbb_l$'s advance service (i.e., those choosing the strategy $\l \in\{1,2\}$), and $\Noset$ as the set of {\eus} operating on channel $k$ and \emph{not} subscribing to any advance service (i.e., those choosing the strategy $\l = 0$).
That is, $\Nkset^{[1]} \bigcup \Nkset^{[2]} \bigcup \Noset = \Nkset $.
Then, for a particular WSD, its experienced interference (on channel $k$) \textbf{known by database $\dbb_l$} is
% (and thus will be included in the database $\dbb_i$'s advanced service to this WSD) is
\begin{equation}\label{eq:known_inf}
\begin{aligned}
\textstyle
\InfKnown_{\k}^{[l]} \triangleq \InfTV_{\k} + \sum_{m \in \Nkset^{[l]}} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from TV licensees and all {\eus} (operating on channel $k$)  subscribing to the database $\dbb_l$'s advanced service.
The WSD's experienced interference (on channel $k$) \textbf{\emph{not} known by database $\dbb_l$} is
% (and thus will not be included in the database $\dbb_i$'s advanced information) is
\begin{equation}\label{eq:unknown_inf}
\begin{aligned}
\textstyle
\InfUnknown_{\k}^{[l]}  \triangleq \InfOut_{\k} +\sum_{m \in \Noset} \InfEU_{\k,m} + \sum_{m \in \Nkset^{[i]},i\neq l} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from outside systems and all {\eus} (operating on channel $k$) not subscribing to the database $\dbb_l$'s advanced service.
Obviously, both $\InfUnknown_{\k}^{[l]}$ and $\InfKnown_{\k}^{[l]}$ are also random variables with temporal- and frequency-independence.
Accordingly, the total interference on {\ch} $\k$ for a WSD can be written as
%\begin{equation}\label{eq:total_inf_new}
%\begin{aligned}
$\textstyle
\InfTot_{\k} = \InfKnown_{\k}^{[l]} + \InfUnknown_{\k}^{[l]}.$~~~~~~
% = \InfTV_{\k} +\InfOut_{\k}+ \sum_{n \in \Nkset} \InfEU_{\n,\k}.
%\end{aligned}
%\end{equation}

\textbf{Since the database $\dbb_l$ knows only $\InfKnown_{\k}^{[l]}$, it will provide this information (instead of the total interference $\InfTot_k$) as the {advanced service} to a subscribing {\eu}.}
%to its advanced service.
It is easy to see that the more {\eus} subscribing to the database $\dbb_l$'s advanced service, the more information the database $\dbb_l$ knows, and the more accurate the database $\dbb_l$'s information will be.~~~~~~~~


Next we can characterize the accuracy of a database's information explicitly.
Due to the frequency independence assumption, it is reasonable to assume that each channel $k\in\Kset$ will be occupied by an average of $\frac{\N}{\K}$ {\eus}.
Let $\Prob_l$ denote the percentage of {\eus} subscribing to the advanced service of database $\dbb_l$ (called the \emph{market share} of database $\dbb_l$).
%Notice that each {\eu} will
%be ``assigned'' to each channel with an equal probability due
%to the assumption of the frequency independence.
Then, among all  $\frac{\N}{\K}$ {\eus} operating on channel $k$, there are, \emph{on average}, $\frac{\N}{\K}\cdot\Prob_l$ {\eus}  subscribing to the database $\dbb_l $'s advanced service, and $\frac{\N}{\K}\cdot(1-\Prob_1 -\Prob_2)$ {\eus} not subscribing to any advanced service.
That is, $| \Nkset | = \frac{\N}{\K}$, $| \Nkset^{[l]} | = \frac{\N}{\K}\cdot\Prob_l, \forall l\in\{1,2\}$, and $|\Noset | = \frac{\N}{\K}\cdot(1-\Prob_1-\Prob_2)$.\footnotesc{{Note that the above discussion is from the aspect of expectation, and in a particular time period, the realized numbers of {\eus} in different channels may be different.}}
Finally, by the {user-independence} of $\InfEU_{\k,m}$, we can immediately calculate the distributions of $ \InfKnown_{\k}^{[l]}$ and $ \InfUnknown_{\k}^{[l]}$ under any given market share $\Prob_l$ via (\ref{eq:known_inf}) and (\ref{eq:unknown_inf}).

%That is, there are an average $\N\cdot \Prob_1$ {\eus} subscribing to the $\dbb_1$'s advanced service, $\N\cdot \Prob_2$ {\eus} subscribing to the $\dbb_2$'s advanced service, and $\N\cdot (1-\Prob_1 - \Prob_2)$ {\eus} not subscribing to the advanced service.
%%Suppose the {\eu} number $\N$ is very large, and
%Since the {\eus} are independent with each other,  then, from a system perspective, all the {\eus} will be ``assigned'' to all available channels equally (i.e., $|\Nset_k| = \frac{\N}{\K}$).
%That is,
%on every available channel $k$, there are on average $\frac{\N}{\K}\cdot\Prob_{\i} $ {\eus} subscribing to the advanced serve of database $\i$ (whose interference (to any particular {\eu}) can be computed by the database) where $ \i \in \{ 1, 2\}$, and $\frac{\N}{\K}\cdot(1-\Prob_1 - \Prob_2)$ {\eus} not subscribing to the advanced serve (whose interference cannot be computed by the database)\footnotesc{This is because of the diversity of users' locations as well as their
%environments. The good channels for a user may not be good for others.
%Moreover, even if users share the similarity in the environment, they
%are likely to be directed to different channels for the purpose of
%interference avoidance.}.
%Similarly, we assume that the interference from single {\eu} {$\{\InfEU_{\n, \k}\}_{\n \in \Nkset}$}, are iid with a CDF   $F_{\InfEU}(\cdot)$.
%
%
%%We denote these three kinds of interference for \ch~$\k$ as random variable $\InfTV_{\k}$, and $\InfOut_{\k}$. We let random variable $\InfEU_{\n}$ as \eu $\n$'s interference.
%%We denote these three kinds of interference as random variable $\InfTV$, $\InfOut$, and $\InfEU$, respectively.
%%We also assume $\{ \InfTV_{\k} \}_{\k \in \Kset}$, $\{ \InfOut_{\k} \}_{\k \in \Kset}$, and $\{ \InfEU_{\n} \}_{\n \in \Nset}$ are i.i.d. random variables.
%%Let $F_{\InfTV}(\cdot)$, $F_{\InfOut}(\cdot)$, and $F_{\InfEU}(\cdot)$ denote the CDF of above three random variable. And correspondingly, let $f_{\InfTV}(\cdot)$, $f_{\InfOut}(\cdot)$, and $f_{\InfEU}(\cdot)$ denote their probability density function (PDF).
%
%%As we assume the total number of \eus~$\N$ is very large, we can consider \eus~are uniformly assign to each \ch,~i.e., there are ${ \N }/{\K}$ \eus~in each \ch.
%%Hence, the total interference level of \ch~$\k$ is:
%%\begin{equation}\label{eq:total_inf}
%%\begin{aligned}
%%%\textstyle
%%\vspace{2mm}
%%\InfTot_{\k} \triangleq \InfTV_{\k} +\InfOut_{\k}+ \frac{\N}{\K} \cdot \InfEU
%%\vspace{2mm}
%%\end{aligned}
%%\end{equation}
%
%%Since every \eu~needs to report its location to \db, \db~can calculate the TV station's interference to each \eu. Hence, \db~knows the distribution of $\InfTV$.
%%As we assume that advanced \eu~will choose the \ch~with highest ranking, therefore, \db~can also calculate the total interference caused by advanced \eu. We denote $\Prob$ as the percentage of advanced \eus \footnotesc{"percentage of advanced \eus" is used throughout this paper to mean the proportion of \eus~in the market that subscribe to advanced service}~. Then, the number of advanced \eus~is $\N \cdot \Prob$. As we assume $\N$ is very large, we can consider both advanced \eus~and basic \eus~are uniformly assign to each \ch,~i.e., there are $\frac{ \N \cdot \Prob }{\K}$ advanced \eus~and $\frac{ \N \cdot (1-\Prob) }{\K}$ basic \eus~in each \ch.
%
%In summary, for each \ch~$\k$, the interference level known by the \db~$\i$ is
%\begin{equation}\label{eq:known_inf}
%\begin{aligned}
%\textstyle
%\InfKnown^{\i}_{\k} \triangleq \InfTV^{\i}_{\k} + \sum_{n \in \Naiset} \InfEU_{\n, \k}~\i = \{ 1 , 2\}.
%%\sum_{n=1}^{\frac{ \N }{\K}  \cdot \Prob_{\i}} \InfEU_{n},~\i = \{ 1 , 2\}.
%\end{aligned}
%\end{equation}
%The interference level not known by the \db~$\i$ is
%\begin{equation}\label{eq:unknown_inf}
%\begin{aligned}
%\textstyle
%\InfUnknown^{\i}_{\k} \triangleq \InfOut^{\i}_{\k} + \sum_{n \in \Noset} \InfEU_{n, \k} + \sum_{n \in \Najset} \InfEU_{n, \k}~\j \neq \i.
%%\InfUnknown^{\i}_{\k} \triangleq \InfOut^{\i}_{\k} + \sum_{n=1}^{\frac{ \N  }{\K}\cdot (1 - \Prob_{\i} - \Prob_{\j})} \InfEU_{n} + \sum_{n=1}^{\frac{ \N  }{\K}\cdot \Prob_{\j}} \InfEU_{n}~\j \neq \i.
%\end{aligned}
%\end{equation}
%The total interference level  on  \ch~$\k$ is
%\begin{equation}\label{eq:total_inf_new}
%\begin{aligned}
%\textstyle
%\InfTot_{\k} = \InfKnown_{\k} + \InfUnknown_{\k} = \InfTV_{\k} +\InfOut_{\k}+ \sum_{n \in \Nkset} \InfEU_{\n,\k}
%\end{aligned}
%\end{equation}
%where $\Naiset$ denotes the set of {\eus} operating on the channel $k$ and subscribing to the advance service of database $\i$; $\Najset$ denotes the set of {\eus} operating on the channel $k$ and subscribing to the advance service of database $\j \neq \i$; $\Noset$ denotes the set of {\eus} operating on the same channel $k$ and not subscribing to the advance service of both database, and $\Nkset$ denotes the set of {\eus} operating on the same channel $k$. Besides, we have $|\Naiset| = \frac{N}{K}\cdot{\eta_i}$, $|\Najset| = \frac{N}{K}\cdot{\eta_j}$, and $|\Noset| = \frac{N}{K}\cdot( 1 - \eta_1 - \eta_2)$. Moreover, we have $\i, \j \in \{1 ,2 \}$, $\i \neq \j$, $\Nkset = \Naiset \bigcup \Najset \bigcup \Noset$, and $\Naiset \bigcap \Najset \bigcap \Noset = \emptyset$.
%The database knows the precise value of $\InfKnown_{\k}$ on every channel $k$, which will be provided for {\eus} who subscribing to the advanced service.
%It is easy to see that the more {\eus} subscribing to this advanced service, the more accurate the advanced information will be.
%%It is assumed that the \db~knows the realized value of $\InfKnown_{\k}$.
%{
%By the iid assumption on $\InfTV_{\k}$, $\InfEU_{\n,\k}$, and $\InfOut_{\k}$, we can easily find that (i) $\{ \InfKnown_{\k} \}_{ \k\in\Kset }$, are i.i.d., (ii) $\{ \InfUnknown_{\k}\}_{\k\in\Kset}$, are i.i.d., and (iii) $\{ \InfTot_{\k} \}_{ \k\in\Kset }$, are i.i.d..
%Finally, we assume that both the \db~and \eus~knows \emph{a priori} the distributions of $\InfTV_{\k}$, $\InfEU_{\n,\k}$, and $\InfOut_{\k}$, and therefore the distributions of $\InfKnown_{\k}$, $\InfUnknown_{\k}$, and $\InfTot_{\k}$ given the market share $\Prob$.
%}

\textbf{Information Value.}
Now we evaluate the value of database $\dbb_l$'s information to {\eus}, which is
reflected by the {\eu}'s benefit (utility) that can be achieved from this information.

We first consider the expected  utility of a {\eu} when not subscribing to any advanced service (i.e., $\l=0$).
In this case, the {\eu} will randomly select a channel from the available channel list, and its expected utility is
\begin{equation}\label{eq:rate-random-fixed}
\begin{aligned}
\textstyle
\RB   \textstyle \triangleq \ut(\R_0) = \ut\left(\int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z)\right),
%& \textstyle = \ut\left( \Ex_{\InfTot} \big[ \rt \left( \InfTot_{\k} \right) \big] \right)
%\\
%& \textstyle = \ut\left( \int_{z} \rt(z) \cdot f_{\InfTot}(z) \cdot \mathrm{d}z \right).
%\vspace{8mm}
\end{aligned}
\end{equation}
where $\R_0$ is the expected data rate given in (\ref{eq:rkgs}).
%By (\ref{eq:total_inf_new}), the distribution of $\InfTot$ is independent of the percentage of advanced {\eus} $\Prob$. Therefore, the value of $\RB$ is also independent of $\Prob$.
%and for an {\eu} with $\l = \S$, its expected utility is
%\begin{equation}\label{eq:rate-sense-fixed}
%\begin{aligned}
%\RS  & \textstyle  \triangleq \ut\left(\Rks\right) ,
%%=  \ut\left( \Ex_{\InfTotMin} \big[ \rt \left(\InfTotMin \right) \big] \right)
%%\\
%%&\textstyle= \ut\big( \K  \int_z \rt(z) \cdot [ 1 - F_{\InfTot}(z)]^{\K - 1} \cdot f_{\InfTot}(z) \cdot \mathrm{d}z \big),
%%\vspace{8mm}
%\end{aligned}
%\end{equation}
%where $\R^{(\G_i)} $ is the expected data rates defined in (\ref{eq:rkgs}).
Obviously, $\RB$ depends only on the distribution of the total interference $\InfTot_k$, while not on the specific distributions of $\InfKnown_k^{[l]}$ and $\InfUnknown_k^{[l]}$. This implies that the accuracy of the database $\dbb_l$'s information does not affect the utilities of those {\eus} not subscribing to its advanced service.


Then we consider the expected utility of a {\eu} when subscribing to the database $\dbb_l$'s advance service (i.e., $\l\in\{1,2\}$).
In this case, the {\db} $\dbb_l$ returns the interference $\{\InfKnown_{k}^{[l]}\}_{k\in\Kset}$ to the {\eu}, together with the basic information such as the available channel list.
%Notice that the total interference also includes the interference $\{\InfUnknown_{k}\}_{k\in\Kset} $ not provided by the database.
%\db~ranks the  {\chs} in ascending order given {\ch} interference level it known (i.e., $\InfKnown_{1}, \InfKnown_{2}, \ldots, \InfKnown_{\K} $). The ranked interference level are denoted by $\InfKnown_{(1)}, \InfKnown_{(2)}, \ldots, \InfKnown_{(\K)}$ and satisfy $\InfKnown_{(1)} < \ldots< \InfKnown_{(\K)}$.
For a rational {\eu}, it will always choose the channel with the minimum $\InfKnown_{k}^{[l]}$ (since $\{\InfUnknown_{k}^{[l]}\}_{k\in\Kset}$ are iid).
%\footnote{This is because the uncertain interference $\{\InfUnknown_{k}\}_{k\in\Kset} $ are i.i.d.}
Let $\InfKnownMin^{[l]} =  \min\{ \InfKnown_{1}^{[l]},  \ldots, \InfKnown_{K}^{[l]}  \} $ denote the minimum interference indicated by the database $\dbb_l$'s information.
Then, the actual interference experienced by a {\eu} (subscribing to the database $\dbb_l$'s advanced service) can be formulated as the sum of two random variables, denoted by $\InfTot^{[l]} = \InfKnownMin^{[l]} + \InfUnknown$. Accordingly, the {\eu}'s expected data rate and expected utility under the strategy $l\in\{1,2\}$ can be computed by
%Hence, the advanced {\eus} transmit at the {\ch} with lowest $\InfKnown$ and with total interference level $\InfTotA = \InfKnownMin + \InfUnknown$. Therefore, the advanced \eu's expect data rate is
\begin{equation}\label{eq:rate-pay-fixed}
\begin{aligned}
\Rl & \textstyle = \Ex_{\InfTot^{[l]}} \big[ \rt \left(\InfTot^{[l]} \right) \big] = \int_z \rt(z)  \mathrm{d} F_{\InfTot ^{[l]}}(z),
\\
\RA_l & \textstyle  \triangleq \ut\left(\Rl\right) = \ut\left(\int_z \rt(z)  \mathrm{d} F_{\InfTot ^{[l]}}(z)	\right) ,
% \textstyle =  \ut\left(\Ex_{\InfTotA} \big[ \rt \left(\InfTotA \right) \big] \right),
%\\
%&= \Ex_{\InfTotA} \big[ \rt \big( \InfKnownMin + \InfUnknown \big) \big] \\
%&= \K \cdot \int_{\InfTotA} \rt(z) \cdot \big[ \int_{\infty}^{\infty} f_{\InfKnown}(z -y) \cdot [ 1 - F_{\InfKnown}(y)]^{K-1} \cdot f_{\InfUnknown}(y) \mathrm{d}y  \big] \mathrm{d}z
%& \textstyle  = \ut \big( \int_z \rt(z) \cdot f_{\InfTotA}(z) \cdot \mathrm{d}z \big),
%\vspace{8mm}
\end{aligned}
\end{equation}
where
 $F_{\InfTot^{[l]}}(z)$ is the CDF of $\InfTot^{[l]}$.
% , and defined by
%\begin{equation*}\label{eq:min-known-pdf}
%%\begin{aligned}
%\textstyle
%f_{\InfTotA}(z) = \K   \int_y \big[ 1 - F_{\InfKnown}(z - y) \big]^{K-1} \cdot f_{\InfKnown}(z -y) \cdot f_{\InfUnknown}(y) \cdot \mathrm{d}y.
%%\vspace{8mm}
%%\end{aligned}
%\end{equation*}
It is easy to see that both $\Rl$ and $\RA_l$ depend on the distributions of $\InfKnown_k^{[l]}$ and $\InfUnknown_k^{[l]}$, and thus depend on the market share $\Prob_l$.
Thus, we will write $\RA_l$ as $\RA_l(\Prob_l)$.
We can further check that $\RA_l(\Prob_l)$ increases with $\Prob_l$.~~~~
%, because the more {\eus} subscribing to the database $\dbb_i$'s advanced service, the more accurate the database $\dbb_i$'s information, and further the more benefit for the {\eus} subscribing to the database $\dbb_i$'s advanced service.
%For convenience, we assume that $\RA_l(\Prob_l)$ is concave in $\Prob_l$ \rev{\footnote{This is validated by the simulation}}.~~~~~~~~~~~


%By (\ref{eq:rate-random-fixed})--(\ref{eq:rate-pay-fixed}), we can find the following useful properties.
%%, which are very important for the later analysis.
%
%\begin{proposition}
%%[Properties of $\RA, \RB, \RS$]
%\label{prop:ABS}
%~
%\begin{itemize}
%\item
% $\RB$ in (\ref{eq:rate-random-fixed})  does not depend on $\Prob_i$, $i\in\{1,2\}$;
% \item
% $\RA_i(\Prob_i)$ in (\ref{eq:rate-pay-fixed}) monotonously increases with $\Prob_i$;
% \item
% $\RA_i(\Prob_i) \geq \RB $, $\forall \Prob_i \in [0, 1]$;
% \item
%$\RA_i(\Prob_i)  = \RB$, only when $\Prob_i=0$ and meanwhile there is no licensee interference $\{ \InfTV_{\k} \}_{k\in\Kset}$.
%\end{itemize}
%\end{proposition}
%
%
%
%Then we consider the expected data rate of the \eus~who subscribe to the advance service (i.e., $\l=\A_{\i}, \i \in \{ 1, 2 \}$).
%With this advanced service, the \db~$\i$ returns the interference $\{ \InfKnown^{\i}_{k}\}_{k\in\Kset}$ to {\eus}, together with the basic information such as the available channel list.
%Notice that the actual interference also includes the interference part $\{\InfUnknown^{\i}_{k}\}_{k\in\Kset} $ not known by the database $\i$.
%%\db~ranks the \chs~in ascending order given \ch~interference level it known (i.e., $\InfKnown_{1}, \InfKnown_{2}, \ldots, \InfKnown_{\K} $). The ranked interference level are denoted by $\InfKnown_{(1)}, \InfKnown_{(2)}, \ldots, \InfKnown_{(\K)}$ and satisfy $\InfKnown_{(1)} < \ldots< \InfKnown_{(\K)}$.
%For a rational {\eu}, he will always choose the channel with the lowest $\InfKnown^{\i}_{k}$ provided~by~the~database.\footnotesc{This is because the uncertain interference $\{\InfUnknown^{\i}_{k}\}_{k\in\Kset} $ are i.i.d.}
%Let $\InfKnownMin^{\i} =  \min\{ \InfKnown^{\i}_{1},  \ldots, \InfKnown^{\i}_{\k}  \} $ denote the lowest interference provided by the database.
%Then, the actual interference experienced by the {\eu} is $\InfTotA^{\i} = \InfKnownMin^{\i} + \InfUnknown$, and accordingly the expected data rate is
%%Hence, the advanced \eus~transmit at the \ch~with lowest $\InfKnown$ and with total interference level $\InfTotA = \InfKnownMin + \InfUnknown$. Therefore, the advanced \eu's expect data rate is
%\begin{equation}\label{eq:rate-pay-fixed}
%\begin{aligned}
%\ut(\R^{\A_{\i}})  = \RA^{\i} & \textstyle \triangleq \ut( \Ex_{\InfTotA^{\i}} \big[ \rt \big(\InfKnownMin^{\i} + \InfUnknown^{\i} \big) \big] ) \\
%%&= \Ex_{\InfTotA} \big[ \rt \big( \InfKnownMin + \InfUnknown \big) \big] \\
%%&= \K \cdot \int_{\InfTotA} \rt(z) \cdot \big[ \int_{\infty}^{\infty} f_{\InfKnown}(z -y) \cdot [ 1 - F_{\InfKnown}(y)]^{K-1} \cdot f_{\InfUnknown}(y) \mathrm{d}y  \big] \mathrm{d}z
%& \textstyle  = \ut( \int_{\InfTotA^{\i}} \rt(z) \cdot h(z) \cdot \mathrm{d}z ),
%%\vspace{8mm}
%\end{aligned}
%\end{equation}
%where
% $h(\cdot)$ is the pdf of $\InfTotA^{\i}$, defined by
%\begin{equation*}\label{eq:min-known-pdf}
%%\begin{aligned}
%\textstyle
%h(z) = \K \cdot \int f_{\InfKnown^{\i}}(z -y) \cdot \big[ 1 - F_{\InfKnown^{\i}}(z - y) \big]^{K-1} \cdot f_{\InfUnknown^{\i}}(y) \cdot \mathrm{d}y.
%%\vspace{8mm}
%%\end{aligned}
%\end{equation*}
%By (\ref{eq:rate-pay-fixed}), we can see that $\RA^{\i}$ depends on the distributions of $\InfKnown^{\i}_k$ and $\InfUnknown^{\i}_k$, and accordingly depends on the market share $\Prob_{\i}$ (and thus, we will also write $\RA^{\i}$ as $\RA(\Prob_{\i})$).
%We can further check that $\RA(\Prob_{\i})$ increases with $\Prob_{\i}$. This is because the more {\eus} subscribing to the advanced service,  the more accurate the database's information is, and further the more benefit for the {\eus} subscribing to the advanced service. We can also note that if two database $\dbb_1$ and $\dbb_2$ share their market shared information, both of them can obtain more accurate information. However, they compete for the same pool of {\eus}. Sharing the information may lead to the decreasing of their own profit.

%Based on the above, we can find the following useful properties, which are very important for the later analysis.
%\begin{proposition}\label{prop:ABS}
%~
%\begin{itemize}
%\item
% $\RB$ in (\ref{eq:rate-random-fixed}) and $\RS$ in (\ref{eq:rate-sense-fixed}) do not depend on $\Prob$;
% \item
% $\RA(\Prob)$ in (\ref{eq:rate-pay-fixed}) monotonously increases with $\Prob$;
% \item
% $\RB\leq \RA(\Prob) \leq \RS $, $\forall \Prob \in [0, 1]$;
% \item
%$\RA(1)  = \RS$, if no outside interference $\{ \InfOut_{\k} \}_{k\in\Kset}$;
% \item
%$\RA(0)  = \RB$, if no licensee interference $\{ \InfTV_{\k} \}_{k\in\Kset}$.
%\end{itemize}
%\end{proposition}




\textbf{Problem Formulation.}
Suppose that each {\eu} is rational, and will always choose the strategy that maximizes its payoff.
We are interested in the following problems: given the information prices $\{\p_1, \p_2\}$ and initial market shares $\{\Prob^0_1, \Prob^0_2 \}$ of databases, how these market shares dynamically evolve and what is the market equilibrium?

%We will study the oligopoly price competition game between databases $\dbb_1$ and $\dbb_2$.
%In the proposed oligopoly price competition game, each database $\dbb_i$ chooses the price $\p_i$ for its information, aiming at maximizing its revenue
%$$
%\Udb_i = \p_i\cdot \Prob_i \cdot N.
%$$
%%given the distributions of licensee interference $\InfTV_{\k}$, outside interference $\InfOut_{\k}$, and single {\eu} interference $\InfEU_{\n,\k}$.
%Note that the market share $\Prob_i $ of the database $\dbb_i$ depends not only on its own price $\p_i$, but also on the other database $\dbb_j$'s price $\p_j$, and thus can be written as $\Prob_i(\p_1, \p_2)$.
%Moreover, the change of $\Prob_i$ will affect the distributions of $\InfKnown_k^i$ (known by the database $\dbb_i$) and $\InfUnknown_k^i$ (not known by the database $\dbb_i$), which in turn will affect the {\eu}'s utility $\RA_i(\Prob_i)$ achieved from the database $\dbb_i$'s advanced service.

%
%revenue maximization where two database compete by choosing prices, given the distributions of licensee interference $\InfTV_{\k}$, outside interference $\InfOut_{\k}$, and single {\eu} interference $\InfEU_{\n}$.
%For database $\i$, its {revenue} is $\p_{\i} \cdot \Prob_{\i}(\bp) \cdot N$.
%%optimal information pricing plan (i.e., $\p_1$ and $\p_2$) that maximizes the database's
%Notice that the database $\dbb_{\i}$'s market share $\Prob_{\i}(\bp)$ is a function of $\bp = (\p_1, \p_2)$.
%Moreover, the change of $\BProb$ will affect the interference levels $\InfKnown^{\i}_k$ (known by the database) and $\InfUnknown^{\i}_k$ (not known by the database), which in turn will affect the {\eu}'s expected data rate $\RA^{\i}(\BProb)$ achieved from the advanced service, and the {\eu}'s decision.

% (ii)
%By comparing (\ref{eq:rate-random-fixed}), (\ref{eq:rate-sense-fixed}), and (\ref{eq:rate-pay-fixed}), we have $\RB \leq \RA \leq \RS$
%When the random variable $\InfKnown$ is zero, we have $\RA = \RB$. Otherwise, $\RA > \RB$, $\forall \Prob \in [0,1]$. If the value of $\InfUnknown$ is zero, we have $\RA = \RS$. Otherwise, $\RA < \RS$, $\forall \Prob \in [0,1]$.

%We associate interference caused by TV station denoted by $\InfTV$, which is a random variable follows from a continuous distribution with cdf $F_{\InfTV}(\cdot) $ and pdf $f_{\InfTV}(\cdot)$. $\InfOut$ represents the interference cause by other database's {\eus} and is a random variable follows from a continuous distribution with cdf $F_{\InfOut}(\cdot) $ and pdf $f_{\InfOut}(\cdot)$ and represents the interference cause by other database's {\eus}. For particular {\eu}, we assume its receiving interference from each {\eu} in the same network \footnotesc{We assume {\eus} who connect to the same database acting in the same network.} $Y$ is a random variable with cdf $F_{Y}(\cdot) $ and pdf $f_{Y}(\cdot)$.



==> Latex_ParticipateSensing_infocom_camera/Section_Ref.tex <==
%!TEX root = main_hybrid_market.tex
%SourceDoc main_hybrid_market.tex


\begin{thebibliography}{1}

%=======================================================

%TV white space
%\bibitem{Obama2013tvws}
%Presidential Memorandum, \emph{Expanding America's Leadership in Wireless Innovation}, June. 2013.

%\bibitem{sen2013sdp}
%S.~Sen, C.~Joe-Wong, S.~Ha, and M.~Chiang, "Smart Data Pricing (SDP): Economic Solution to Network Congestion", \emph{SIGCOMM eBook on Recent Advances in Netowkring}, vol.~1, 2013.

\bibitem{sen2013sdp}
Cisco, ``Cisco Visual Networking Index: Global Mobile Data Traffic
Forecast Update, 2012-2017'', White Paper, Feb. 2013

\bibitem{Microsoft2010report}
%Microsoft Report, \emph{Cambridge TV White Space Trial: A Summary of the Technical Findings}, April.~2012.
Microsoft, ``Cambridge TV White Space Trial'', Tech. Rep., April.~2012.

\bibitem{Ofcom2012tvws}
%OFCOM, \emph{TV White Spaces - A Consultation on White Space Device Requirements}, Nov. 2012.
OFCOM, ``A Consultation on White Space Device Requirements'', 2012.

%\bibitem{FCC2010dractreport}
%FCC Report 159: \emph{Technical and Operational Requirements}, Sep.~2010.


\bibitem{federal2012third}
FCC 12-36, \emph{Third Memorandum Opinion and Order}, 2012.

%\bibitem{cognitive}
%M.~A.~McHenry and D.~McCloskey, \emph{Spectrum Occupancy Measurements: Chicago, Illinois, Novemeber 16-18, 2005}, techniqucal report, Shared Spectrum Company, 2005.

\bibitem{cognitive}
FCC 10-174, \emph{Second Memorandum Opinion and Order}, 2010.


\bibitem{Ofcom2010geo}
Ofcom, ``Implementing Geolocation'', Nov. 2010.




%=======================================================

%Geolocation-database

%=======================================================

% TV white space company and orangization
\bibitem{Google}
Google Spectrum Database, \url{http://www.google.org/spectrum/whitespace/}

\bibitem{SpectrumBridge}
Spectrum Bridge TV White Space, \url{http://www.spectrumbridge.com/ProductsServices/WhiteSpacesSolutions/WhiteSpaceOverview.aspx}

\bibitem{Microsoft}
Microsoft Reserach WhiteFiService, \url{http://whitespaces.msresearch.us/}

%\bibitem{IEEE80222}
%IEEE 802.22 WRAN, [Online] \url{http://www.ieee802.org/22/}
%
%\bibitem{WSAlliance}
%Whitespace Alliance, [Online] \url{www.whitespacealliance.org}

%\bibitem{Microsoft}
%Microsoft Reserach WhiteFiServiice, \url{http://whitespaces.msresearch.us/}


%=======================================================
% TV white space trial network and commercial network

\bibitem{SpectrumBridgeCommericial}
Spectrum Bridge White Space Plus, \url{http://www.spectrumbridge.com/ProductsServices/WhiteSpacesSolutions/OperatorsUsers.aspx}

%=======================================================
\bibitem{federal2004leasing}
%FCC 04-167, \emph{Second Report and Order, Order on Reconsideration, and Second Further Notice of Proposed Rulemarking}, 2004.
FCC 04-167, \emph{Second Report and Order}, 2004.

%\bibitem{FCC_leasing}
%FCC Spectrum Leasing, \url{http://wireless.fcc.gov/licensing/index.htm?job=spectrum_leasing}

%=======================================================
%%% secondary market new product

\bibitem{SpectrumBridgeCommericial2}
Spectrum Bridge SpecEx, \url{http://www.spectrumbridge.com/ProductsServices/search.aspx}


%=======================================================
% TV white space business model secondary market
%\bibitem{luo2012}
%Y.~Luo, L.~Gao, and J. Huang, "Spectrum Broker by Geo-location Database", \emph{IEEE GLOBECOM}, 2012.
\bibitem{luo2012}
%H.~Bogucka, M.~Parzy, P.~Marques, J.~W.~Mwangoka, T.~Forde, ``Secondary Spectrum Trading in TV White Spaces'', \emph{IEEE Communications Magazine}, vol.~50, no.~11, pp.~121-129, Nov. 2012.
H.~Bogucka, \emph{et al.}, ``Secondary Spectrum Trading in TV White Spaces'', \emph{IEEE Commun. Mag.}, vol.~50, no.~11, pp.~121-129, Nov. 2012.

\bibitem{feng2013database}
X.~Feng, J.~Zhang, and J.~Zhang, ``Hybrid Pricing for TV White Space Database'', \emph{IEEE INFOCOM}, 2013.

%\bibitem{luo2013}
%Y.~Luo, L.~Gao, and J. Huang, "White Space Ecosystem: A Secondary Network Operator's Perspective", \emph{IEEE GLOBECOM}, 2013.

\bibitem{luo2013}
%S.~Liu, H.~Zhu, R.~Du, C.~Chen, and X.~Guan, ``Location Privacy Preserving Dynamic Spectrum Auction in Cognitive Radio Network'', \emph{IEEE ICECS}, July. 2013.
S.~Liu, \emph{et al.}, ``Location Privacy Preserving Dynamic Spectrum Auction in Cognitive Radio Network'', \emph{IEEE ICECS}, July. 2013.

%=======================================================
% auction
\bibitem{zhou2008}
%S.~Liu, H.~Zhu, R.~Du, C.~Chen, and X.~Guan, ``Location Privacy Preserving Dynamic Spectrum Auction in Cognitive Radio Network'', \emph{IEEE ICECS}, July. 2013.
X.~Zhou, \emph{et al. }, ``eBay in the Sky: Strategy-Proof Wireless Spectrum Auctions'', \emph{IEEE Mobicom}, Sept. 2008.

\bibitem{zhou2009}
X.~Zhou and H.~Zheng, ``TRUST: A General Framework for Truthful Double Spectrum Auctions'', \emph{IEEE INFOCOM}, April. 2009.


%=======================================================
% Information market
\bibitem{luo2014wiopt}
Y.~Luo, L.~Gao, and J.~Huang, ``Trade Information, Not Spectrum: A Novel TV White Space Information Market Model'', \emph{IEEE WiOpt}, 2014.

\bibitem{luo2014SDP}
Y.~Luo, L.~Gao, and J.~Huang, ``Information Market for TV White Space'', \emph{IEEE INFOCOM Workshop on Smart Data Pricing}, 2014.


%=======================================================
% bargainig theory
\bibitem{harsanyi1977bargaining}
J.~Harsanyi, \emph{Rational Behavior and Bargaining Equilibrium in Games and Social Situations}, {Cambridge Univ. Press}, 1977.

%=======================================================
% supermodular game
\bibitem{topkis1998supermodular}
D.~M.~Topkis, \emph{Supermodularity and Complementarity}, Princeton Univ. Press, 1998.

%=======================================================
% unifor distribution

%\bibitem{Lj2013uniform}
%L.~Duan, J.~Hunag, and B.~Shou, "Optimal Pricing for Local adn Global WiFi Market", \emph{IEEE INFOCOM}, Apr.~2013.

\bibitem{manshaei2008evolution}
%M.~Manshaei, J.~Freudiger, M.~Felegyhazi, P.~Marbach, and J~.P.~Hubaux, ``On Wireless Social Community Networks'', \emph{IEEE INFOCOM}, Apr.~2008.
M.~Manshaei, \emph{et al.}, ``On Wireless Social Community Networks'', \emph{IEEE INFOCOM}, Apr.~2008.

%=======================================================
%% two kindes of TV channels
%\bibitem{kawade2012registed}
%S.~Kawade, "Long-Range Communications in Licence-Exempt TV White Spaces: An Introduction to Soft-License Concept", \emph{International Conference on Cognitive Radio Oriented Wireless Network}, 2012.
%
%\bibitem{FCC2010report}
%FCC Tecchnical Report, \emph{Frees UP Vacant TV Airwaves for Super Wi-Fi Technologies and Other Technologies}, 2010.


%=======================================================

%network effect

%\bibitem{laffont2003network}
%J.~J.~Laffont, \emph{et al}, "Internet Interconncetion and the Off-Net-Cost Pricing Principle", \emph{The RAND Journal of Economics}, 32(2), 2003.
%
%%\bibitem{johari2010network}
%%R.~Johari, and S.~Kummar, "Congestible Services and Network Effects", \emph{The 11th ACM conference on Electronic Commerce}, Jun.~2010.
%
%\bibitem{candogan2012network}
%O.~Candogan, K.~Bimplikis, and K.~Ozadaglar, "Optimal Pricing in Networks with Externalities", \emph{Operation Research}, 60(4), 2012.
%
%\bibitem{jin2008network}
%Y.~Jin, \emph{et al}, "Dynamics of Competition Between Incumbent and Emerging Network Technologies", \emph{IEEE NetEcon}, 2008.

%=======================================================
%% Tipping point
%\bibitem{Gladwell2000tipping}
%M.~Gladwell, \emph{The Tipping Point: How Little Things Can Make a Big Difference}, Back Bay Books, Jan.~2002.

%=======================================================
% TV white space trial
%\bibitem{TVTrial2010}
%The Cape Town TV White Spaces Trial, [Online] \url{http://www.tenet.ac.za/about-us/the-cape-town-tv-white-spaces-trial}


%=======================================================

%Channel independence

%\bibitem{sabharwal2007channel}
%A.~Sabharwal, A.~Khoshnevis, and E.~Knightly,, "Opportunistic Spectral Usage: Bounds and A Multi-Band CSMA/CA Protocal", \emph{IEEE/ACM Transactions on Networking}, pp.533-545, Jun.~2007.

%\bibitem{Zafer2007channel}
%M.~Zafer, and E.~Modiano, "Joint Scheduling of Rate-Guaranteed and Best-Effort Users over a Wireless Fading Channel", \emph{IEEE Transactions on Wirieless Communications}, vol.~6, no.~10, pp.~3825-3835, Oct.~2007.

%\bibitem{chang2009channel}
%N.~B.~Chang, and M.~Liu, "Optimal Channel Probing and Transmission Scheduling for Opportunistic Spectrum Access", \emph{IEEE/ACM Transactions on Networking}, vol.~17, no.~6, pp.~1805-1818, Dec.~2009.
%
%\bibitem{jiang2009channel}
%H.~Jiang, L.~Lai, R.~Fan, and H.~V.~Poor, "Optimal selection of channel sensing order in cognitive radio", \emph{IEEE Transactions on Wirieless Communications}, vol.~8, no.~1, pp.~297-307, Jan.~2009.
%
%\bibitem{zhou2011channel}
%H.~Zhou, P.~Fan, D.~Guo, "Joint Channel Probing and Proportional Fair Scheduling in Wireless Networks", \emph{IEEE Transactions on Wirieless Communications}, vol.~10, no.~10, pp.~3496-3505, Oct.~2011.

%=======================================================
% congestion and positive network effect
\bibitem{shetty2010congestion}
N.~Shetty, G.~Schwartz, and J.~Walrand, ``Internet QoS and Regulations'', \emph{IEEE Trans. Networking}, vol.~17, no.~6, pp.~1725-1737, Dec.~2010.

%\bibitem{acemoglu2010congestion}
%D.~Acemoglu, and A.~Ozdaglar, "Competition and Efficiency in Congested Markets", \emph{Mathematics of Operations Research}, vol.~32, no.~1, pp.~1-31, Feb.~2007.

%\bibitem{westland1992congestion}
%J.~C.~Westland, "Congestion and Network Externalities in the Short Run Pricing of Information System Services", \emph{Management Science}, vol.~38, no.~7, pp.~992-1009, July 1992.

\bibitem{johari2010congestion}
R.~Johari, G.~Y.~Weintraub, and B.~Van~Roy, ``Investment and Market Structure in Industries with Congestion'', \emph{Oper. Res.}, vol.~58, no.~5, pp.~1303-1317, Sept. 2010.

%=======================================================
% price competition game

%\bibitem{Jia2008game}
%J.~Jia, and Q.~Zhang, "Competition and Dynamic of Duopoly Wireless Service Providers in Dynamic Spectrum Market," \emph{ACM Mobihoc}, May, 2008.
%
%
%\bibitem{Duan2012game}
%L.~Duan, J.~Huang, and B.~Shou, "Duopoly Competition in Dynamics Spectrum Leasing and Pricing," \emph{IEEE Trans. Mobile Computing}, vol.11, no. 11, pp. 1706-1719, Nov. 2012.
%
%\bibitem{Niyato2009game}
%D.~Niyato, E.~Hossain, and Z.~Han, "Dynamics Spectrum Access in IEE 802.22-Based Cognitive Wireless Networks: A Game Theoretic Model for Competitive Spectrum Bidding and Pricing," \emph{IEEE Wireless Communications}, vol.16, no. 2, pp. 16-23, Apr. 2009.


% uniform preference

%\bibitem{Lj2013uniform}
%L.~Duan, J.~Hunag, and B.~Shou, "Optimal Pricing for Local adn Global WiFi Market", \emph{IEEE INFOCOM}, Apr.~2013.
%
%\bibitem{manshaei2008evolution}
%M.~Manshaei, \emph{et al}, "On Wireless Social Community Networks", \emph{IEEE INFOCOM}, Apr.~2008.
%
%
%% revenue maximization
%\bibitem{hande2009revenue}
%P.~Hande, \emph{et al}, "Network Pricing and Rate Allocation with Content Provider Participation", \emph{IEEE INFOCOM}, Apr.~2009.


%%=======================================================
%%backward indcution
%\bibitem{fudenberg1991BI}
%D.~Fudenberg and J.~Tirole, Game Theory, MIT Press, 1991
%
%%=======================================================
%
%% tech report

%\bibitem{techrpt}
%Y. Luo, L. Gao, and J. Huang, Tech. Report, [Online]
%\url{http://jianwei.ie.cuhk.edu.hk/publication/AppendixInformationCompetition.pdf}



%=======================================================
%
%%subscription dynmaic
%\bibitem{zemlianov2005evolution}
%A.~Zemlianov and J.~Kephart, "Cooperation and Decision Making in Wireless Multiprovider Setting", \emph{IEEE INFOCOM}, Mar.~2005.
%
%
%\bibitem{ren2011evolution}
%S.~Ren, J.~Park, and M.~Schaar, "User Subscription Dynamics and Revenue Maximization in Communications Markets", \emph{IEEE INFOCOM}, Apr.~2011.
%
%
%%=======================================================
%%refund policy
%
%\bibitem{Courcoubetis2003refund}
%C.~Courcoubetis, and R.~Weber, Pricing Communication Networks: Economics, Technology and Modelling, Wiley Press, 2003.
%
%%=======================================================
%% TV white space techinicial study
%
%\bibitem{feng2011database}
%X.~Feng, J.~Zhang, and Q.~Zhang, ``Database-assisted Multi-AP Network on TV
%  White Spaces: Architecture, Spectrum Allocation and AP Discovery,'' \emph{IEEE DySPAN}, 2011.
%
%\bibitem{chen2012}
%X. Chen and J. Huang, ``Game Theoretic Analysis of Distributed Spectrum Sharing with
%  Database,'' \emph{IEEE ICDCS}, 2012.

%%=======================================================
%% bargaining one-dimentioan search
\bibitem{bargai2001search}
N.~Nisan, \emph{Algorithmic Game Theory},  {Cambridge Univ. Press}, 2007.



\bibitem{report}
Online Technical Report, available at \url{https://www.dropbox.com/s/7gw10z5ahanlr2j/AppendixHySIM.pdf}
\end{thebibliography}


==> Latex_ParticipateSensing_infocom_camera/Section_Simulation.tex <==
%!TEX root = main_hybrid_market.tex
%SourceDoc main_hybrid_market.tex





\begin{figure*}[t]
\centering
\begin{minipage}[t]{0.32\linewidth}
\centering
  \includegraphics[width=2in]{fig_eq_wholes_price}  
  \caption{\rev{Equivalent wholesale price vs $\RL$ under strong positive network externality and strong negative network externality}}.\label{fig:price-vs-diff-L}
\end{minipage}
\begin{minipage}[t]{0.32\linewidth}
\centering
  \includegraphics[width=2in]{fig_NE_price_fixed_network}
  \caption{\rev{The \db's and the \lh's retail price (where LH denotes Licensee and DB denotes database) vs $\RL$ under different network externality}}.\label{fig:price-vs-diff-L2}
\end{minipage}
\begin{minipage}[t]{0.32\linewidth}
\centering
  \includegraphics[width=2.5in]{Fig_NP_fixed_network_effect_normalize2}
  \caption{\rev{Network profit vs $\RL$ under both revenue sharing scheme (RSS) under fixed network externality}.}\label{fig:NP-vs-diff-L}
\end{minipage}
\vspace{-4mm}
\end{figure*}

\vspace{-4mm}
\section{Simulation Result}\label{sec:simulation}


%\com{Lin: Simulations will be updated soon}
In this section,
we provide simulations to evaluate the system performance (e.g., the network profit, the \db's profit, and the \lh's profit) achieved under revenue sharing scheme (RSS).

\subsubsection{Commission Bargaining Solution and Equilibrium Retail Price}
We first show the Nash bargaining solution of RSS, and the corresponding equilibrium retail prices.
In this simulation:
We choose the function $\fx( \Probl ) = \alpha_1 - {\beta_1}\cdot ( 1 - \Probl )^{\gamma_1}$ to model the negative network externality, and choose the function $\gy = \alpha_2 + (\beta_2 - \alpha_2) \cdot {\Proba}^{\gamma_2}$ to model the positive network externality.
%the function $\fx = \log{(P)} - \log[ \alpha_1 + \beta_1 \cdot ( 1 - \Probl) ]$ to model the congestion effect, and have the function $\gy = \alpha_2 + (\beta_2 - \alpha_2) \cdot {\Proba}^{\gamma}$ to model the positive network effect.
We fix $\alpha_1 = 1.8$, $\alpha_2 = 1$, $\beta_1 = 0.8$, $\beta_2 = 1.2$, $\gamma_1 = 0.8$, $\gamma_2 = 0.6$, and change the leasing service quality $\RL$ from $6$ to $10$.
%By letting $\gamma = 0.6$ and adjusting the value of $\alpha_1$, $\alpha_2$, $\beta_1$, and $\beta_2$, we vary $\RB \in [1,1.8]$ for the basic \TVWS~service; $\RA \in [2,3]$ for the advance \TVWS~service. We also let the utility of leasing service $\RL$ vary in $[6,10]$.
%%to map the interference to the instant data rate, where the transmission power is $P = 1000$.





%
%\begin{figure}
%  \centering
%%  \vspace{1mm}
%  \includegraphics[width=2.2in]{fig_w_fixed_network_effect}
%\vspace{-3mm}
%  \caption{Equivalent wholesale price vs $\RL$ under the revenue sharing scheme (RSS) and the wholesale pricing scheme (WPS)}.\label{fig:price-vs-diff-L}
%  \vspace{-4mm}
%\end{figure}
%
%\begin{figure}
%  \centering
%%  \vspace{-1mm}
%  \includegraphics[width=2.2in]{Fig_NE_price_fixed_network_effect}
%\vspace{-2mm}
%  \caption{The \db's and the \lh's retail price (where LH denotes Licensee and DB denotes database) vs $\RL$ under RSS and WPS}.\label{fig:price-vs-diff-L2}
%  \vspace{-7.5mm}
%\end{figure}

Figure \ref{fig:price-vs-diff-L} shows the bargaining solution under different degree of network externality.
For fair comparison, we transform the revenue sharing factor $\delta^{*}$ under RSS into the equivalent wholesale price by $\w^{*} = \delta^{*} \cdot \Probl^{*}$.
From this figure, we can see that the equivalent wholesale price increases with $\RL$ under different degree of network externality.
This is because a higher quality of leasing service attracts more \eus~to the licensed channels, and hence a higher wholesale price is desired to compensate the database's  revenue loss from the advanced service.
Moreover, the wholesale price under strong negative networker externality is higher than that under strong positive network externality.
%This implies that WPS gives more bargaining power to the \db.
\rev{This is because when the information market is negative network externality, the increases number of {\eus}  will severely jeopardize the quality of unlicensed TV channels. Hence, {\eus} are willing to choose licensed channels in order to obtain guarantee quality of service. In such case, the database wants to increase the wholesale price to maintain its revenue.}

Figure \ref{fig:price-vs-diff-L2} shows the equilibrium retail prices under the bargaining solution.
We can see that the equilibrium price of the \db~(denoted by DB) is almost independent of $\RL$, while the equilibrium   price of the \lh~(denote by LH) increases with $\RL$.
This is because a higher quality of leasing service will attract more \eus~to the licensed channels, and thus allows the \lh~to charge a higher service price.
Moreover, the equilibrium price of \lh~under strong negative network externality is higher than that under strong positive externality.
This is because under strong negative network externality, the small increase of {\eus} in the information market will dramatically decreases the quality of unlicensed TV channels. Hence, the licensee can charge a higher price due to more {\eus} will choose leasing service. 


%\begin{figure*}
%  \centering
%  \includegraphics[width=2.2in]{fig_network_vs_L_db_new2}
%  \includegraphics[width=2.2in]{fig_network_vs_L_licensee_new2}
%  \includegraphics[width=2.2in]{fig_network_vs_L_NP_new2}
%%  \includegraphics[width=2.2in]{fig_DB_diff_L_mix_new}
%  \caption{(a) The \db's profit, (b) The \lh's profit, (c) Network profit under the revenue sharing scheme (RSS) and the wholesale pricing scheme (WPS). The blue square denotes that WPS outperforms RSS, while the red circle denotes that RSS has better performance than WPS.}\label{fig:rss_vs_wps}
%  \vspace{-3mm}
%\end{figure*}

\subsubsection{System Performance}
Now we show the network profit, i.e., the aggregate profit of the \db~and the \lh~achieved under both RSS in Figure \ref{fig:NP-vs-diff-L} given the fixed network externality.
%\begin{figure*}
%  \centering
%  \includegraphics[width=3.2in]{Fig_NP_fixed_network_effect2}
%  \includegraphics[width=3.2in]{Fig_SW_fixed_network_effect}
%%  \includegraphics[width=2.2in]{fig_DB_diff_L_mix_new}
%%  \vspace{-5mm}
%  \caption{(a) Network profit and (b) Social Welfare vs $\RL$ under revenue-sharing-scheme(RSS) and wholesale-price-scheme(WPS).}\label{fig:profit-vs-diff-L}
%\end{figure*}
In this figure, we use the black dash-dot line (with mark $+$) to denote the coordination benchmark, where the \db~and the \lh~act as an integrated party to maximize their aggregate profit. We use the red dash-dot line (with mark $\times$) to denote the non-cooperation benchmark (with pure information market only), where the \db~does not want to display the \lh's licensed \ch~information. The brown dash-dot line (with mark $\bullet$) denotes the case where the \lh~sells channels on a third-party spectrum market platform.

Figure \ref{fig:NP-vs-diff-L} shows that our proposed RSS outperform the non-cooperation scheme significantly (e.g., increasing the network profit up to $87\%$).
It further shows that the gap between our proposed RSS and coordination benchmark is small (e.g., less than $4\%$).
Such a gap is caused by the \emph{imperfect} coordination of the database and the licensee.
%Namely, both the \db~and the \lh~aim at maximizing their own profits instead of the aggregated profit.
In other words, they cooperate somewhat  but not coordinate completely.
We call this gap as the non-coordination loss.
We can also see that our proposed RSS always outperforms the scheme with a third-party platform, in terms of the network profit.
%\rev{However, WPS is better than the third-party platform only when $\RL$ is not too high.
%This is because the database is more aggressive in the price competition game under WPS than under RSS.
%%When the quality of leasing service is high, the competition between the database and the licensee is not so severe. Hence,
%The aggressive behavior of the database causes more non-coordination loss, and thus harms the aggregated network profit.}


%\subsubsection{Comparison between RSS and WPS}
%%Now we compare the performance of revenue-sharing-scheme (RSS) with that of wholesale-price-scheme (WPS). We use our previous analytical results and some numerical examples to outline a possible choice of scheme selection strategy. in terms of the \db's and the \lh's profit while considering the impact of congestion effect, positive network effect, and the quality of leasing service.
%%Note that the performances of revenue-sharing-scheme (RSS) with that of wholesale-price-scheme (WPS) are closely related to the quality of leasing service and the network effect. Hence, we classify the two proposed schemes along these two dimensions as illustrated in Figure \ref{fig:rss_vs_wps}. However, we do not explicitly draw boundaries between these two schemes because these boundaries depend not only on the expected profits, but also on unquantifiable factors such as complexities of bargaining form. Next, we summarize our results through a discussion around this figure.
%Now we compare RSS with WPS, in terms of the \db's, the \lh's, and the network profit, under different degrees of network externality and different levels of leasing service quality $\RL$.
%%
%%while considering the impact of negative network externality, positive network externality, and the quality of leasing service.
%
%%In order to capture the impact of the congestion effect and positive network effect, we approximate the function $\fx(\cdot)$ and $\gy(\cdot)$ as follows:
%%\begin{equation}\label{eq:congestion_function2}
%%\begin{aligned}
%%\textstyle
%%%\fx( \Probl, \Proba ) &= Pt - {\beta_1}\cdot ( 1 - \Probl )^{\alpha_1} \\
%%%&= Pt - {\beta_1}\cdot ( \Proba + \Probb )^{\alpha_1}
%%\fx( \Proba ) &= P - {\beta_1}\cdot ( \Proba + \Probb )^{\gamma_1}
%%\end{aligned}
%%\end{equation}
%%\begin{equation}\label{eq:positive_function2}
%%\textstyle
%%\gy( \Proba ) =  {\beta_2}\cdot ( \Proba )^{\gamma_1}
%%\end{equation}
%%%Note that $1 - \Probl = \Proba + \Probb$.
%%
%%In such case, we have the utility provided by the database's advance service and basic service are
%%\begin{equation}\label{eq:basic service}
%%\textstyle
%%%\RB(\Probl,\Proba) = \fx( \Probl, \Proba)
%%\RB(\Proba) = \fx( \Proba)
%%\end{equation}
%%\begin{equation}\label{eq:advanced service}
%%\begin{aligned}
%%\textstyle
%%%\RA(\Proba) &= \fx( \Probl, \Proba) + \gy(\Proba) \\
%%%&= Pt - {\beta_1}\cdot ( \Proba + \Probb )^{\alpha_1} + {\beta_2}\cdot ( \Proba )^{\alpha_2}
%%\RA(\Proba) &= P - {\beta_1}\cdot ( \Proba + \Probb )^{\gamma_1} + {\beta_2}\cdot ( \Proba )^{\gamma_1}
%%\end{aligned}
%%\end{equation}
%
%To characterize the degree of negative or positive network externality in the information market, we first derive the first-order derivative of $\RA$ with respect to $\Proba$, i.e.,
%$
%\textstyle
%\frac{ \partial{\RA} }{ \partial{\Proba} } = -{\gamma_1} \cdot{\beta_1}\cdot ( \Proba + \Probb )^{\gamma_1 - 1} + {\gamma_2}\cdot {\beta_2}\cdot ( \Proba )^{\gamma_2-1}.
%$
%Notice that if $\frac{ \partial{\RA} }{ \partial{\Proba} } > 0$, the value of advance information increases with the market share $\Proba$ (i.e., the percentage of users purchasing the advanced information).
%In this case, we can intuitively say that the positive network externality is dominant.
%On the other hand, if $\frac{ \partial{\RA} }{ \partial{\Proba} } < 0$,
%the value of advance information decreases with the market share $\Proba$, and we can intuitively say that the negative network externality is dominant.
%
%For an easily comparison, we set $\gamma_1 = \gamma_2$ and change the value of $\beta_1$ and $\beta_2$ to achieve different degrees of network externality.
%Specifically, we introduce $\lambda = \beta_1/\beta_2$ to represent the degree of network externality.
%Obviously, if $\lambda = \beta_1/\beta_2  < 1$, then $\frac{ \partial{\RA} }{ \partial{\Proba} } > 0$ for any $\{ \Proba, \Probb \}$, hence the information market is positive dominant. If $\lambda > (\frac{\Proba + \Probb}{\Proba})^{\gamma_1 - 1}$, then $\frac{ \partial{\RA} }{ \partial{\Proba} } < 0$, hence the information market is negative dominant.
%Then, a small $\lambda$ denotes that positive network effect is dominant, while a large $\lambda$ denotes that negative network externality is dominant.
%
%In Figure \ref{fig:rss_vs_wps}, we compare RSS with WPS, in terms of the database's profit, the licensee's profit, and the total network profit, under different $\lambda$ and $\RL$.
%The $x$-axis is the network effect parameter $\lambda $, and the  $y$-axis is leasing service quality $\RL$.
%The blue square denotes that WPS outperforms RSS, while the red circle denotes that RSS outperforms WPS.
%
%From Figure \ref{fig:rss_vs_wps}.(a), we can see that when the negative network externality is dominant ($\lambda$ is large), RSS always outperforms WPS in terms of the database's profit; when the positive network externality is dominant ($\lambda$ is small), RSS outperforms WPS only when $\RL$ is large.
%This implies that RSS is a better choice for the \db~in most network scenarios.
%\rev{This is because when the positive network externality is dominant, the market share is more important to the \db~than the price. As the database is more aggressive in terms of market competition under WPS than under RSS, the \db~is willing to choose WPS. On the contrary, when the negative network externality is dominant, the increase of the \db's market share may severely decrease the quality of advanced service. In this case, it is better for the \db~to let the \lh~take the large fraction of the market share and earn the profit by charging the commission charge from the \lh. Hence, RSS is the better choice for the \db.}
%
%%This is because when the positive effect is dominant, the market share dominates the retail price for the database (from the simulation, it shows that the NE price of the database is almost zero, but the market share is approximate $30\%$). In such case, the wholesale-price-scheme is a better choice for the database because it can charges a higher wholesale price. On the contrary, when the congestion effect is dominant, the retail price dominates the market share for the database (from the simulation, it shows that the market share of the database is almost zero, but the price can be slowly higher). In such case, the revenue-sharing-scheme is a better choice for the database.
%
%From Figure \ref{fig:rss_vs_wps}.(b), we can see that when the positive network externality is dominant ($\lambda$ is small), WPS always outperforms RSS, in terms of the database's profit; when the negative  network externality is dominant ($\lambda$ is large), WPS outperforms RSS only when $\RL$ is large.
%This implies that WPS is a better choice for the \lh~in most network scenarios.
%\rev{This is because when the positive network externality is dominant, the competition between the database and the licensee becomes severe. The number of successful transactions on leasing service may be small. %Moreover, the retail price of both the database and the licensee decreases, so that the wholesale price charged by the database also decreases.
%In such case, the licensee is more willing to pay the database commission charge based on each successful transaction. On the contrary, when the negative network externality is dominant, more and more users are wiling to use leasing service. The licensee is more wiling to share a fixed percentage of revenue with the database.}
%
%%\rev{As both RSS and WPS aim at coordinating the strategies of the \db~and the \lh~so that the network profit would be close to the benchmark (i.e., the \db~and the \lh~acts as an integrated party to make the decision),}
%%\com{This is not what we have proposed? This is in fact the reason behind the non-coordination loss? }
%Figure \ref{fig:rss_vs_wps}.(c) shows that the regulator prefers WPS when the negative network externality is dominant, and prefers RSS when the positive network externality is dominant.
%%\rev{from the regulator's point of view, it prefers WPS when the negative network externality is dominant, and prefers RSS when the positive network externality is dominant.}
%
%%From Figure \ref{fig:rss_vs_wps}.(c), we can further see that when the positive network externality is dominant ($\lambda$ is small), WPS often outperforms RSS, in terms of the total network profit; when the negative  network externality is dominant ($\lambda$ is large), RSS often outperforms WPS.
%
%
%
%%However, when the value of $\RL$ increases, it is more precipitous to drop the wholesale price than to cut the retail price of the \lh.
%
%%Because the competition in the WPM scheme is more severe than that in the RSM, the double marginalization problem can be solved better in the WPM scheme than than in the RSM. Hence, the \db~has better performance in the WPM scheme.
%%This is because a higher wholesale price leads to a higher leasing price, and thus lower market share of the \lh~as shown in Figure \ref{fig:price-vs-diff-L}. When the value of $\RL$ is small, i.e., the competition between the \db~and the \lh~is sever, setting a higher wholesale price can help the \db~obtain a larger market share while grasping
%
%
%
%
%%\textbf{Market Equilibrium.}
%%Figure \ref{fig:db-payoff-vari-tv} illustrate the market equilibrium (i.e., the stable percentage of end-users subscribing to the advanced service) vs the information price $\p$.
%%We can see that the market share decreases with the price. This means that less end-users are willing to purchase information under a higher price.
%%We can also see that the market share increases with the end-user's sensing cost (recall that $\alpha = \frac{c}{S-B}$).
%%This means that more end-users are willing to purchase information if the sensing is expensive.
%%More interestingly, we can see that there exists the \emph{tipping price point}, at which a slight change will lead to a dramatic decrease on the market equilibrium.
%%
%%
%%
%%\textbf{Database Revenue.}
%%Figure \ref{fig:db-payoff-vari-out} illustrates the \db's~revenue under different licensee interferences $\InfTV$ (with a mean changing from $10$mw to $100$mw). The mean value of $\InfOut$ and $\InfEU$ are fixed at $40$mw and $10$mw, respectively.
%%%and the standard variances of $\InfOut$ and $\InfEU$ is $12$ and $3$, respectively.
%%We can see that the database's revenue increases with the mean of the licensee interference. This is because the licensee interference is known by the database, and a larger licensee interference makes the database's information more valuable for the end-users.
%%We can further see from each bar group that the database's revenue increases with the end-user's sensing cost.
%
%
%
%
%%Each bar group denotes the performance under different sensing cost (from $\afa =0.1$ to $1$ with step 0.1).
%%We can see that the \db'~revenue increases with the sensing cost, since a larger sensing cost will drive more end-users subscribing to the service.
%%Moreover, comparing different bar groups, we can see that the database's revenue increases with the mean of $\InfTV$, since a large $\InfTV$ increases the value of the database's information.
%%
%
%
%%The reason is as follow. As the sensing cost increases, the \db~can set a higher price to make the stable point reach $\Probc$. In such case, the revenue of \db~increases. If we compare across different bar groups, then we can see the \db~revenue is increasing with the mean of $\InfTV$ given the same value of sensing cost. This is because with the increase of $\InfTV$ 's mean, the \eus~total interference mainly caused by the TV stations. As the \db~knows the TV station's interference perfectly, it can use its information advantage to set a higher price to attract \eus. Therefore, the revenue of \db~increases.
%%
%%\begin{figure}[t]
%%\vspace{-4mm}
%%  \centering
%%  \includegraphics[width=2.9in]{fig-profit-new2}
%%\vspace{-3mm}
%%  \caption{Database's revenue under different licensee interferences.}
%%  \label{fig:db-payoff-vari-out}
%%  \vspace{-7mm}
%%\end{figure}
%
%%
%%Figure \ref{fig:db-payoff-vari-out} illustrates the the \db's~revenue under different outside interference $\InfOut$ (with a mean from $10$mw to $100$mw with step $10$mw), where the mean of $\InfTV$ and $\InfEU$ are fixed at $40$mw and $10$mw.
%%Similarly, we can see that the \db'~revenue increases with the sensing cost.
%%Comparing different bar groups, we can see that the database's revenue decreases with the mean of $\InfOut$, since a large $\InfOut$ decreases the value of the database's information.
%%
%
%%\com{Would it be more interesting if we use the figure showing the impact of end-users distribution?}
%%Figure \ref{fig:db-payoff-vari-tv} illustrates the performance of the \db's~revenue under different mean and variances of $\InfOut$ (from $10$ to $100$ with step $10$), while the mean of $\InfOut$ and $\InfEU$ is $40$ and $10$, and the standard variances of $\InfOut$ and $\InfEU$ is $12$ and $3$, respectively. In each bar group, the sensing cost is $\beta$ times of $( \RS - \RB)$ and $\beta$ changes from $0.1$ to $1$ with step $0.1$. If we compare across different bar groups, then we can see the \db~revenue is decreasing with the mean of $\InfOut$ given the same value of sensing cost. This is because with the increase of $\InfOut$ 's mean, the \eus~total interference mainly caused by the outside interference which is unknown by \db.~As the \db~knows less about the channel total interference, its quality of advanced service is worse than sensing service. Therefore, the revenue of \db~decreases.
%
%%\begin{figure}[t]
%%%\vspace{-3mm}
%%  \centering
%%  \includegraphics[width=3.4in]{DB_profit_EU_new}
%%  \caption{Database's profit with different \eus~interference }
%%  \label{fig:db-payoff-vari-eu}
%%  \vspace{-2mm}
%%\end{figure}
%%
%%Figure \ref{fig:db-payoff-vari-eu} illustrates the performance of the \db's~revenue under different mean and variances of $\InfEU$ (from $2$ to $20$ with step $2$), while the mean of $\InfTV$ and $\InfOut$ is $40$ and $40$, and the standard variances of $\InfOut$ and $\InfEU$ is $12$ and $12$, respectively. We can get the similar results in each bar group. If we compare across different bar groups, then we can see the \db~revenue is a convex function of the mean of $\InfEU$ given the same value of sensing cost. This is because $\InfEU$'s impact on $\InfTot$ increases with the mean of $\InfEU$. In such case, the \db~has to decrease its price to attract more \eus~in order to guarantee its quality of its advanced service \footnote{Note that the quality of advanced service depends on the \db's information accuracy concerning the total interference. More advanced users can help \db~know more about the total interference level}. When the mean of $\InfEU$ is small, the benefit brought by attracting \eus~can not compensate the decreasing price. Hence, the revenue of \db~is first decrease with the mean of $\InfEU$. However, when the mean of $\InfEU$ keeps on increasing until the total interference mainly comes from $\InfEU$, i.e, $\Ex (\InfTot) \approx \Ex (\InfEU)$, the benefit of attracting more \eus is large than the loss of decreasing price. Hence, the revenue of \db~is increasing with the mean of $\InfEU$.
%
%
%
%


==> Latex_ParticipateSensing_infocom_camera/Section_Subscription_dynamic.tex <==
%!TEX root = main_hybrid_market.tex
%SourceDoc main_hybrid_market.tex


\section{Layer III -- User Behavior and Market Equilibrium}
\label{sec:user_subscript}

In this section, we study the user behavior and market dynamics in Layer III, given the database's information price $\pa$ and the licensee's channel price $\pl$ (in Layer II).
In the following, we first discuss the {\eu}'s best choice, and show how the user behavior dynamically evolves, and how the market converges to an equilibrium point.

\vspace{-3mm}
\subsection{{\Eu}'s Best Strategy}\label{sec:user-best}

Now we study the best strategy of   {\eus}, given the prices $\{\pl, \pa\}$ and the initial market state $\{\Probl^0, \Proba^0, \Probb^0\}$ where $\Probb^0 + \Proba^0 + \Probl^0 = 1$.
Notice that each {\eu} will choose a strategy that maximizes its payoff defined in (\ref{eq:utility-basic}).
Hence, for a type-$\th$ {\eu}, its best strategy is\footnote{{Here, ``iff'' stands for ``if and only if''.
Note that we omit the case of $\th \cdot \RL -  \pl = \max\{ \th \cdot \RA  -  \pa ,\ \th \cdot \RB\}$, $\th \cdot \RA -  \pa = \max\{ \th \cdot \RL  -  \pl ,\ \th \cdot \RB\}$, and $\th \cdot \RB  = \max\{ \th \cdot \RL - \pl, \th \cdot \RA  -  \pa \}$, which are negligible (i.e., occurring with zero probability) due to the continuous distribution of $\th$.}}~~~~
\begin{equation}
\left\{
\begin{aligned}
\l_{\th}^* = \LS, & \mbox{~~~~iff~~} \th \cdot \RL -  \pl > \max\{ \th \cdot \RA  -  \pa ,\ \th \cdot \RB\}
\\
\l_{\th}^* = \A, & \mbox{~~~~iff~~} \th \cdot \RA  -  \pa >  \max\{ \th \cdot \RL  -  \pl ,\
 \th \cdot \RB\}
\\
\l_{\th}^* = \B, & \mbox{~~~~iff~~} \th \cdot \RB > \max\{ \th \cdot \RL  -  \pl, \ \th \cdot \RA -  \pa \}
\end{aligned}
\right.
\end{equation}
where $\RB =  \fx(1- \Probl^0)$, and $\RA = \fx(1- \Probl^0) + \gy(\Proba^0)$.\footnote{Here we have written $\Proba^0 + \Probb^0$ as $1-\Probl^0$. For convenience, we will use $\Probl $ (the leasing service's market share) and $\Proba$ (the advanced service's market share) to represent the market state, since the basic service's market share $\Probb = 1 - \Probl - \Proba$ can be directly computed by $\Probl $ and $ \Proba $.}


To better illustrate the above best strategy, we introduce the following notations:
\begin{equation*}\label{eq:p-thres}
\textstyle
\thlb \eq \frac{ \pl}{ \RL- \RB },
~~~~
\thab \eq \frac{ \pa}{ \RA- \RB },
~~~~
\thla \eq \frac{\pl-\pa}{\RL - \RA}.
\end{equation*}
%\begin{equation*}\label{eq:p-thres}
%\textstyle \pth_{02} = \frac{ \p_0}{ \RS- \RB },
%~~\textstyle \pth_{12} = \frac{ \p_1}{ \RA- \RB },
%~~\mbox{and}~~ \pth_{01} = \frac{\p_0-\p_1}{\RS - \RA}.
%\end{equation*}
%\begin{equation*}\label{eq:p-thres}
%\textstyle \thlb(\Probl^0) = \frac{ \pl}{ \RL- \RB },
%~~\textstyle \thab(\Proba^0) = \frac{ \pa}{ \RA- \RB },
%~~\mbox{and}~~ \thla(\Probl^0,\Proba^0) = \frac{\pl-\pa}{\RL - \RA}.
%\end{equation*}
%\com{Yuan: do you think if it is better to use the following equation would be better?
%\begin{equation*}\label{eq:p-thres}
%\textstyle \thlb(\Probl^0) = \frac{ \pl}{ \RL- \fx(1- \Probl^0) },
%~~\textstyle \thab(\Probl^0) = \frac{ \pa}{ \fx(1- \Probl^0) },
%~~\mbox{and}~~ \thla(\Probl^0,\Proba^0) = \frac{\pl-\pa}{\RL - \fx(1 - \Probl^0) - \gy(\Proba^0)}.
%\end{equation*}
%}
Intuitively, $\thlb$ denotes the smallest $\th$ such that a type-$\th$ \eu~prefers the leasing service than the basic service; $\thab$ denotes the smallest $\th$ such that a type-$\th$ \eu~prefers the advanced service than the basic service; and $\thla$ denotes the smallest $\th$ such that a type-$\th$ \eu~prefers the leasing service than the advanced service.
Notice that $\RA$ and $\RB$ are functions of initial market shares $\{\Probl^0, \Proba^0, \Probb^0\}$. Hence, $\thlb $, $\thab$, and $\thla$ also functions of $\{\Probl^0, \Proba^0, \Probb^0\}$.
Figure \ref{fig:threshold} illustrates the relationship of $\thlb$, $\thab$, and $\thla$.

\begin{figure}
\centering
  \includegraphics[width=2.6in]{threshold}
  \vspace{-2mm}
  \caption{Illustration of $\thlb$, $\thab$, and $\thla$.}\label{fig:threshold}
  \vspace{-4mm}
\end{figure}

%Figure \ref{fig:threshold} illustrates the relationship of $\thlb$, $\thab$, and $\thla$.
%The upper subfigure illustrates the relationship when  $\thlb > \thab$.
%In this case, it is easy to check that
%%$$
%%\thla - \thlb = \frac{\pl(\RA-\RB) - \pa(\RL-\RB)}{(\RL-\RA)(\RL-\RB)} > 0 ,
%%$$
%%since $\RL > \RA $, $\RL > \RB $, and
%%$\pl (\RA-\RB) > \pa(\RL-\RB) $ as $\thlb > \thab$.
%%Hence, we have:
%$\thla > \thlb > \thab $.
%This subfigure illustrates that when  $\thlb > \thab$, (i)
%the best strategy of users with $\th \in [0, \thab)$ is to choose the basic service,
%(ii) the best strategy of users with  $\th \in (\thab, \thla)$ is
%to choose the advanced service,
%and (iii) the best strategy of users with  $\th \in (\thla, 1]$ is
%to choose  the leasing service.
%The lower subfigure illustrates the relationship when $\thlb < \thab$.
%We can similarly check that
%$\thla - \thlb < 0$, and hence $\thla < \thlb < \thab $.
%This subfigure shows that when  $\thlb < \thab$, (i)
% the best strategy of users with $\th \in [0, \thlb)$
% is to choose the basic service,
%(ii)  the best strategy of users with $\th \in (\thlb, 1]$
% is to choose the leasing service,
% and (iii) no user is willing to choose the advanced service.~~~~~~~~~~~~~

\rev{
Intuitively, Figure \ref{fig:threshold} implies that the users with a high utility evaluation factor $\th$ are more willing to choose the leasing service in order to achieve a large utility.
The users with a low utility evaluation factor $\th$ are more willing to choose the basic service so that they will pay zero service cost.
The users with a middle utility evaluation factor $\th$ are willing to choose the advanced service, in order to achieve a relatively large utility with a relatively low service cost.
Notice that when the information price $\pa$ is high or the information value (i.e., $\RA-\RB$) is low, we could have $\thlb < \thab$, in which no users will choose the advanced service (as illustrated in the lower subfigure of Figure \ref{fig:threshold}).
}


%\begin{figure*}
%\centering
%  \includegraphics[width=3.4in]{market_share_fix}
%  ~~
%  \includegraphics[width=3.4in]{market_share_fix2}
%  ~~
%  \vspace{-2mm}
%  \caption{Market share of (a) the \lh~, and (b) the \db~when $\RL > \RA$.}\label{fig:demand}
%  \vspace{-4mm}
%\end{figure*}

Next we characterize the new market shares (called the \emph{derived market shares}) resulting from the users' best choices mentioned above.
Such derived market shares are important for analyzing the user behavior dynamics and market evolutions in the next subsection.
Recall that $\th$ is uniformly distributed in $[0,1]$.
Then, given any initial market shares $\{\Probl^0, \Proba^0 \}$, the newly derived market shares $\{ \Probl,\Proba \}$ are
\begin{itemize}
\item
If $\thlb > \thab$, then $\Probl = 1 -  \thla$ and $\Proba  = \thla - \thab$;
\item
If $\thlb \leq \thab$, then $\Probl = 1 - \thlb$ and $\Proba  = 0$.
\end{itemize}

Formally, we have the following derived market shares.
\vspace{-2mm}
\begin{lemma}\label{lemma:market-share}
Given any initial market shares $\Probl^0$ and $\Proba^0$, the derived market shares  $\Probl$ and $\Proba$ are given by
\begin{equation}\label{eq:user-prob-1}
\textstyle
\left\{
\begin{aligned}
\Probl  & \textstyle
= \max \big\{ 1 - \max\{ \thla, \thlb \} ,\ 0  \big\},\\
\Proba  & \textstyle
= \max \big\{ \min\{ \thla ,1 \} - \thab ,\ 0  \big\}.
\end{aligned}
\right.
\end{equation}
\end{lemma}

The results in Lemma \ref{lemma:market-share} assume that all \eus~update the best strategies once and simultaneously.
Since $\thlb$, $\thab$, and $\thla$ are functions of initial market shares $\{\Probl^0, \Proba^0\}$, the derived market shares $\{\Probl ,\Proba \}$  are also functions of  $\{\Probl^0,\Proba^0\}$, and hence can be written as  $\Probl(\Probl^0, \Proba^0)$ and $\Proba(\Probl^0, \Proba^0)$.



%In such case, no {\eus} will chose leasing licensed spectrum. All {\eus} only make the choice between the \db's basic service and advance service. This is the pure information market for the TV white space network and has been analyzed in \cite{luo2014wiopt}. Later, we will compare our hybrid market model with the pure information market.


%Based on the {\eus}' best choices, we can compute the new derived market shares of the \lh~$\Probl$ and of the \db~$\Proba$.
%For convenience, we introduce the following notations:
%%\begin{equation*}\label{eq:p-thres}
%%\textstyle \pth_{02} = \frac{ \p_0}{ \RS- \RB },
%%~~\textstyle \pth_{12} = \frac{ \p_1}{ \RA- \RB },
%%~~\mbox{and}~~ \pth_{01} = \frac{\p_0-\p_1}{\RS - \RA}.
%%\end{equation*}
%\begin{equation*}\label{eq:p-thres}
%\textstyle \thlb(\Probl^0) = \frac{ \pl}{ \RL- \RB },
%~~\textstyle \thab(\Proba^0) = \frac{ \pa}{ \RA- \RB },
%~~\mbox{and}~~ \thla(\Probl^0,\Proba^0) = \frac{\pl-\pa}{\RL - \RA}.
%\end{equation*}
%%\com{Yuan: do you think if it is better to use the following equation would be better?
%%\begin{equation*}\label{eq:p-thres}
%%\textstyle \thlb(\Probl^0) = \frac{ \pl}{ \RL- \fx(1- \Probl^0) },
%%~~\textstyle \thab(\Probl^0) = \frac{ \pa}{ \fx(1- \Probl^0) },
%%~~\mbox{and}~~ \thla(\Probl^0,\Proba^0) = \frac{\pl-\pa}{\RL - \fx(1 - \Probl^0) - \gy(\Proba^0)}.
%%\end{equation*}
%%}
%Intuitively, $\thlb$ represents the smallest $\th$ such that a type-$\th$ \eu~prefers the leasing service of the \lh~than the basic service of the \db; $\thab$ represents the smallest $\th$ such that a type-$\th$ \eu~prefers the advanced service of the \db~than the basic service of the \db, and $\thla$ represents the smallest $\th$ such that a type-$\th$ \eu~prefers the leasing service of the \lh~than the advanced service of the \db.

%The change of market share depends on the relative relationship between $\RB$, $\RA$, and $\RL$. It is easy to check that $\RB < \RA$. Hence, we only need to consider the following 3 cases.

%\textbf{Case I: $\RB < \RA < \RL$.}
%This case means leasing service brings higher expected utility to the \eu~than both basic service and advance service do.
%For clarity, we illustrate the values of $\thlb$, $\thab$, and $\thla$ in Figure \ref{fig:threshold}.
%Specifically, one can show that in the case where $\thlb > \thab$, then $\thab < \thlb < \thla$, and in the case where $\thlb < \thab$, then $\thla < \thlb < \thab$.
%Intuitively, {\eus} with high valuation of service utility (i.e., $\th \in [ \max\{\thlb, \thla\}, 1]$) are willing to lease the licensed spectrum and use the spectrum exclusively. For those {\eus} with low valuation (i.e., $\th \in [ \max\{\thlb, \thla\}, 1]$) values the free basic service than the quality of \ch. Only the {\eus} with median value would value the \db's advanced service which provides better service than the basic service does and charges less fee than the leasing service.
%\com{This paragraph basically repeats Figure 1. The more important question is what are the insights and intuitions behind these observations? }
%In the former, all \eus~with $\th \in (0, \thab)$ prefer to randomly access to the TV channel, all \eus~with $\th \in (\thab, \thla)$ prefer to subscribe to the advanced service of the \db, and the \eus~with $\th \in (\thla, 1)$ prefer to lease licensed spectrum.
%In the latter case, the \eus~with $\th \in (0, \thlb)$ prefer to randomly access to the TV channel, all \eus~with $\th \in (\thlb,1)$ prefer to lease licensed spectrum.
%Because the type of the \eus~is uniformly distributed, the new derived market shares $\{ \Probl,\Proba \}$ given the initial market share $\{\Probl^0, \Proba^0 \}$ are
%\begin{itemize}
%\item
%If $\thlb > \thab$, then $\Probl = 1 -  \thla$ and $\Proba  = \thla - \thab$;
%\item
%If $\thlb \leq \thab$, then $\Probl = 1 - \thlb$ and $\Proba  = 0$.
%\end{itemize}
%Formally, we summarize the above derived market shares in the following lemma.

%\begin{lemma}\label{lemma:market-share}
%Given the initial market share $\Probl^0$ and $\Proba^0$, the derived market shares of the \lh~$\Probl$ and of the \db~$\Proba$ are
%\begin{equation}\label{eq:user-prob-1}
%\begin{aligned}
%\Probl(\Probl^0, \Proba^0) & \textstyle
%= \max \big\{ 1 - \max\{ \thla, \thlb \} ,\ 0  \big\},\\
%\Proba(\Probl^0, \Proba^0)  & \textstyle
%= \max \big\{ \min\{ \thla ,1 \} - \thab ,\ 0  \big\}.
%\end{aligned}
%\end{equation}
%\end{lemma}

%The results in Lemma \ref{lemma:market-share} assume that all \eus~change their choices simultaneously. Note that $\thlb$, $\thab$ and $\thla$ are functions of the initial market shares $\Probl^0$ and $\Proba^0$ (as $\RB$ and $\RA$ are functions of $\Probl^0$ and $\Proba^0$). Thus, the derived market shares $\Probl$ and $\Proba$ are also functions of  $\Probl^0$ and $\Proba^0$, and can be written as $\Probl(\Probl^0, \Proba^0)$ and $\Proba(\Probl^0, \Proba^0)$.
%
%\textbf{Case II: $\RB < \RL < \RA$.}
%The analysis in Case II is similar to that in Case I, and we can directly use the result in Case I by swapping the position of $\RL$ and $\RA$.
%
%\textbf{Case III: $\RL < \RB < \RA$.}
%In such case, no {\eus} will chose leasing licensed spectrum. All {\eus} only make the choice between the \db's basic service and advance service. This is the pure information market for the TV white space network and has been analyzed in \cite{luo2014wiopt}. Later, we will compare our hybrid market model with the pure information market.

%Figure \ref{fig:demand} illustrate the derived market shares of the \lh~and \db~. The \lh's market share becomes more price elastic when the leasing price exceeds $\thab \cdot (L -B)$ as shown in Figure \ref{fig:demand}.a. This is because the \lh~loses \eus~to the \db's \TVWS~service. When the leasing price is high, some of the \eus~will find that the \db's \TVWS~service is the best choice even though they have to give up some expected data rate $L - A$.
\vspace{-3mm}
\subsection{{Market Dynamics and Equilibrium}}

When the market shares change,
%the information structure will also change according to (\ref{eq:known_inf}) and (\ref{eq:unknown_inf}).
the users' payoffs (on the advanced service and basic service) change accordingly, as $\RA$ and $\RB$ change.
As a result, users will update their best strategies continuously, hence the market shares will evolve dynamically, until reaching a {stable} point (called \emph{market equilibrium}).
In this subsection, we will study such a market dynamics and equilibrium, given the prices $\{ \pl, \pa \}$.~~~~~~~~~~~~~~~~~~~


For convenience, we introduce a virtual time-discrete system with slots $\t=1,2,\ldots$, where {\eu}s change their decisions at the beginning of every slot, based on the derived market shares in the previous slot.
Let $( \Probl^{\t}, \Proba^{\t} )$ denote the market shares derived at the end of slot $t$ (which serve as the initial market shares in the next slot $t+1$).
%Take a particular slot $t$ as an example.
%The initial market shares is $( \Probl^{\t-1}, \Proba^{\t-1} )$ obtained in the previous slot $\t-1$,  and
%the derived market share $( \Probl^{\t}, \Proba^{\t} )$ in the current slot $t$ is given by Lemma \ref{lemma:market-share}.
%Note that $( \Probl^{\t}, \Proba^{\t} )$ are derived from $( \Probl^{\t-1}, \Proba^{\t-1} )$ according to Lemma \ref{lemma:market-share}.
We further denote $\triangle \Probl  $ and $\triangle \Proba $ as the changes (dynamics) of market shares between two successive time slots, e.g., $\t$ and $\t+1$, that is,
\begin{equation}\label{eq:user-prob-diff}
\begin{aligned}
\textstyle
\triangle \Probl(\Probl^{\t}, \Proba^{\t}) &= \Probl^{\t+1} - \Probl^{\t }, ~
\triangle \Proba(\Probl^{\t}, \Proba^{\t}) &= \Proba^{\t+1} - \Proba^{\t },
\end{aligned}
\end{equation}
where $( \Probl^{\t+1}, \Proba^{\t+1} )$ are the derived market share in slot $\t+1$, which can be computed by Lemma \ref{lemma:market-share}.
%A positive (negative) $\triangle \Probl$ (or $\triangle \Proba$) implies that the market share $\Prob$ (or $\Prob$) will increase (decrease) along the dynamics.
%Note that both $\triangle \Probl $ and $\triangle \Probl $ are the functions of $\Probl^{\t-1}$ and $\Proba^{\t-1}$. Hence, we can write $\triangle \Probl $ and $\triangle \Proba$ as  $\triangle \Probl(\Probl^{\t-1}, \Proba^{\t-1})$ and $\triangle \Proba(\Probl^{\t-1}, \Proba^{\t-1})$.
Obviously, if both $\triangle \Probl $ and $\triangle \Proba $ are zero in  a slot $\t+1$, i.e., $\Probl^{\t+1} = \Probl^{\t} $ and $\Proba^{\t+1} = \Proba^{\t} $, then users will no longer change their strategies in the future. This implies that the market achieves a stable state, which we call the \emph{market equilibrium}.
Formally,

%A \emph{market equilibrium} is defined as a fixed point of the market shares.
%In other words, if an equilibrium market share is achieved, it will not change any more. Formally,
\vspace{-2mm}
\begin{definition}[Market Equilibrium]\label{def:stable-pt}
A pair of market shares $\BProb^{*} = \{ \Probl^{*}, \Proba^{*} \}$ is a market equilibrium, if and only if
\begin{equation} \label{eq:market_equilibrium}
\textstyle
\triangle \Probl (\Probl^*, \Proba^*) = 0, \mbox{~~~and~~~}
\triangle \Proba (\Probl^*, \Proba^*) = 0.
\end{equation}
\end{definition}

Next, we study the existence and uniqueness of the market equilibrium, and further characterize the market equilibrium analytically.
These results are very important for analyzing the price competition game in Layer II (Section \ref{sec:layer2}).
\vspace{-2mm}
\begin{proposition}[Existence]\label{lemma:existence-eq_pt}
Given any feasible price pair $( \pl, \pa)$,
there exists at least one market equilibrium.
\end{proposition}
\vspace{-3mm}
\begin{proposition}[Uniqueness]\label{lemma:uniqueness-eq_pt}
Given any feasible price pair $( \pl, \pa)$,
there exists a unique market equilibrium $(\Probl^*, \Proba^*)$, if there exists a tuple $(\Probl, \Proba)$ with $\Probl + \Proba \leq 1$ such that\footnote{{Here, $\gy^{\prime}(\Proba)$ is the first-order derivative of $\gy(\cdot)$ with respect to $\Proba$. Note that $\RA$ is a function of $\Proba$ and $\Probl$, and $\RB$ is a function of $\Probl$.}}
%\begin{equation}\label{eq:stable_condition}
%\textstyle
%\max_{\Probl, \Proba \in [0,1]}  \gy^{'}(\Proba) \cdot \left[ \frac{ \pl - \pa }{ ( L - \fx(\Probl) - \gy(\Proba) )^2} + \frac{ \pa }{ \gy^2(\Proba) } \right]   \leq 1
%\end{equation}
%\end{proposition}
\begin{equation}\label{eq:stable_condition}
%\max_{\Probl, \Proba \in [0,1]}
\textstyle
%\max_{\Proba \in [0,1]} \frac{ \gy^{\prime}(\Proba) }{ \gy(\Proba)  } \cdot \frac{ \RL - \RB(\Probl, \Proba)  }{ \RL - \RA(\Probl, \Proba) }  \leq 1,\quad \forall \Probl, \Proba \in [0,1].
{ \frac{ \gy^{\prime}(\Proba) }{ \gy(\Proba)  } \cdot \frac{ \RL - \RB }{ \RL - \RA }  \leq 1.}
\end{equation}
\end{proposition}
%\com{explain what $\gy^{\prime}(\Proba)$ means. The A and B here: are they function of the initial market share, or for ANY values of $\eta_A$ and $\eta_L$? initial market share with superscript 0? }
%\com{Yuan: Since the condition is the function of $\eta_A$ and $\eta_L$, hence, we should find a market share pair $\{\eta_L, \eta_A \}$ such that the upper bound of $\frac{ \gy^{\prime}(\Proba) }{ \gy(\Proba)  } \cdot \frac{ \RL - \RB(\Probl, \Proba)  }{ \RL - \RA(\Probl, \Proba) }$ is less than $1$.}

%\begin{proof}
%The proof sketch for the existence of market equilibrium is as follows.
%By Definition \ref{def:stable-pt}, $\BProb^{*} = \{ \Probl^{*}, \Proba^{*} \}$ is an equilibrium point if and only if it is a solution of (\ref{eq:market_equilibrium}). By substitution, we can transform (\ref{eq:market_equilibrium}) with two variables $\{ \Probl, \Proba \}$ into function $\Phi(\Proba) = 0$ with one variable $\Proba \in [0,1]$ only. We can check that $\left.\Phi(\Proba)\right|_{\Proba = 0}  > 0$ and $\left.\Phi(\Proba)\right|_{\Proba = 1}  < 0$. As $\Phi(\cdot)$ is continuous on $[0,1]$, we can get the conclusion that $\Phi(\Proba) = 0$ has a root on the domain of $\Proba$. By plugging the solution of $\Phi(\Proba) = 0$ into (\ref{eq:market_equilibrium}), we can get the corresponding solution of $\Probl$. Hence, we can show the existence of market equilibrium.
%In order to proof the uniqueness, we only need to show that the function $\Phi(\cdot)$ is strictly decreasing on $[0,1]$ if the condition (\ref{eq:stable_condition}) is satisfied.
%\end{proof}

\begin{figure}
\centering
%  \includegraphics[width=2.5in]{fig_user_subscription_dynmics_quiver.pdf}
  \includegraphics[width=2.8in]{fig_user_subscription_dynamics2}
  \caption{Illustration of Market Dynamics and Market Equilibrium. Red Curve:  $\triangle \Probl(\Probl, \Proba) = 0$; Blue Curve: $\triangle \Proba(\Probl, \Proba) = 0$. The intersection between   blue   and red curve is the market equilibrium.}
%  $\pl = 1.56$ and $\pa = 0.52$.
  \label{fig:dyna-users}
%  \caption{Dynamics of the market shares $\Prob_1$ and $\Prob_2$.
%From the initial market shares ${\BProb}_a^0 = \{0.3,0.1\}$, the market shares will gradually evolve to $\BProb_a^1,\ \BProb_a^2,\ ...\ $, and eventually achieves the equilibrium $\BProb_a^*$ located on the top-left corner.
%From the initial market shares $\BProb_b^0=\{0.4,0.05\}$, the market shares will evolve to the equilibrium $\BProb_b^*$ located on the bottom-right corner.}\label{fig:dyna-p2-2}
  \vspace{-6mm}
\end{figure}

A practical implication of (\ref{eq:stable_condition}) is that if the information value $\gy(\Proba)$ (positive network externality) does not increase very fast with $\Proba$, then there exists a unique equilibrium.
Note that the condition (\ref{eq:stable_condition}) is sufficient but not necessary for the uniqueness.
In particular, we observe through numerical simulations that in some cases, the market converges to a unique equilibrium for a wide range of prices under which the condition (\ref{eq:stable_condition}) is violated.
Nevertheless, the sufficient condition in (\ref{eq:stable_condition}) leads to the insight that if the impact of positive network externality is significant, there may exist multiple equilibrium points.
Note that even if there exist multiple equilibrium points,
%\rev{a similar policy as that in \cite{luo2014wiopt} is needed to make sure the \db~has a large initial market share.}
the market always converges to a unique one of them, given the initial market shares. {Please refer to \cite{report} for more details.}
%\com{How to prove this? How do we know that the dynamics will not enter loops? }

%A practical implication of the derived uniqueness condition is as follows. If attracting one advanced {\eu} can significantly increases the utility provided by the advanced service (i.e., $g^{'}(\Proba)$ is larger than $\gy(\Proba)$), it is better for the \db~not to provide the \lh's leased \ch~information.
%Moreover, a similar policy as that in \cite{luo2014wiopt} is needed to make sure the \db~has a large initial market share. On the contrary, if the congestion effect is a dominant network effect, providing the licensed \ch's information can alleviate the congestion effect of the TV white space network and guarantee the stable of the system.
%\com{This explanation is based on the new derived Proposition \ref{lemma:uniqueness-eq_pt}.}

For a better understanding, we illustrate the dynamics of market shares in Figure \ref{fig:dyna-users}.
The $x$-axis denotes the leasing service's market share-$\Probl$, and the $y$-axis denotes the advanced service's market share-$\Proba$.
Notice that a feasible pair of market shares $\{\Probl, \Proba\}$ satisfies $\Probl + \Proba \leq 1$.
An arrow denotes the dynamics of market shares under a particular initial market shares (at the starting point of the arrow).
For example, {from the initial market shares $\BProb^{0} = \{\Probl = 0.6, \Proba = 0\}$, the  market will evolve to $\BProb^{1} = \{0.32, 0.16\}$, then $\BProb^{2} = \{0.35, 0.2\}$, and eventually converge to the equilibrium point $\BProb^{*} = \{0.33,0.24\}$.}
%\rev{the  market will evolve to $\BProb^{1} = \{\Probl = 0.32, \Proba =0.16\}, \BProb^{2} = \{\Probl = 0.35, \Proba =0.2\} $ and eventually achieves the equilibrium market share $\BProb^{*} = \{\Probl^{*} = 0.33, \Proba^{*} =0.24\}$.}
%\com{It is a bit confusing, as the arrow from (1,0) does not land at (0.2, 0.2). I understand that the figure might become messy if the arrow is from (1,0) to (0.2, 0.1). See how we can explain this better. }
The red curve denotes the isoline of $\triangle \Probl(\Probl, \Proba) = 0$,  and the blue curve denotes the isoline of $\triangle \Proba(\Probl, \Proba) = 0$.
By Definition \ref{def:stable-pt}, the intersection between the blue curve and the red curve is the market equilibrium point.
In this example, there is a unique market equilibrium point.
%Based on the above two Propositions, the following Theorem provides equations characterizing the stable market equilibrium.

Suppose the uniqueness condition (\ref{eq:stable_condition})  is satisfied. We characterize the unique equilibrium by the following theorem.
\vspace{-2mm}
\begin{theorem}[Market Equilibrium]\label{thrm:stable-eq_pt}
Suppose the uniqueness condition (\ref{eq:stable_condition}) holds.
Then, for any feasible price pair $( \pl, \pa)$, the unique market equilibrium is given by
\begin{itemize}
\item[(a)]
If $ \left.\thlb(\Probl, \Proba)\right|_{\Probl = 0} \leq \left.\thab(\Probl, \Proba)\right|_{\Proba = 0}$, then there is a unique market equilibrium  $\BProb^{\dag} = \{ \Probl^{\dag}, \Proba^{\dag} \}$ given by
%    $\Prob^*_1 = 0$, and  $\Prob^*_0$ satisfies
    \begin{equation}\label{eq:NE-pt-1}
%   \left\{
%      \begin{aligned}
 \textstyle  \Probl^{\dag} = 1 - \thlb(\Probl^{\dag},\Proba^{\dag}) , \mbox{~~~and~~~}
  \Proba^{\dag} = 0;
%       \end{aligned}
%    \right.
      %\textstyle  1 - \pth_{02}(\Prob^*_0) - \Prob^*_0 = 0;
    \end{equation}

\item[(b)]
If $ \left.\thlb(\Probl, \Proba)\right|_{\Probl = 0} > \left.\thab(\Probl, \Proba)\right|_{\Proba = 0}$, then there is a unique market equilibrium  $\BProb^{*} = \{ \Probl^{*}, \Proba^{*} \}$ given by
    \begin{equation}\label{eq:NE-pt-22}
    \left\{
      \begin{aligned}
      &\textstyle  \Probl^{*} = 1 - \thla(\Probl^{*}, \Proba^{*}) , \\
      &\textstyle  \Proba^{*} = \thla(\Probl^{*}, \Proba^{*}) - \thab(\Probl^{*}, \Proba^{*}).
       \end{aligned}
    \right.
    \end{equation}
\end{itemize}
\end{theorem}

\begin{proof}
First, we obtain the derived market shares by substituting the market shares given in (\ref{eq:NE-pt-1}) or (\ref{eq:NE-pt-22}) into (\ref{eq:user-prob-1}).
Then, we can check the above derived market shares satisfy the equilibrium condition (\ref{eq:market_equilibrium}).
For the detailed proof, please refer to \cite{report}.
%The proof sketch is as follows. By utilizing a similar proof method in Proposition \ref{lemma:existence-eq_pt} and Proposition \ref{lemma:uniqueness-eq_pt}, we can get the conclusion according to Lemma \ref{lemma:market-share}.
\end{proof}

%Suppose $\BProb^{*} = \{ \Probl^{*}, \Proba^{*} \}$ is the unique market equilibrium under prices $\{\pl, \pa\}$, then we can write the unique market equilibrium $\BProb^{*} = \{ \Probl^{*}, \Proba^{*} \}$
%as functions of $\{\pl, \pa\}$.

%Finally, we provide some useful properties for the market equilibrium,  regarding the changing of prices $\{\pa, \pl\}$, which are useful for analyzing the price competition game in Layer II  (Section \ref{sec:layer2}).
%%\begin{property}
%Suppose $\BProb^{*} = \{ \Probl^{*}, \Proba^{*} \}$ is the unique market equilibrium under prices $\{\pl, \pa\}$. Then, we have
%\begin{itemize}
%\item
%$\Probl^{*}\in[0,1] $ is decreasing in $\pl $, and increasing with $\pa$;
%\item
%$\Proba^{*}\in[0,1] $ is decreasing in $\pa $, and increasing with $\pl$.
%\end{itemize}
%%\end{property}
%Hence, we can write the unique market equilibrium $\BProb^{*} = \{ \Probl^{*}, \Proba^{*} \}$
%as functions of $\{\pl, \pa\}$.



















==> Latex_ParticipateSensing_infocom_camera/Section_network_effect.tex <==

\section{The Value of Information and the Network Effect}
%If a \eu~chooses operating on TV \ch, it can only operate on one of the available TV \chs from the \ch~set $\Kset = \{ 1,\ldots, \K \}$ at a particular time on the shared basis (i.e., each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques).
%Let $\Kset = \{ 1,\ldots, \K \}$ denote the set of available TV channels in this area. One \eu~can only operate on \emph{one} of the available \chs~at a particular time on the shared basis (i.e., each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques).
%
%Each \eu~makes its choice through the online platform provided by a \db. We assume that a \db~has the available TV \chs~information and provides such information to each querying \eu~in order to let the \eu~operate on \emph{one} of the available \chs~at a particular time. Note that each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques.
%We also assume that the licensed spectrum holders display their licensed spectrum

For each {\eu} $n\in \Nset$, each channel $\k$ is associated with an \emph{interference level}, denoted by  $\InfTot_{\n,\k}$, which reflects the aggregate interference from all other nearby devices (including TV stations
%\footnotesc{{Notice each TV station has the right to transmit on a particular channel within certain coverage area centered around the TV station, and unlicensed users may be allowed to transmit in this coverage \emph{with a strictly constrained power}. Hence, the TV station might generate interference to unlicensed users (whereas the reverse is not allowed).}}
and other {\eus}) operating on this channel.
%For convenience, we also refer to $\InfTot_{\k}$ as the \emph{quality} of channel $k$.
Due to the fast changing of wireless channels and the uncertainty of {\eus}' mobilities and activities, the interference $\InfTot_{\n,\k}$ is a random variable.
For convenience, we assume that
$$
\InfTot_{\n,\k} \mbox{ is \emph{temporal-independence} and \emph{frequency-independence}}.
$$
That is,
(i) the interference $\InfTot_{\n,\k}$ on channel $\k$ is independent identically distributed (iid) at different times, and (ii)
the interferences on different channels, $\InfTot_{\n,\k}, \k\in\Kset$, are also iid at the same time.\footnotesc{Note that the iid assumption is a reasonable approximation of the practical scenario, where all channel quality distributions are the same but the realized instant qualities of different channels are different (e.g., \cite{chang2009channel,jiang2009channel,zhou2011channel}).}
%Under the i.i.d. assumption, we assume that all channel states $\{ \InfTot_{\k} \}_{\k \in \Kset}$ have the same cumulative distribution function (CDF)
As we are talking about a general WSD $n$, \textbf{we will omit the WSD index $n$ in the notations (e.g., write $\InfTot_{\n,\k}$ as $\InfTot_{\k}$), whenever there is no confusion caused.}
Let $F_{\InfTot}(\cdot)$ and $f_{\InfTot}(\cdot)$ denote the cumulative distribution function (CDF) and probability distribution function (PDF) of $\InfTot_{\k}$, $\forall \k\in\Kset$.\footnotesc{In this paper, we will conventionally  use $F_X(\cdot)$ and $f_X(\cdot)$ to denote the CDF and PDF of a random variable $X$, respectively.}~~~~

For convenience, we illustrate the basic service and advanced service by the example in the following table.
In the basic service, the database provides the available channel set (i.e., \{CH1, CH3, CH4, CH6\}) to a particular \eu. In the advanced service, the database provides the interference levels on available channels (i.e., \{$\InfTot_1$, $\InfTot_3$, $\InfTot_4$, $\InfTot_6$\}) to the \eu, in addition to the available channel set.

\begin{table}[h]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Channel ID} & \textbf{CH1}& \textbf{CH2}& \textbf{CH3} & \textbf{CH4} & \textbf{CH5} & \textbf{CH6}
\\
\hline
Availability & Yes & No & Yes & Yes & No & Yes
\\
\hline
Interference Level & $\InfTot_1$ &  - & $\InfTot_3$ & $\InfTot_4$ &  - & $\InfTot_6$
\\
\hline
\end{tabular}
\end{table}


\textbf{Interference Level (Information).}
{For a particular {\eu}}, its experienced interference $\InfTot_{\k}$ on a channel $k$ is the aggregate interference from all other (nearby) devices operating on channel $k$,
and usually consists of the following three components:
\begin{enumerate}
\item
$\InfTV_{\k}$: the interference from licensed TV stations;
\item
$\InfEU_{\k,m}$: the interference from another {\eu} $m$ operating on the same channel $k$;
\item
$\InfOut_{\k}$: any other interference from outside systems.
\end{enumerate}
%Here $\InfEU_{\n,\k}$ denotes the interference from an {\eu} $\n$ operating on channel $\k$, and
The total interference on channel $k$ is
$
\InfTot_{\k} = \InfTV_k + \InfEU_k + \InfOut_k
$, where  $\InfEU_k  \triangleq \sum_{m \in \Nkset} \InfEU_{\k,m}$ is the total interference from all other {\eus} operating on channel $k$ (denoted by $\Nkset$).
Similar to $\InfTot_{\k}$, we assume that  $ \InfTV_k , \InfEU_k , \InfEU_{\k,m}$, and $ \InfOut_k$ are random variables with \emph{temporal-independence} (i.e., iid across time) and \emph{frequency-independence} (i.e., iid across frequency).
We further assume that $\InfEU_{\k,m}$ is \emph{user-independence}, i.e., $\InfEU_{\k,m}, m\in \Nkset$, are iid.
%Similarly, we assume that $\{ \InfTV_k \}_{\k \in \Kset}$ are i.i.d., with the CDF $F_{\InfTV}(\cdot)$, and
%$\{ \InfOut_k \}_{\k \in \Kset}$, are i.i.d., with the CDF $F_{\InfOut}(\cdot)$.
%Let $F_{\InfTV}(\cdot)$, $F_{\InfEU}(\cdot)$, and $F_{\InfOut}(\cdot)$ denote the CDFs of $ \InfTV_k , \InfEU_{\n,\k}$, and $\InfOut_k $, respectively.
{It is important to note that \textbf{different {\eus} may experience different interferences $\InfTV_k$ (from TV stations), $ \InfEU_{\k,m} $ (from another WSD), and $ \InfOut_k$ (from outside systems) on a channel $k$, as we have omitted the \eu~index $n$ for all these notations for clarity.}}

Next we discuss these interferences in more details.

\begin{itemize}
\item
Each database is able to compute the interference $\InfTV_k$ from TV stations to every {\eu} (on channel $k$), as it knows the locations and channel occupancies of all TV stations.~~~~
%\footnotesc{Here we consider the long-term average interference, not the instantaneous interference. The same applies to {\eu} and outside interference.}

\item
Each database cannot compute the interference
$\InfOut_k$ from outside systems, due to the lack of outside interference source information.
%\footnotesc{Such outside interference may come from WSDs interacting with other databases, different wireless systems operating on the same or nearby frequency bands, etc.}
Thus, the interference $\InfOut_{\k}$ will \emph{not} be included in a database's information sold to {\eus}.~~~~~~~~
%This reduces the accuracy of information.

\item
Each database may or may not be able to compute the interference $\InfEU_{\k,m}$ from another {\eu} $m$, depending on whether {\eu} $m$ subscribes to the database's advanced service.
Specifically, if {\eu} $m$ subscribes to the advanced service, the database can predict its channel selection (since the {\eu} is fully rational and will always choose the channel with the lowest interference level indicated by the database at the time of subscription), and thus can compute its interference to any other \eu.
However, if {\eu} $m$ does not subscribe to the advanced service, the database cannot predict its channel selection, and thus cannot compute its interference to other \eus.~~~~
\end{itemize}


For convenience, we denote $\Nkset^{[l]},l\in\{1,2\}$, as the set of {\eus} operating on channel $k$ and subscribing to the database $\dbb_l$'s advance service (i.e., those choosing the strategy $\l \in\{1,2\}$), and $\Noset$ as the set of {\eus} operating on channel $k$ and \emph{not} subscribing to any advance service (i.e., those choosing the strategy $\l = 0$).
That is, $\Nkset^{[1]} \bigcup \Nkset^{[2]} \bigcup \Noset = \Nkset $.
Then, for a particular WSD, its experienced interference (on channel $k$) \textbf{known by database $\dbb_l$} is
% (and thus will be included in the database $\dbb_i$'s advanced service to this WSD) is
\begin{equation}\label{eq:known_inf}
\begin{aligned}
\textstyle
\InfKnown_{\k}^{[l]} \triangleq \InfTV_{\k} + \sum_{m \in \Nkset^{[l]}} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from TV licensees and all {\eus} (operating on channel $k$)  subscribing to the database $\dbb_l$'s advanced service.
The WSD's experienced interference (on channel $k$) \textbf{\emph{not} known by database $\dbb_l$} is
% (and thus will not be included in the database $\dbb_i$'s advanced information) is
\begin{equation}\label{eq:unknown_inf}
\begin{aligned}
\textstyle
\InfUnknown_{\k}^{[l]}  \triangleq \InfOut_{\k} +\sum_{m \in \Noset} \InfEU_{\k,m} + \sum_{m \in \Nkset^{[i]},i\neq l} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from outside systems and all {\eus} (operating on channel $k$) not subscribing to the database $\dbb_l$'s advanced service.
Obviously, both $\InfUnknown_{\k}^{[l]}$ and $\InfKnown_{\k}^{[l]}$ are also random variables with temporal- and frequency-independence.
Accordingly, the total interference on {\ch} $\k$ for a WSD can be written as
%\begin{equation}\label{eq:total_inf_new}
%\begin{aligned}
$\textstyle
\InfTot_{\k} = \InfKnown_{\k}^{[l]} + \InfUnknown_{\k}^{[l]}.$~~~~~~
% = \InfTV_{\k} +\InfOut_{\k}+ \sum_{n \in \Nkset} \InfEU_{\n,\k}.
%\end{aligned}
%\end{equation}

\textbf{Since the database $\dbb_l$ knows only $\InfKnown_{\k}^{[l]}$, it will provide this information (instead of the total interference $\InfTot_k$) as the {advanced service} to a subscribing {\eu}.}
%to its advanced service.
It is easy to see that the more {\eus} subscribing to the database $\dbb_l$'s advanced service, the more information the database $\dbb_l$ knows, and the more accurate the database $\dbb_l$'s information will be.~~~~~~~~


Next we can characterize the accuracy of a database's information explicitly.
Due to the frequency independence assumption, it is reasonable to assume that each channel $k\in\Kset$ will be occupied by an average of $\frac{\N}{\K}$ {\eus}.
Let $\Prob_l$ denote the percentage of {\eus} subscribing to the advanced service of database $\dbb_l$ (called the \emph{market share} of database $\dbb_l$).
%Notice that each {\eu} will
%be ``assigned'' to each channel with an equal probability due
%to the assumption of the frequency independence.
Then, among all  $\frac{\N}{\K}$ {\eus} operating on channel $k$, there are, \emph{on average}, $\frac{\N}{\K}\cdot\Prob_l$ {\eus}  subscribing to the database $\dbb_l $'s advanced service, and $\frac{\N}{\K}\cdot(1-\Prob_1 -\Prob_2)$ {\eus} not subscribing to any advanced service.
That is, $| \Nkset | = \frac{\N}{\K}$, $| \Nkset^{[l]} | = \frac{\N}{\K}\cdot\Prob_l, \forall l\in\{1,2\}$, and $|\Noset | = \frac{\N}{\K}\cdot(1-\Prob_1-\Prob_2)$.\footnotesc{{Note that the above discussion is from the aspect of expectation, and in a particular time period, the realized numbers of {\eus} in different channels may be different.}}
Finally, by the {user-independence} of $\InfEU_{\k,m}$, we can immediately calculate the distributions of $ \InfKnown_{\k}^{[l]}$ and $ \InfUnknown_{\k}^{[l]}$ under any given market share $\Prob_l$ via (\ref{eq:known_inf}) and (\ref{eq:unknown_inf}).

%That is, there are an average $\N\cdot \Prob_1$ {\eus} subscribing to the $\dbb_1$'s advanced service, $\N\cdot \Prob_2$ {\eus} subscribing to the $\dbb_2$'s advanced service, and $\N\cdot (1-\Prob_1 - \Prob_2)$ {\eus} not subscribing to the advanced service.
%%Suppose the {\eu} number $\N$ is very large, and
%Since the {\eus} are independent with each other,  then, from a system perspective, all the {\eus} will be ``assigned'' to all available channels equally (i.e., $|\Nset_k| = \frac{\N}{\K}$).
%That is,
%on every available channel $k$, there are on average $\frac{\N}{\K}\cdot\Prob_{\i} $ {\eus} subscribing to the advanced serve of database $\i$ (whose interference (to any particular {\eu}) can be computed by the database) where $ \i \in \{ 1, 2\}$, and $\frac{\N}{\K}\cdot(1-\Prob_1 - \Prob_2)$ {\eus} not subscribing to the advanced serve (whose interference cannot be computed by the database)\footnotesc{This is because of the diversity of users' locations as well as their
%environments. The good channels for a user may not be good for others.
%Moreover, even if users share the similarity in the environment, they
%are likely to be directed to different channels for the purpose of
%interference avoidance.}.
%Similarly, we assume that the interference from single {\eu} {$\{\InfEU_{\n, \k}\}_{\n \in \Nkset}$}, are iid with a CDF   $F_{\InfEU}(\cdot)$.
%
%
%%We denote these three kinds of interference for \ch~$\k$ as random variable $\InfTV_{\k}$, and $\InfOut_{\k}$. We let random variable $\InfEU_{\n}$ as \eu $\n$'s interference.
%%We denote these three kinds of interference as random variable $\InfTV$, $\InfOut$, and $\InfEU$, respectively.
%%We also assume $\{ \InfTV_{\k} \}_{\k \in \Kset}$, $\{ \InfOut_{\k} \}_{\k \in \Kset}$, and $\{ \InfEU_{\n} \}_{\n \in \Nset}$ are i.i.d. random variables.
%%Let $F_{\InfTV}(\cdot)$, $F_{\InfOut}(\cdot)$, and $F_{\InfEU}(\cdot)$ denote the CDF of above three random variable. And correspondingly, let $f_{\InfTV}(\cdot)$, $f_{\InfOut}(\cdot)$, and $f_{\InfEU}(\cdot)$ denote their probability density function (PDF).
%
%%As we assume the total number of \eus~$\N$ is very large, we can consider \eus~are uniformly assign to each \ch,~i.e., there are ${ \N }/{\K}$ \eus~in each \ch.
%%Hence, the total interference level of \ch~$\k$ is:
%%\begin{equation}\label{eq:total_inf}
%%\begin{aligned}
%%%\textstyle
%%\vspace{2mm}
%%\InfTot_{\k} \triangleq \InfTV_{\k} +\InfOut_{\k}+ \frac{\N}{\K} \cdot \InfEU
%%\vspace{2mm}
%%\end{aligned}
%%\end{equation}
%
%%Since every \eu~needs to report its location to \db, \db~can calculate the TV station's interference to each \eu. Hence, \db~knows the distribution of $\InfTV$.
%%As we assume that advanced \eu~will choose the \ch~with highest ranking, therefore, \db~can also calculate the total interference caused by advanced \eu. We denote $\Prob$ as the percentage of advanced \eus \footnotesc{"percentage of advanced \eus" is used throughout this paper to mean the proportion of \eus~in the market that subscribe to advanced service}~. Then, the number of advanced \eus~is $\N \cdot \Prob$. As we assume $\N$ is very large, we can consider both advanced \eus~and basic \eus~are uniformly assign to each \ch,~i.e., there are $\frac{ \N \cdot \Prob }{\K}$ advanced \eus~and $\frac{ \N \cdot (1-\Prob) }{\K}$ basic \eus~in each \ch.
%
%In summary, for each \ch~$\k$, the interference level known by the \db~$\i$ is
%\begin{equation}\label{eq:known_inf}
%\begin{aligned}
%\textstyle
%\InfKnown^{\i}_{\k} \triangleq \InfTV^{\i}_{\k} + \sum_{n \in \Naiset} \InfEU_{\n, \k}~\i = \{ 1 , 2\}.
%%\sum_{n=1}^{\frac{ \N }{\K}  \cdot \Prob_{\i}} \InfEU_{n},~\i = \{ 1 , 2\}.
%\end{aligned}
%\end{equation}
%The interference level not known by the \db~$\i$ is
%\begin{equation}\label{eq:unknown_inf}
%\begin{aligned}
%\textstyle
%\InfUnknown^{\i}_{\k} \triangleq \InfOut^{\i}_{\k} + \sum_{n \in \Noset} \InfEU_{n, \k} + \sum_{n \in \Najset} \InfEU_{n, \k}~\j \neq \i.
%%\InfUnknown^{\i}_{\k} \triangleq \InfOut^{\i}_{\k} + \sum_{n=1}^{\frac{ \N  }{\K}\cdot (1 - \Prob_{\i} - \Prob_{\j})} \InfEU_{n} + \sum_{n=1}^{\frac{ \N  }{\K}\cdot \Prob_{\j}} \InfEU_{n}~\j \neq \i.
%\end{aligned}
%\end{equation}
%The total interference level  on  \ch~$\k$ is
%\begin{equation}\label{eq:total_inf_new}
%\begin{aligned}
%\textstyle
%\InfTot_{\k} = \InfKnown_{\k} + \InfUnknown_{\k} = \InfTV_{\k} +\InfOut_{\k}+ \sum_{n \in \Nkset} \InfEU_{\n,\k}
%\end{aligned}
%\end{equation}
%where $\Naiset$ denotes the set of {\eus} operating on the channel $k$ and subscribing to the advance service of database $\i$; $\Najset$ denotes the set of {\eus} operating on the channel $k$ and subscribing to the advance service of database $\j \neq \i$; $\Noset$ denotes the set of {\eus} operating on the same channel $k$ and not subscribing to the advance service of both database, and $\Nkset$ denotes the set of {\eus} operating on the same channel $k$. Besides, we have $|\Naiset| = \frac{N}{K}\cdot{\eta_i}$, $|\Najset| = \frac{N}{K}\cdot{\eta_j}$, and $|\Noset| = \frac{N}{K}\cdot( 1 - \eta_1 - \eta_2)$. Moreover, we have $\i, \j \in \{1 ,2 \}$, $\i \neq \j$, $\Nkset = \Naiset \bigcup \Najset \bigcup \Noset$, and $\Naiset \bigcap \Najset \bigcap \Noset = \emptyset$.
%The database knows the precise value of $\InfKnown_{\k}$ on every channel $k$, which will be provided for {\eus} who subscribing to the advanced service.
%It is easy to see that the more {\eus} subscribing to this advanced service, the more accurate the advanced information will be.
%%It is assumed that the \db~knows the realized value of $\InfKnown_{\k}$.
%{
%By the iid assumption on $\InfTV_{\k}$, $\InfEU_{\n,\k}$, and $\InfOut_{\k}$, we can easily find that (i) $\{ \InfKnown_{\k} \}_{ \k\in\Kset }$, are i.i.d., (ii) $\{ \InfUnknown_{\k}\}_{\k\in\Kset}$, are i.i.d., and (iii) $\{ \InfTot_{\k} \}_{ \k\in\Kset }$, are i.i.d..
%Finally, we assume that both the \db~and \eus~knows \emph{a priori} the distributions of $\InfTV_{\k}$, $\InfEU_{\n,\k}$, and $\InfOut_{\k}$, and therefore the distributions of $\InfKnown_{\k}$, $\InfUnknown_{\k}$, and $\InfTot_{\k}$ given the market share $\Prob$.
%}

\textbf{Information Value.}
Now we evaluate the value of database $\dbb_l$'s information to {\eus}, which is
reflected by the {\eu}'s benefit (utility) that can be achieved from this information.

We first consider the expected  utility of a {\eu} when not subscribing to any advanced service (i.e., $\l=0$).
In this case, the {\eu} will randomly select a channel from the available channel list, and its expected utility is
\begin{equation}\label{eq:rate-random-fixed}
\begin{aligned}
\textstyle
\RB   \textstyle \triangleq \ut(\R_0) = \ut\left(\int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z)\right),
%& \textstyle = \ut\left( \Ex_{\InfTot} \big[ \rt \left( \InfTot_{\k} \right) \big] \right)
%\\
%& \textstyle = \ut\left( \int_{z} \rt(z) \cdot f_{\InfTot}(z) \cdot \mathrm{d}z \right).
%\vspace{8mm}
\end{aligned}
\end{equation}
where $\R_0$ is the expected data rate given in (\ref{eq:rkgs}).
%By (\ref{eq:total_inf_new}), the distribution of $\InfTot$ is independent of the percentage of advanced {\eus} $\Prob$. Therefore, the value of $\RB$ is also independent of $\Prob$.
%and for an {\eu} with $\l = \S$, its expected utility is
%\begin{equation}\label{eq:rate-sense-fixed}
%\begin{aligned}
%\RS  & \textstyle  \triangleq \ut\left(\Rks\right) ,
%%=  \ut\left( \Ex_{\InfTotMin} \big[ \rt \left(\InfTotMin \right) \big] \right)
%%\\
%%&\textstyle= \ut\big( \K  \int_z \rt(z) \cdot [ 1 - F_{\InfTot}(z)]^{\K - 1} \cdot f_{\InfTot}(z) \cdot \mathrm{d}z \big),
%%\vspace{8mm}
%\end{aligned}
%\end{equation}
%where $\R^{(\G_i)} $ is the expected data rates defined in (\ref{eq:rkgs}).
Obviously, $\RB$ depends only on the distribution of the total interference $\InfTot_k$, while not on the specific distributions of $\InfKnown_k^{[l]}$ and $\InfUnknown_k^{[l]}$. This implies that the accuracy of the database $\dbb_l$'s information does not affect the utilities of those {\eus} not subscribing to its advanced service.


Then we consider the expected utility of a {\eu} when subscribing to the database $\dbb_l$'s advance service (i.e., $\l\in\{1,2\}$).
In this case, the {\db} $\dbb_l$ returns the interference $\{\InfKnown_{k}^{[l]}\}_{k\in\Kset}$ to the {\eu}, together with the basic information such as the available channel list.
%Notice that the total interference also includes the interference $\{\InfUnknown_{k}\}_{k\in\Kset} $ not provided by the database.
%\db~ranks the  {\chs} in ascending order given {\ch} interference level it known (i.e., $\InfKnown_{1}, \InfKnown_{2}, \ldots, \InfKnown_{\K} $). The ranked interference level are denoted by $\InfKnown_{(1)}, \InfKnown_{(2)}, \ldots, \InfKnown_{(\K)}$ and satisfy $\InfKnown_{(1)} < \ldots< \InfKnown_{(\K)}$.
For a rational {\eu}, it will always choose the channel with the minimum $\InfKnown_{k}^{[l]}$ (since $\{\InfUnknown_{k}^{[l]}\}_{k\in\Kset}$ are iid).
%\footnote{This is because the uncertain interference $\{\InfUnknown_{k}\}_{k\in\Kset} $ are i.i.d.}
Let $\InfKnownMin^{[l]} =  \min\{ \InfKnown_{1}^{[l]},  \ldots, \InfKnown_{K}^{[l]}  \} $ denote the minimum interference indicated by the database $\dbb_l$'s information.
Then, the actual interference experienced by a {\eu} (subscribing to the database $\dbb_l$'s advanced service) can be formulated as the sum of two random variables, denoted by $\InfTot^{[l]} = \InfKnownMin^{[l]} + \InfUnknown$. Accordingly, the {\eu}'s expected data rate and expected utility under the strategy $l\in\{1,2\}$ can be computed by
%Hence, the advanced {\eus} transmit at the {\ch} with lowest $\InfKnown$ and with total interference level $\InfTotA = \InfKnownMin + \InfUnknown$. Therefore, the advanced \eu's expect data rate is
\begin{equation}\label{eq:rate-pay-fixed}
\begin{aligned}
\Rl & \textstyle = \Ex_{\InfTot^{[l]}} \big[ \rt \left(\InfTot^{[l]} \right) \big] = \int_z \rt(z)  \mathrm{d} F_{\InfTot ^{[l]}}(z),
\\
\RA_l & \textstyle  \triangleq \ut\left(\Rl\right) = \ut\left(\int_z \rt(z)  \mathrm{d} F_{\InfTot ^{[l]}}(z)	\right) ,
% \textstyle =  \ut\left(\Ex_{\InfTotA} \big[ \rt \left(\InfTotA \right) \big] \right),
%\\
%&= \Ex_{\InfTotA} \big[ \rt \big( \InfKnownMin + \InfUnknown \big) \big] \\
%&= \K \cdot \int_{\InfTotA} \rt(z) \cdot \big[ \int_{\infty}^{\infty} f_{\InfKnown}(z -y) \cdot [ 1 - F_{\InfKnown}(y)]^{K-1} \cdot f_{\InfUnknown}(y) \mathrm{d}y  \big] \mathrm{d}z
%& \textstyle  = \ut \big( \int_z \rt(z) \cdot f_{\InfTotA}(z) \cdot \mathrm{d}z \big),
%\vspace{8mm}
\end{aligned}
\end{equation}
where
 $F_{\InfTot^{[l]}}(z)$ is the CDF of $\InfTot^{[l]}$.
% , and defined by
%\begin{equation*}\label{eq:min-known-pdf}
%%\begin{aligned}
%\textstyle
%f_{\InfTotA}(z) = \K   \int_y \big[ 1 - F_{\InfKnown}(z - y) \big]^{K-1} \cdot f_{\InfKnown}(z -y) \cdot f_{\InfUnknown}(y) \cdot \mathrm{d}y.
%%\vspace{8mm}
%%\end{aligned}
%\end{equation*}
It is easy to see that both $\Rl$ and $\RA_l$ depend on the distributions of $\InfKnown_k^{[l]}$ and $\InfUnknown_k^{[l]}$, and thus depend on the market share $\Prob_l$.
Thus, we will write $\RA_l$ as $\RA_l(\Prob_l)$.
We can further check that $\RA_l(\Prob_l)$ increases with $\Prob_l$.~~~~
%, because the more {\eus} subscribing to the database $\dbb_i$'s advanced service, the more accurate the database $\dbb_i$'s information, and further the more benefit for the {\eus} subscribing to the database $\dbb_i$'s advanced service.
%For convenience, we assume that $\RA_l(\Prob_l)$ is concave in $\Prob_l$ \rev{\footnote{This is validated by the simulation}}.~~~~~~~~~~~


%By (\ref{eq:rate-random-fixed})--(\ref{eq:rate-pay-fixed}), we can find the following useful properties.
%%, which are very important for the later analysis.
%
%\begin{proposition}
%%[Properties of $\RA, \RB, \RS$]
%\label{prop:ABS}
%~
%\begin{itemize}
%\item
% $\RB$ in (\ref{eq:rate-random-fixed})  does not depend on $\Prob_i$, $i\in\{1,2\}$;
% \item
% $\RA_i(\Prob_i)$ in (\ref{eq:rate-pay-fixed}) monotonously increases with $\Prob_i$;
% \item
% $\RA_i(\Prob_i) \geq \RB $, $\forall \Prob_i \in [0, 1]$;
% \item
%$\RA_i(\Prob_i)  = \RB$, only when $\Prob_i=0$ and meanwhile there is no licensee interference $\{ \InfTV_{\k} \}_{k\in\Kset}$.
%\end{itemize}
%\end{proposition}
%
%
%
%Then we consider the expected data rate of the \eus~who subscribe to the advance service (i.e., $\l=\A_{\i}, \i \in \{ 1, 2 \}$).
%With this advanced service, the \db~$\i$ returns the interference $\{ \InfKnown^{\i}_{k}\}_{k\in\Kset}$ to {\eus}, together with the basic information such as the available channel list.
%Notice that the actual interference also includes the interference part $\{\InfUnknown^{\i}_{k}\}_{k\in\Kset} $ not known by the database $\i$.
%%\db~ranks the \chs~in ascending order given \ch~interference level it known (i.e., $\InfKnown_{1}, \InfKnown_{2}, \ldots, \InfKnown_{\K} $). The ranked interference level are denoted by $\InfKnown_{(1)}, \InfKnown_{(2)}, \ldots, \InfKnown_{(\K)}$ and satisfy $\InfKnown_{(1)} < \ldots< \InfKnown_{(\K)}$.
%For a rational {\eu}, he will always choose the channel with the lowest $\InfKnown^{\i}_{k}$ provided~by~the~database.\footnotesc{This is because the uncertain interference $\{\InfUnknown^{\i}_{k}\}_{k\in\Kset} $ are i.i.d.}
%Let $\InfKnownMin^{\i} =  \min\{ \InfKnown^{\i}_{1},  \ldots, \InfKnown^{\i}_{\k}  \} $ denote the lowest interference provided by the database.
%Then, the actual interference experienced by the {\eu} is $\InfTotA^{\i} = \InfKnownMin^{\i} + \InfUnknown$, and accordingly the expected data rate is
%%Hence, the advanced \eus~transmit at the \ch~with lowest $\InfKnown$ and with total interference level $\InfTotA = \InfKnownMin + \InfUnknown$. Therefore, the advanced \eu's expect data rate is
%\begin{equation}\label{eq:rate-pay-fixed}
%\begin{aligned}
%\ut(\R^{\A_{\i}})  = \RA^{\i} & \textstyle \triangleq \ut( \Ex_{\InfTotA^{\i}} \big[ \rt \big(\InfKnownMin^{\i} + \InfUnknown^{\i} \big) \big] ) \\
%%&= \Ex_{\InfTotA} \big[ \rt \big( \InfKnownMin + \InfUnknown \big) \big] \\
%%&= \K \cdot \int_{\InfTotA} \rt(z) \cdot \big[ \int_{\infty}^{\infty} f_{\InfKnown}(z -y) \cdot [ 1 - F_{\InfKnown}(y)]^{K-1} \cdot f_{\InfUnknown}(y) \mathrm{d}y  \big] \mathrm{d}z
%& \textstyle  = \ut( \int_{\InfTotA^{\i}} \rt(z) \cdot h(z) \cdot \mathrm{d}z ),
%%\vspace{8mm}
%\end{aligned}
%\end{equation}
%where
% $h(\cdot)$ is the pdf of $\InfTotA^{\i}$, defined by
%\begin{equation*}\label{eq:min-known-pdf}
%%\begin{aligned}
%\textstyle
%h(z) = \K \cdot \int f_{\InfKnown^{\i}}(z -y) \cdot \big[ 1 - F_{\InfKnown^{\i}}(z - y) \big]^{K-1} \cdot f_{\InfUnknown^{\i}}(y) \cdot \mathrm{d}y.
%%\vspace{8mm}
%%\end{aligned}
%\end{equation*}
%By (\ref{eq:rate-pay-fixed}), we can see that $\RA^{\i}$ depends on the distributions of $\InfKnown^{\i}_k$ and $\InfUnknown^{\i}_k$, and accordingly depends on the market share $\Prob_{\i}$ (and thus, we will also write $\RA^{\i}$ as $\RA(\Prob_{\i})$).
%We can further check that $\RA(\Prob_{\i})$ increases with $\Prob_{\i}$. This is because the more {\eus} subscribing to the advanced service,  the more accurate the database's information is, and further the more benefit for the {\eus} subscribing to the advanced service. We can also note that if two database $\dbb_1$ and $\dbb_2$ share their market shared information, both of them can obtain more accurate information. However, they compete for the same pool of {\eus}. Sharing the information may lead to the decreasing of their own profit.

%Based on the above, we can find the following useful properties, which are very important for the later analysis.
%\begin{proposition}\label{prop:ABS}
%~
%\begin{itemize}
%\item
% $\RB$ in (\ref{eq:rate-random-fixed}) and $\RS$ in (\ref{eq:rate-sense-fixed}) do not depend on $\Prob$;
% \item
% $\RA(\Prob)$ in (\ref{eq:rate-pay-fixed}) monotonously increases with $\Prob$;
% \item
% $\RB\leq \RA(\Prob) \leq \RS $, $\forall \Prob \in [0, 1]$;
% \item
%$\RA(1)  = \RS$, if no outside interference $\{ \InfOut_{\k} \}_{k\in\Kset}$;
% \item
%$\RA(0)  = \RB$, if no licensee interference $\{ \InfTV_{\k} \}_{k\in\Kset}$.
%\end{itemize}
%\end{proposition}




\textbf{Problem Formulation.}
Suppose that each {\eu} is rational, and will always choose the strategy that maximizes its payoff.
We are interested in the following problems: given the information prices $\{\p_1, \p_2\}$ and initial market shares $\{\Prob^0_1, \Prob^0_2 \}$ of databases, how these market shares dynamically evolve and what is the market equilibrium?

%We will study the oligopoly price competition game between databases $\dbb_1$ and $\dbb_2$.
%In the proposed oligopoly price competition game, each database $\dbb_i$ chooses the price $\p_i$ for its information, aiming at maximizing its revenue
%$$
%\Udb_i = \p_i\cdot \Prob_i \cdot N.
%$$
%%given the distributions of licensee interference $\InfTV_{\k}$, outside interference $\InfOut_{\k}$, and single {\eu} interference $\InfEU_{\n,\k}$.
%Note that the market share $\Prob_i $ of the database $\dbb_i$ depends not only on its own price $\p_i$, but also on the other database $\dbb_j$'s price $\p_j$, and thus can be written as $\Prob_i(\p_1, \p_2)$.
%Moreover, the change of $\Prob_i$ will affect the distributions of $\InfKnown_k^i$ (known by the database $\dbb_i$) and $\InfUnknown_k^i$ (not known by the database $\dbb_i$), which in turn will affect the {\eu}'s utility $\RA_i(\Prob_i)$ achieved from the database $\dbb_i$'s advanced service.

%
%revenue maximization where two database compete by choosing prices, given the distributions of licensee interference $\InfTV_{\k}$, outside interference $\InfOut_{\k}$, and single {\eu} interference $\InfEU_{\n}$.
%For database $\i$, its {revenue} is $\p_{\i} \cdot \Prob_{\i}(\bp) \cdot N$.
%%optimal information pricing plan (i.e., $\p_1$ and $\p_2$) that maximizes the database's
%Notice that the database $\dbb_{\i}$'s market share $\Prob_{\i}(\bp)$ is a function of $\bp = (\p_1, \p_2)$.
%Moreover, the change of $\BProb$ will affect the interference levels $\InfKnown^{\i}_k$ (known by the database) and $\InfUnknown^{\i}_k$ (not known by the database), which in turn will affect the {\eu}'s expected data rate $\RA^{\i}(\BProb)$ achieved from the advanced service, and the {\eu}'s decision.

% (ii)
%By comparing (\ref{eq:rate-random-fixed}), (\ref{eq:rate-sense-fixed}), and (\ref{eq:rate-pay-fixed}), we have $\RB \leq \RA \leq \RS$
%When the random variable $\InfKnown$ is zero, we have $\RA = \RB$. Otherwise, $\RA > \RB$, $\forall \Prob \in [0,1]$. If the value of $\InfUnknown$ is zero, we have $\RA = \RS$. Otherwise, $\RA < \RS$, $\forall \Prob \in [0,1]$.

%We associate interference caused by TV station denoted by $\InfTV$, which is a random variable follows from a continuous distribution with cdf $F_{\InfTV}(\cdot) $ and pdf $f_{\InfTV}(\cdot)$. $\InfOut$ represents the interference cause by other database's {\eus} and is a random variable follows from a continuous distribution with cdf $F_{\InfOut}(\cdot) $ and pdf $f_{\InfOut}(\cdot)$ and represents the interference cause by other database's {\eus}. For particular {\eu}, we assume its receiving interference from each {\eu} in the same network \footnotesc{We assume {\eus} who connect to the same database acting in the same network.} $Y$ is a random variable with cdf $F_{Y}(\cdot) $ and pdf $f_{Y}(\cdot)$.



==> Section_Information_Market.tex <==
%!TEX root = main_hybrid_market.tex
%SourceDoc main_hybrid_market.tex


\section{Information Value} 

%Before we solve the three-stage model discussed in the previous section with backwards induction. We first need to characterize the utility provided by different service so that we can analyze the subscription choice of {\eus}. Hence, in the next section, we will analyze the value of information to {\eus}.
%

Before analyzing the hybrid market, we first need to compute the value of advanced information for those WSD users using the unregistered channels. 
In this section, we first characterize the interference level on each unregistered channel for each \eu~(using the unregistered \chs), which essentially defines the advanced information. 
Then, we establish a framework to evaluate the value of advanced information for the WSD users using the unregistered channels.

%\subsection{Basic Service and Advanced Service}
%As mentioned in the previous section, the basic service is mainly consisted of the available TV \chs~list, while the advanced service is the interference level on every available \ch~for a particular \eu~and is denoted as $\{\InfTot_{\k}\}_{k\in\Kset}$.
%
%For convenience, we illustrate the basic service and advanced service by the example in the following table.
%In the basic service, the database provides the available channel set (i.e., \{CH1, CH3, CH4, CH6\}) to a particular \eu. In the advanced service, the database provides the interference levels on available channels (i.e., \{$\InfTot_1$, $\InfTot_3$, $\InfTot_4$, $\InfTot_6$\}) to the \eu, in addition to the available channel set.
%
%\begin{table}[h]
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\textbf{Channel ID} & \textbf{CH1}& \textbf{CH2}& \textbf{CH3} & \textbf{CH4} & \textbf{CH5} & \textbf{CH6}
%\\
%\hline
%Availability & Yes & No & Yes & Yes & No & Yes
%\\
%\hline
%Interference Level & $\InfTot_1$ &  - & $\InfTot_3$ & $\InfTot_4$ &  - & $\InfTot_6$
%\\
%\hline
%\end{tabular}
%\end{table}

\subsection{Interference Information}
\label{sec:interference_info}

\com{iid over time is easier to understand, assuming that the number of users on the channel does not change, but the channel gains change over time due to fading.
however, we need to better justify the iid assumption over frequency. This relies on the assumption that the number of users on each channel (which is a random variable) is iid.
We need to explain
- why this is a good assumption (possible answer: users with basic service will randomly choose, hence the number of such users per channel will follow the same distribution. Users with advanced service will go to the channel with the minimum "actual" interference. If the interference among each pair of users is iid over time, then statistically the number of such users in each channel will also follow the same distribution. )
-  why under such an assumption the information market still is useful (possible answer: the market provides the accurate interference information instead of the statistical information.)
Some of the above detailed discussions can be deferred to later part (the bottom part of the 2nd column on this page). However, it is important to make sure that readers understand (at this point) that the iid assumption is justified to certain extent, instead of just convenient assumption for analytical purpose.
Finally, important assumptions need to be put into the "Assumption" environment. So here which one is the fundamental assumption we make, and which ones are actually derived from the assumption (and hence are not assumption themselves)?
}

\rev{
For each {\eu} $n\in \Nset$ operating on the TV \ch, each channel $\k$ is associated with an \emph{interference level}, denoted by  $\InfTot_{\n,\k}$, which reflects the aggregate interference from all other nearby devices (including TV stations
and other {\eus}) operating on this channel.
Due to the fast changing of wireless channels and the uncertainty of {\eus}' mobilities and activities, the interference $\InfTot_{\n,\k}$ is a random variable. We impose assumptions on the interference $\InfTot_{\n,\k}$ as follows.
\begin{assumption}\label{assum:iid}
For each {\eu} $n\in \Nset$, each channel $\k$'s interference level $\InfTot_{\n,\k}$ is \emph{temporal-independence} and \emph{frequency-independence}.
\end{assumption}

This assumption shows that
(i) the interference $\InfTot_{\n,\k}$ on channel $\k$ is independent identically distributed (iid) at different times, and (ii)
the interferences on different channels, $\InfTot_{\n,\k}, \k\in\Kset$, are also iid at the same time.\footnotesc{\rev{Note that the iid assumption is a reasonable approximation of the practical scenario (e.g., \cite{chang2009channel,jiang2009channel,zhou2011channel}). This is because {\eus} with basic service will randomly choose one TV \ch, hence the number of such {\eus} per channel will follow the same distribution. For {\eus} with advanced service, they will go to the TV \ch~with the minimum realized interference. If the interference among each pair of users is iid over time, then statistically the number of such users in each channel will also follow the same distribution. Note that even though all channel quality distributions are the same, the realized instant qualities of different channels are different. Hence, the advanced information provided by the \db~is still valuable as such an advanced information is accurate interference information.} }
As we are talking about a general \eu~$n$, \textbf{we will omit the {\eu} index $n$ in the notations (e.g., write $\InfTot_{\n,\k}$ as $\InfTot_{\k}$), whenever there is no confusion caused.}
Let $F_{\InfTot}(\cdot)$ and $f_{\InfTot}(\cdot)$ denote the cumulative distribution function (CDF) and probability distribution function (PDF) of $\InfTot_{\k}$, $\forall \k\in\Kset$.\footnotesc{In this paper, we will conventionally  use $F_X(\cdot)$ and $f_X(\cdot)$ to denote the CDF and PDF of a random variable $X$, respectively.}~~~~
}

Usually, a particular {\eu}'s experienced interference $\InfTot_{\k}$ on a \ch~$\k$ consistss of the following three components:
\begin{enumerate}
\item
$\InfTV_{\k}$: the interference from licensed TV stations;
\item
$\InfEU_{\k,m}$: the interference from another {\eu} $m$ operating on the same channel $k$;
\item
$\InfOut_{\k}$: any other interference from outside systems.
\end{enumerate}
The total interference on channel $k$ is
$
\InfTot_{\k} = \InfTV_k + \InfEU_k + \InfOut_k
$, where  $\InfEU_k  \triangleq \sum_{m \in \Nkset} \InfEU_{\k,m}$ is the total interference from all other {\eus} operating on channel $k$ (denoted by $\Nkset$).
Similar to $\InfTot_{\k}$, we also assume that  $ \InfTV_k , \InfEU_k , \InfEU_{\k,m}$, and $ \InfOut_k$ are random variables with \emph{temporal-independence} (i.e., iid across time) and \emph{frequency-independence} (i.e., iid across frequency).
We further assume that $\InfEU_{\k,m}$ is \emph{user-independence}, i.e., $\InfEU_{\k,m}, m\in \Nkset$, are iid.
{It is important to note that \textbf{different {\eus} may experience different interferences $\InfTV_k$ (from TV stations), $ \InfEU_{\k,m} $ (from another \eu~operating on the same \ch), and $ \InfOut_k$ (from outside systems) on a channel $k$, as we have omitted the \eu~index $n$ for all these notations for clarity.}}
\com{Similarly, the iid assumption over space is ok for Lk, Ik, and even Wk,m, but not for Wk which depends on the number of users on each channel? Need to explain.}

Next we discuss these interferences in more details.

\begin{itemize}
\item
The \db~is able to compute the interference $\InfTV_k$ from TV stations to every {\eu} (on channel $k$), as it knows the locations and channel occupancies of all TV stations.~~~~

\item
The \db~cannot compute the interference
$\InfOut_k$ from outside systems, due to the lack of outside interference source information.
Thus, the interference $\InfOut_{\k}$ will \emph{not} be included in a database's advanced information sold to {\eus}.~~~~~~~~

\item
The \db~may or may not be able to compute the interference $\InfEU_{\k,m}$ from another {\eu} $m$, depending on whether {\eu} $m$ subscribes to the \db's advanced service.
Specifically, if {\eu} $m$ subscribes to the advanced service, the \db~can predict its channel selection (since the {\eu} is fully rational and will always choose the channel with the lowest interference level indicated by the \db~at the time of subscription), and thus can compute its interference to any other \eu.
However, if {\eu} $m$ only chooses the \db's basic service, the \db~cannot predict its channel selection, and thus cannot compute its interference to other \eus.~~~~
\end{itemize}

For convenience, we denote $\Nkset^{[\A]}$, as the set of {\eus} operating on \ch~$k$ and subscribing to the \db's advance service (i.e., those choosing the strategy $\l = \A$), and $\Nkset^{[\B]}$ as the set of {\eus} operating on channel $k$ and choosing the \db's basic service (i.e., those choosing the strategy $\l = \B$).
That is, $\Nkset^{[\A]} \bigcup \Nkset^{[\B]} = \Nkset $.
Then, for a particular {\eu}, its experienced interference (on channel $k$) \textbf{known by the \db} is
% (and thus will be included in the database $\dbb_i$'s advanced service to this WSD) is
\begin{equation}\label{eq:known_inf}
\begin{aligned}
\textstyle
\InfKnown_{\k} \triangleq \InfTV_{\k} + \sum_{m \in \Nkset^{[\A]}} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from TV licensees and all {\eus} (operating on channel $k$)  subscribing to the \db's advanced service.
The \eu's experienced interference (on channel $k$) \textbf{\emph{not} known by the \db} is
% (and thus will not be included in the database $\dbb_i$'s advanced information) is
\begin{equation}\label{eq:unknown_inf}
\begin{aligned}
\textstyle
\InfUnknown_{\k}  \triangleq \InfOut_{\k} + \sum_{m \in \Nkset^{[\B]}} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from outside systems and all {\eus} (operating on channel $k$) choosing the \db's basic service.
Obviously, both $\InfUnknown_{\k}$ and $\InfKnown_{\k}$ are also random variables with temporal- and frequency-independence.
Accordingly, the total interference on {\ch} $\k$ for a {\eu} can be written as
$\textstyle
\InfTot_{\k} = \InfKnown_{\k} + \InfUnknown_{\k}.$~~~~~~

\textbf{Since the \db~knows only $\InfKnown_{\k}$, it will provide this information (instead of the total interference $\InfTot_k$) as the {advanced service} to a subscribing {\eu}.}
It is easy to see that the more {\eus} subscribing to the \db's advanced service, the more information the \db~knows, and the more accurate the \db~information will be.


Next we can characterize the accuracy of a database's information explicitly. Note that $\Proba$ and $\Probl$ denote the fraction of {\eus} choosing the advanced service and leasing licensed spectrum, respectively. Moreover, $(1 - \Proba - \Probl)$ denotes the fraction of {\eus} choosing the basic service.
Hence, there are $(1 - \Probl) \cdot \N$ {\eus} in the network that we consider operating on the TV \chs.
Due to the Assumption \ref{assum:iid}, it is reasonable to assume that each channel $k\in\Kset$ will be occupied by an average of $\frac{\N}{\K} \cdot ( 1 - \Probl)$ {\eus}.\com{Yuan: Do we need to add more explanation on this?}
%Let $\Prob_l$ denote the percentage of {\eus} subscribing to the advanced service of database $\dbb_l$ (called the \emph{market share} of database $\dbb_l$).
Then, among all $\frac{\N}{\K} \cdot ( 1 - \Probl)$ {\eus} operating on channel $k$, there are, \emph{on average}, $\frac{\N}{\K}\cdot\Proba$ {\eus}  subscribing to the \db's advanced service, and $\frac{\N}{\K}\cdot ( 1 - \Proba - \Probl )$ {\eus} choosing the \db's basic service.
That is, $| \Nkset | = \frac{\N}{\K} \cdot ( 1 - \Probl)$, $| \Nkset^{[\A]} | = \frac{\N}{\K}\cdot\Proba$, and $|\Nkset^{[\B]} | = \frac{\N}{\K}\cdot(1-\Proba-\Probl)$.\footnotesc{{Note that the above discussion is from the aspect of expectation, and in a particular time period, the realized numbers of {\eus} in different channels may be different.}}
Finally, by the {user-independence} of $\InfEU_{\k,m}$, we can immediately calculate the distributions of $ \InfKnown_{\k}$ and $ \InfUnknown_{\k}$ under any given market share $\Proba$ and $\Probl$ via (\ref{eq:known_inf}) and (\ref{eq:unknown_inf}).

\rev{
\subsection{Information Value}
Now we evaluate the value of the \db's advanced information to {\eus}, which is
reflected by the {\eu}'s benefit (utility) that can be achieved from this information.

We first consider the expected  utility of a {\eu} when choosing the \db's basic service (i.e., $\l=\B$).
In this case, the {\eu} will randomly choosing a \tvch~based on the information provided in the free basic service,
and its expected data rate is
\begin{equation}\label{eq:rate-random-fixed}
\begin{aligned}
\textstyle
\R_0( 1 - \Probl)  \textstyle = \Ex_{Z} [\rt(\InfTot)] = \int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z), \\
%\RB   \textstyle \triangleq \fx = \ut(\R_0) = \ut\left(\int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z)\right),
\end{aligned}
\end{equation}
%where $\R_0$ is the expected data rate and is given as follows.
%\begin{equation}\label{eq:rkgs}
%\begin{aligned}
%& \R_0  \textstyle = \Ex_{Z} [\rt(\InfTot)] = \int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z),
%\end{aligned}
%\end{equation}
where $\rt(\cdot)$ is the transmission rate function (e.g.,
the Shannon capacity) under any given interference.
As shown in Section \ref{sec:interference_info}, each channel $k\in\Kset$ will be occupied by an average of $\frac{\N}{\K} \cdot ( 1 - \Probl)$ {\eus} based on the Assumption \ref{assum:iid}. Hence,
$\R_0( 1 - \Probl) $ depends only on the distribution of the total interference $\InfTot_k$, and thus depends on the fraction of {\eus} operating on TV \chs~(i.e., $1 - \Probl$). Then the expected utility provided by the basic service is:
\begin{equation}\label{eq:utility-random-fixed}
\begin{aligned}
\textstyle
\RB(1 - \Probl) = \textstyle \ut\bigg(\R_0( 1 - \Probl)\bigg),
% = \ut\left(\int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z)\right),
\end{aligned}
\end{equation}
where $\ut(\cdot)$ is the utility function of the \eu. We can easily check that
the more {\eus} operating on the TV \chs, the higher value of $\InfTot_k$ is, and thus the lower expected utility provided by the basic service. Hence, the basic service's expected utility reflects the congestion level of the TV \chs.
We use the function $\fx(\cdot)$ to characterize the congestion effect and have $\fx(1 - \Probl) = \RB( 1 - \Probl)$.
%while not on the specific distributions of $\InfKnown_k$ and $\InfUnknown_k$. This implies that the accuracy of the \db's information does not affect the utilities of those {\eus} choosing the basic service. However, as t

Then we consider the expected utility of a {\eu} when subscribing to the \db's advance service.
In this case, the {\db} returns the interference $\{\InfKnown_{k}\}_{k\in\Kset}$ to the {\eu} subscribing to the advanced service, together with the basic information such as the available channel list.
For a rational {\eu}, it will always choose the channel with the minimum $\InfKnown_{k}$ (since $\{\InfUnknown_{k}\}_{k\in\Kset}$ are iid).
Let $\InfKnownMin^{[l]} =  \min\{ \InfKnown_{1},  \ldots, \InfKnown_{K} \} $ denote the minimum interference indicated by the \db's advanced information.
Then, the actual interference experienced by a {\eu} (subscribing to the \db's advanced service) can be formulated as the sum of two random variables, denoted by $\InfTotA = \InfKnownMin + \InfUnknown$. Accordingly, the {\eu}'s expected data rate under the strategy $\l = \A$ can be computed by
\begin{equation}\label{eq:rate-pay-fixed}
\begin{aligned}
\Ra(\Proba, \Probl) & \textstyle = \Ex_{\InfTotA} \big[ \rt \left( \InfTotA \right) \big] = \int_z \rt(z)  \mathrm{d} F_{\InfTotA}(z),
%\\
%\RA & \textstyle  \triangleq \ut\left(\Ra\right) = \ut\left(\int_z \rt(z)  \mathrm{d} F_{\InfTotA}(z)	\right) ,
\end{aligned}
\end{equation}
where
$F_{\InfTotA}(z)$ is the CDF of $\InfTotA$. It is easy to see that $\Ra$ depends on the distributions of $\InfKnown_k$ and $\InfUnknown_k$, and thus depend on the market share $\Probl$ and $\Proba$.
Thus, we will write $\Ra$ as $\Ra(\Probl,\Proba)$. Accordingly, the advanced service's utility is:
 \begin{equation}\label{eq:utility-pay-fixed}
\begin{aligned}
%\Ra & \textstyle = \Ex_{\InfTotA} \big[ \rt \left( \InfTotA \right) \big] = \int_z \rt(z)  \mathrm{d} F_{\InfTotA}(z),
%\\
\RA(\Probl,\Proba) & \textstyle  \triangleq \ut\bigg( \Ra( \Probl,\Proba ) \bigg)
%= \ut\left(\int_z \rt(z)  \mathrm{d} F_{\InfTotA}(z)	\right) ,
\end{aligned}
\end{equation}

Note that the congestion effect also affects the value of $\RA$. However, compared with the utility of {\eu} choosing basic service, the benefit of a {\eu} subscribing to the \db's advanced information is coming from the $\InfKnownMin^{[l]}$, i.e., the minimum interference indicated by the \db's advanced information. As the value of $\InfKnownMin^{[l]}$ depends on the $\Proba$ only, we can get the approximation $\RA = \fx(1 - \Probl) + \gy(\Proba)$, where function $\gy(\cdot)$ characterize the benefit brought by $\InfKnownMin^{[l]}$ and denotes the positive network effect.
\com{This is a key assumption, by writing $\RA(\Probl,\Proba)$ as two separate terms. How to justify this? How to verify this? }


%We define $\RB$ and $\RA$ as follows:
%\begin{equation}\label{eq:utility-service-general}
%\begin{aligned}
%\RB & \textstyle \triangleq \fx(1 - \Probl),
%\\
%\RA & \textstyle \triangleq \fx( 1 - \Probl) + \gy(\Proba).
%\end{aligned}
%\end{equation}
%where the function $\fx(\cdot)$ denotes the \emph{congestion effect}, and the function $\gy(\cdot)$ denotes the \emph{positive network effect}.

%Note that the congestion effect depends on the total number of {\eus} in the TV \chs, because the more {\eus} are, the higher co-interference is. The positive network effect depends only on the number of {\eus} subscribing to the \db's advanced service. This is because the more {\eus} subscribing to the \db's advanced service, the more information such as the {\eus}' TV \ch~selection and the transmission power the \db~knows, and the more accurate the information about the best available \ch~will be.

By further checking the properties of $\RB(1 - \Probl)$ and $\RA(\Probl,\Proba)$, we have the following assumptions.

\begin{assumption}\label{assum:congestion}
The function $\fx(\cdot)$ is nonnegative, nonincreasing, convex, and continuously differentiable.
\end{assumption}

\begin{assumption}\label{assum:positive}
The function $\gy(\cdot)$ is nonnegative, nondecreasing, concave, and continuously differentiable.
\end{assumption}

The convexity requirement of $\fx$ due to the characteristic of interference in the expected data rate and is a common assumption in wireless networking (see e.g., \cite{shetty2010congestion,acemoglu2010congestion,johari2010congestion} and references therein). The concavity requirement of $\gy$ results form decelerating returns to increased the number of {\eus} subscribing to the advanced service. This is because in sharing the TV white space network, when the number of {\eus} is small, then each additional \eu~makes the network significantly more useful; but an additional \eu~may go unnoticed when added to a TV white space network.

Because function $\fx$ and $\gy$ can characterize the information value to the {\eus}, we begin to solve the three-stage model discussed in the previous section with backwards induction.
}

%\textbf{Problem Formulation.}
%Suppose that each {\eu} is rational, and will always choose the strategy that maximizes its payoff.
%We are interested in the following problems: given the information prices $\{\p_1, \p_2\}$ and initial market shares $\{\Prob^0_1, \Prob^0_2 \}$ of databases, how these market shares dynamically evolve and what is the market equilibrium?




==> Section_Model_new.tex <==
%!TEX root = main_inform_compe.tex
%SourceDoc main_inform_compe.tex

\section{System Model}\label{sec:model}
\subsection{TV White Space Information Market}
In this section, we first consider a monopoly TV white space network, where a set $\Nset=\{1,...,\N\}$ of unlicensed white space devices ({\eus}) can only operating on idle TV channels requested from a white space database.
Let $\Kset = \{ 1,\ldots, \K \}$ denote the set of available TV channels in the area of the network.
Each \eu~queries a database for the available TV channel set, and  can only operate on \emph{one} of the available \chs~at a particular time.

According to the regulator's ruling (e.g., FCC \cite{federal2010second}), a certified white space {\db} provides the following information for {\eus}: (i) the list of available TV channels, (ii) the transmission constraints (e.g., maximum transmission power) on each available channel, and (iii) some other optional requirements.
This is the basic information (\emph{basic service}) that every {\db} is mandatory to provide for any {\eu} free of charge.

Beyond the basic service, the white space {\db} can also provide certain advanced information (\emph{advanced service}) to make a profit, under the constraint that it does not conflict with the basic service.
Motivated by the practice of Spectrum Bridge \cite{SpectrumBridgeCommericial}, we consider such an advanced service, where each {\db} provides the following advanced information to every WSD $n$ subscribing to its advanced service\footnotesc{{``Subscribe to a \db'' means that the \eu purchases the advanced information from the \db.}}:
$\{\InfTot_{\k}\}_{k\in\Kset}$ (i.e., the interference level on every available channel for this particular \eu).
%When subscribing to the advanced service of a \db,
With this advanced information,
the {\eu} is able to operate on the best available channel (with the lowest interference level).
Accordingly, the {\db} can charge a \emph{subscription fee} (denoted by $\pa$) to every {\eu} subscribing to its advanced service.
This essentially constitutes an \emph{information market}.~~~~~~~~

For convenience, we illustrate the basic service and advanced service by the example in the following table.
In the basic service, the database provides the available channel set (i.e., \{CH1, CH3, CH4, CH6\}) to a particular \eu. In the advanced service, the database provides the interference levels on available channels (i.e., \{$\InfTot_1$, $\InfTot_3$, $\InfTot_4$, $\InfTot_6$\}) to the \eu, in addition to the available channel set.

\begin{table}[h]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Channel ID} & \textbf{CH1}& \textbf{CH2}& \textbf{CH3} & \textbf{CH4} & \textbf{CH5} & \textbf{CH6}
\\
\hline
Availability & Yes & No & Yes & Yes & No & Yes
\\
\hline
Interference Level & $\InfTot_1$ &  - & $\InfTot_3$ & $\InfTot_4$ &  - & $\InfTot_6$
\\
\hline
\end{tabular}
\end{table}


%======================
Assume that \eus are heterogeneous in the valuation of the achieved utility by choosing different services. We denote the \eu's valuation for the achieved utility by $\th$, and for analytic simplicity, assume that is it uniformly distributed in $[0,1]$.


After obtaining the available channel list through the free basic service, each {\eu} has 2 choices (denoted by $\l$) in terms of channel selection:
\begin{itemize}
\item[(i)] $\l = \A$: subscribing to the \db's advanced service, and picking the channel with the lowest interference indicated by the \db;
\item[(ii)] $\l = \B$: choosing an available channel randomly;
\end{itemize}
The \emph{payoff} of {\eu} equals (i) the benefit (\emph{utility}) from the achieved data rate on the selected channel minus (ii) the \emph{subscription fee} if subscribing to  an advanced service.
Formally, the payoff of {\eu} can be defined as:~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\begin{equation}\label{eq:utility-basic}
\Ueu  = \left\{
  \begin{aligned}
  &\textstyle  \th \cdot \ut(\R_l)  -  \p_l , &&  \  \text{if} ~ \l \in\{1,2\}, \\
%  &\textstyle  \th \cdot \ut(\Rkab)  -  \p_2 , &&  \quad  \text{if} ~ \l = \A_2, \\
  &\textstyle  \th \cdot \ut(\R_0) ,      &&  \ \text{if} ~ \l = 0,
%  \\
%  &\textstyle  \th \cdot \ut(\Rkgb) ,      &&  \quad  \text{if} ~ \l = \G_2, \\
   \end{aligned}
\right.
\end{equation}
where $\Rl$ is the expected data rate when the {\eu} chooses a strategy $\l\in \{ 0,1,2\}$, $\ut(\cdot)$ is the utility function (concave and increasing) of the \eu, and $\th$ is the \eu's evaluation for the achieved utility.
Note that different {\eus} may have the different utility evaluation factor $\th$ (e.g., for different applications), that is, {\eus} are heterogeneous in term of $\th$.
For the analytical convenience, we assume that $\th$ is uniformly distributed in $[0,1]$ for all \eus.
%We consider heterogeneous \eus, where different {\eus} value the same data transmission rate or utility differently (due to different wireless applications).
%, and $\kl$, $\l \in \{ \G, \S, \A \}$ is the \ch~index chosen by the type-$\th$ \eu~based on the \ch~state information provided by different service scheme.
%$\Ra$, $\Rs$, and $\Rr$ is expected data rate corresponding to different \eu's choice.
%Note that in our model, the \db~is not allowed to engage in either QoS discrimination nor price discrimination.
%Here assume that all \eus~are charged by the same price $\p_i$ if $\l=\A_i$.
%In other words, the \db~is not allowed to engage in price discrimination for the simplicity of practical implementation.




%We consider a online spectrum information platform which lists the available TV \chs~list and the leasing spectrum information. We assume that a \db~owns this online information platform and the licensed spectrum holders (called \lh) put their licensed spectrum information on this online platform \footnote{According to the regulators' ruling (e.g., FCC \cite{federal2010second}), only the \db~can house the TV \chs availability information. Hence, only the \db~can own this online information platform. We can interpret listing licensed spectrum information as the extra service provided by the \db as currently the Spectrum Bridge does.}.
%In a particular network service area, there are a set $\Nset=\{1,...,\N\}$ of unlicensed white space devices ({\eus}) access to this online information platform and make the choice between operating on the TV  \chs~and leasing the licensed spectrum.
%Let $\Kset = \{ 1,\ldots, \K \}$ denote the set of available TV channels in this area. Each \eu~can only operate on \emph{one} of the available \chs~at a particular time on the shared basis (i.e., each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques).
%We assume that the number of licensed spectrum for leasing is sufficient and each \eu~can use the leasing spectrum exclusively.
%
%\textbf{White Space Database.}
%According to the regulator's ruling (e.g., FCC \cite{federal2010second}), a certified white space {\db} provides the following information for {\eus}: (i) the list of available TV channels, (ii) the transmission constraints (e.g., maximum transmission power) on each available channel, and (iii) some other optional requirements.
%This is the basic information (\emph{basic service}) that every {\db} is mandatory to provide for any {\eu} free of charge.
%
%Beyond the basic service, the white space {\db} can also provide certain advanced information (\emph{advanced service}) to make a profit, under the constraint that it does not conflict with the basic service.
%Motivated by the practice of Spectrum Bridge \cite{SpectrumBridgeCommericial}, we consider such an advanced service, where each {\db} provides the following advanced information to every WSD $n$ subscribing to its advanced service\footnotesc{{``Subscribe to a \db'' means that the \eu purchases the advanced information from the \db.}}:
%$\{\InfTot_{\k}\}_{k\in\Kset}$ (i.e., the interference level on every available channel for this particular \eu).
%%When subscribing to the advanced service of a \db,
%With this advanced information,
%the {\eu} is able to operate on the best available channel (with the lowest interference level).
%Accordingly, each {\db} $\dbb_i $ can charge a \emph{subscription fee} (denoted by $\p_i$) to every {\eu} subscribing to its advanced service.
%%Notice that providing such interference information is not enforced by the regulator, and it is based on the bilateral agreement between a {\eu} and a database.
%%For example, each database can choose whether to offer this advanced service and at what price, and each {\eu} can choose whether and from which database it is going to subscribe to this service.
%This essentially constitutes an \emph{information market}.~~~~~~~~
%
%For convenience, we illustrate the basic service and advanced service by the example in the following table.
%In the basic service, the database provides the available channel set (i.e., \{CH1, CH3, CH4, CH6\}) to a particular \eu. In the advanced service, the database provides the interference levels on available channels (i.e., \{$\InfTot_1$, $\InfTot_3$, $\InfTot_4$, $\InfTot_6$\}) to the \eu, in addition to the available channel set.
%
%\begin{table}[h]
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\textbf{Channel ID} & \textbf{CH1}& \textbf{CH2}& \textbf{CH3} & \textbf{CH4} & \textbf{CH5} & \textbf{CH6}
%\\
%\hline
%Availability & Yes & No & Yes & Yes & No & Yes
%\\
%\hline
%Interference Level & $\InfTot_1$ &  - & $\InfTot_3$ & $\InfTot_4$ &  - & $\InfTot_6$
%\\
%\hline
%\end{tabular}
%\end{table}

%
%\textbf{White Space Devices ({\eus}).}
After obtaining the available channel list through the free basic service, each {\eu} has 3 choices (denoted by $\l$) in terms of channel selection:
\begin{itemize}
\item[(i)] $\l \in\{1,2\}$: subscribing to the database $\dbb_l$'s advanced service, and picking the channel with the lowest interference indicated by database $\dbb_l$;
\item[(ii)] $\l = 0$: choosing an available channel randomly;
% in the available channel list.
%\footnotesc{We do not consider the sensing capability of WSDs, which has been removed in the FCC ruling \cite{federal2010second}.}
\end{itemize}
The \emph{payoff} of {\eu} equals (i) the benefit (\emph{utility}) from the achieved data rate on the selected channel minus (ii) the \emph{subscription fee} if subscribing to  an advanced service.
%We assume that each {\eu} is rational, and will always choose the strategy that maximizes its payoff.
Formally, the payoff of {\eu} can be defined as:~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%We assume the \eus~valuation of expected data rate follows a probability distribution. For analysis tractability, we assume that $\th$ is uniformly distributed in $[0,1]$.
%We use $\a_{\n}$ denote the service scheme selected by \eu~$\n$. $\a_{\n} = 0$ represents the subscription scheme, $\a_{\n} = 1$ represents the sensing scheme, and $\a_{\n}=2$ is the random choosing scheme.
%Let us denote an \eu's choice as $\l$, with $\l = \A_1$ denoting subscribing to the $\dbb_1$'s advanced service, $\l = \A_2$ denoting subscribing to the $\dbb_2$'s advanced service, $\l = \G_1$
%denoting  randomly selecting a channel (under the $\dbb_1$'s basic service), and $\l = \G_2$
%denoting  randomly selecting a channel (under the $\dbb_2$'s basic service).
%Formally, the payoff of a type-$\th$ \eu~is:
\begin{equation}\label{eq:utility-basic}
\Ueu  = \left\{
  \begin{aligned}
  &\textstyle  \th \cdot \ut(\R_l)  -  \p_l , &&  \  \text{if} ~ \l \in\{1,2\}, \\
%  &\textstyle  \th \cdot \ut(\Rkab)  -  \p_2 , &&  \quad  \text{if} ~ \l = \A_2, \\
  &\textstyle  \th \cdot \ut(\R_0) ,      &&  \ \text{if} ~ \l = 0,
%  \\
%  &\textstyle  \th \cdot \ut(\Rkgb) ,      &&  \quad  \text{if} ~ \l = \G_2, \\
   \end{aligned}
\right.
\end{equation}
where $\Rl$ is the expected data rate when the {\eu} chooses a strategy $\l\in \{ 0,1,2\}$, $\ut(\cdot)$ is the utility function (concave and increasing) of the \eu, and $\th$ is the \eu's evaluation for the achieved utility.
Note that different {\eus} may have the different utility evaluation factor $\th$ (e.g., for different applications), that is, {\eus} are heterogeneous in term of $\th$.
For the analytical convenience, we assume that $\th$ is uniformly distributed in $[0,1]$ for all \eus.
%We consider heterogeneous \eus, where different {\eus} value the same data transmission rate or utility differently (due to different wireless applications).
%, and $\kl$, $\l \in \{ \G, \S, \A \}$ is the \ch~index chosen by the type-$\th$ \eu~based on the \ch~state information provided by different service scheme.
%$\Ra$, $\Rs$, and $\Rr$ is expected data rate corresponding to different \eu's choice.
%Note that in our model, the \db~is not allowed to engage in either QoS discrimination nor price discrimination.
%Here assume that all \eus~are charged by the same price $\p_i$ if $\l=\A_i$.
%In other words, the \db~is not allowed to engage in price discrimination for the simplicity of practical implementation.

Next we compute the \eu's expected data rate $\Rl$ under different strategies $\l\in\{0,1,2\}$.
Specifically, when $\l=0$ (choosing channel randomly), the {\eu}'s expected
data rate~is
\begin{equation}\label{eq:rkgs}
\begin{aligned}
& \R_0  \textstyle = \Ex_{Z} [\rt(\InfTot)] = \int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z),
%\\
%& \Rkaa = \Rkab \textstyle = \Ex_{Z_{(1)}} [\rt(Z_{(1)})] = \int_{Z} \rt(z) \mathrm{d} F_{Z_{(1)}}(z),
%\\
%& \Rkaa = \Rkab \textstyle = \Ex_{Z^{1}_{(1)}} [\rt(Z^{1}_{(1)})] = \int_{Z} \rt(z) \mathrm{d} F_{Z^{1}_{(1)}}(z),
%\\
%& \Rkab \textstyle = \Ex_{Z^{2}_{(1)}} [\rt(Z^{2}_{(1)})] = \int_{Z} \rt(z) \mathrm{d} F_{Z^{2}_{(1)}}(z),
\end{aligned}
\end{equation}
where $\rt(\cdot)$ is the transmission rate function (e.g.,
the Shannon capacity) under any given interference.
%$Z_{(1)} \triangleq \min\{Z_1,Z_2,...,Z_K\}$ is the minimum interference on all channels, and $\rt(\cdot)$ is a function that maps \ch~$\k$'s interference level $\InfTot_{\k}$ to the data rate.
%Notice the above formula assumes that the database knows precisely the state of every channel, and thus the \eus~subscribing to any \db's advanced service can always find the best channel (with the minimum interference) for transmission. Soon later we will show that $\Rkaa $ and $ \Rkab $ may not be the same when different databases do not have the precise interference information. {We will also show how the accuracy of the interference information changes with the {\eus}' subscription choices.

It is notable that under the strategy $\l\in \{1,2\}$ (subscribing to the database $\dbb_l$'s advanced service), the {\eu}'s expected data rate $\Rl$ cannot be directly computed, as it depends on the accuracy of the database $\dbb_l$'s information.
{We will provide more details regarding the computation of $\Rl$ in (\ref{eq:rate-pay-fixed}).}




%If a \eu~chooses operating on TV \ch, it can only operate on one of the available TV \chs from the \ch~set $\Kset = \{ 1,\ldots, \K \}$ at a particular time on the shared basis (i.e., each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques).
%Let $\Kset = \{ 1,\ldots, \K \}$ denote the set of available TV channels in this area. One \eu~can only operate on \emph{one} of the available \chs~at a particular time on the shared basis (i.e., each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques).
%
%Each \eu~makes its choice through the online platform provided by a \db. We assume that a \db~has the available TV \chs~information and provides such information to each querying \eu~in order to let the \eu~operate on \emph{one} of the available \chs~at a particular time. Note that each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques.
%We also assume that the licensed spectrum holders display their licensed spectrum

For each {\eu} $n\in \Nset$, each channel $\k$ is associated with an \emph{interference level}, denoted by  $\InfTot_{\n,\k}$, which reflects the aggregate interference from all other nearby devices (including TV stations
%\footnotesc{{Notice each TV station has the right to transmit on a particular channel within certain coverage area centered around the TV station, and unlicensed users may be allowed to transmit in this coverage \emph{with a strictly constrained power}. Hence, the TV station might generate interference to unlicensed users (whereas the reverse is not allowed).}}
and other {\eus}) operating on this channel.
%For convenience, we also refer to $\InfTot_{\k}$ as the \emph{quality} of channel $k$.
Due to the fast changing of wireless channels and the uncertainty of {\eus}' mobilities and activities, the interference $\InfTot_{\n,\k}$ is a random variable.
For convenience, we assume that
$$
\InfTot_{\n,\k} \mbox{ is \emph{temporal-independence} and \emph{frequency-independence}}.
$$
That is,
(i) the interference $\InfTot_{\n,\k}$ on channel $\k$ is independent identically distributed (iid) at different times, and (ii)
the interferences on different channels, $\InfTot_{\n,\k}, \k\in\Kset$, are also iid at the same time.\footnotesc{Note that the iid assumption is a reasonable approximation of the practical scenario, where all channel quality distributions are the same but the realized instant qualities of different channels are different (e.g., \cite{chang2009channel,jiang2009channel,zhou2011channel}).}
%Under the i.i.d. assumption, we assume that all channel states $\{ \InfTot_{\k} \}_{\k \in \Kset}$ have the same cumulative distribution function (CDF)
As we are talking about a general WSD $n$, \textbf{we will omit the WSD index $n$ in the notations (e.g., write $\InfTot_{\n,\k}$ as $\InfTot_{\k}$), whenever there is no confusion caused.}
Let $F_{\InfTot}(\cdot)$ and $f_{\InfTot}(\cdot)$ denote the cumulative distribution function (CDF) and probability distribution function (PDF) of $\InfTot_{\k}$, $\forall \k\in\Kset$.\footnotesc{In this paper, we will conventionally  use $F_X(\cdot)$ and $f_X(\cdot)$ to denote the CDF and PDF of a random variable $X$, respectively.}~~~~



\textbf{Interference Level (Information).}
{For a particular {\eu}}, its experienced interference $\InfTot_{\k}$ on a channel $k$ is the aggregate interference from all other (nearby) devices operating on channel $k$,
and usually consists of the following three components:
\begin{enumerate}
\item
$\InfTV_{\k}$: the interference from licensed TV stations;
\item
$\InfEU_{\k,m}$: the interference from another {\eu} $m$ operating on the same channel $k$;
\item
$\InfOut_{\k}$: any other interference from outside systems.
\end{enumerate}
%Here $\InfEU_{\n,\k}$ denotes the interference from an {\eu} $\n$ operating on channel $\k$, and
The total interference on channel $k$ is
$
\InfTot_{\k} = \InfTV_k + \InfEU_k + \InfOut_k
$, where  $\InfEU_k  \triangleq \sum_{m \in \Nkset} \InfEU_{\k,m}$ is the total interference from all other {\eus} operating on channel $k$ (denoted by $\Nkset$).
Similar to $\InfTot_{\k}$, we assume that  $ \InfTV_k , \InfEU_k , \InfEU_{\k,m}$, and $ \InfOut_k$ are random variables with \emph{temporal-independence} (i.e., iid across time) and \emph{frequency-independence} (i.e., iid across frequency).
We further assume that $\InfEU_{\k,m}$ is \emph{user-independence}, i.e., $\InfEU_{\k,m}, m\in \Nkset$, are iid.
%Similarly, we assume that $\{ \InfTV_k \}_{\k \in \Kset}$ are i.i.d., with the CDF $F_{\InfTV}(\cdot)$, and
%$\{ \InfOut_k \}_{\k \in \Kset}$, are i.i.d., with the CDF $F_{\InfOut}(\cdot)$.
%Let $F_{\InfTV}(\cdot)$, $F_{\InfEU}(\cdot)$, and $F_{\InfOut}(\cdot)$ denote the CDFs of $ \InfTV_k , \InfEU_{\n,\k}$, and $\InfOut_k $, respectively.
{It is important to note that \textbf{different {\eus} may experience different interferences $\InfTV_k$ (from TV stations), $ \InfEU_{\k,m} $ (from another WSD), and $ \InfOut_k$ (from outside systems) on a channel $k$, as we have omitted the \eu~index $n$ for all these notations for clarity.}}

Next we discuss these interferences in more details.

\begin{itemize}
\item
Each database is able to compute the interference $\InfTV_k$ from TV stations to every {\eu} (on channel $k$), as it knows the locations and channel occupancies of all TV stations.~~~~
%\footnotesc{Here we consider the long-term average interference, not the instantaneous interference. The same applies to {\eu} and outside interference.}

\item
Each database cannot compute the interference
$\InfOut_k$ from outside systems, due to the lack of outside interference source information.
%\footnotesc{Such outside interference may come from WSDs interacting with other databases, different wireless systems operating on the same or nearby frequency bands, etc.}
Thus, the interference $\InfOut_{\k}$ will \emph{not} be included in a database's information sold to {\eus}.~~~~~~~~
%This reduces the accuracy of information.

\item
Each database may or may not be able to compute the interference $\InfEU_{\k,m}$ from another {\eu} $m$, depending on whether {\eu} $m$ subscribes to the database's advanced service.
Specifically, if {\eu} $m$ subscribes to the advanced service, the database can predict its channel selection (since the {\eu} is fully rational and will always choose the channel with the lowest interference level indicated by the database at the time of subscription), and thus can compute its interference to any other \eu.
However, if {\eu} $m$ does not subscribe to the advanced service, the database cannot predict its channel selection, and thus cannot compute its interference to other \eus.~~~~
\end{itemize}


For convenience, we denote $\Nkset^{[l]},l\in\{1,2\}$, as the set of {\eus} operating on channel $k$ and subscribing to the database $\dbb_l$'s advance service (i.e., those choosing the strategy $\l \in\{1,2\}$), and $\Noset$ as the set of {\eus} operating on channel $k$ and \emph{not} subscribing to any advance service (i.e., those choosing the strategy $\l = 0$).
That is, $\Nkset^{[1]} \bigcup \Nkset^{[2]} \bigcup \Noset = \Nkset $.
Then, for a particular WSD, its experienced interference (on channel $k$) \textbf{known by database $\dbb_l$} is
% (and thus will be included in the database $\dbb_i$'s advanced service to this WSD) is
\begin{equation}\label{eq:known_inf}
\begin{aligned}
\textstyle
\InfKnown_{\k}^{[l]} \triangleq \InfTV_{\k} + \sum_{m \in \Nkset^{[l]}} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from TV licensees and all {\eus} (operating on channel $k$)  subscribing to the database $\dbb_l$'s advanced service.
The WSD's experienced interference (on channel $k$) \textbf{\emph{not} known by database $\dbb_l$} is
% (and thus will not be included in the database $\dbb_i$'s advanced information) is
\begin{equation}\label{eq:unknown_inf}
\begin{aligned}
\textstyle
\InfUnknown_{\k}^{[l]}  \triangleq \InfOut_{\k} +\sum_{m \in \Noset} \InfEU_{\k,m} + \sum_{m \in \Nkset^{[i]},i\neq l} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from outside systems and all {\eus} (operating on channel $k$) not subscribing to the database $\dbb_l$'s advanced service.
Obviously, both $\InfUnknown_{\k}^{[l]}$ and $\InfKnown_{\k}^{[l]}$ are also random variables with temporal- and frequency-independence.
Accordingly, the total interference on {\ch} $\k$ for a WSD can be written as
%\begin{equation}\label{eq:total_inf_new}
%\begin{aligned}
$\textstyle
\InfTot_{\k} = \InfKnown_{\k}^{[l]} + \InfUnknown_{\k}^{[l]}.$~~~~~~
% = \InfTV_{\k} +\InfOut_{\k}+ \sum_{n \in \Nkset} \InfEU_{\n,\k}.
%\end{aligned}
%\end{equation}

\textbf{Since the database $\dbb_l$ knows only $\InfKnown_{\k}^{[l]}$, it will provide this information (instead of the total interference $\InfTot_k$) as the {advanced service} to a subscribing {\eu}.}
%to its advanced service.
It is easy to see that the more {\eus} subscribing to the database $\dbb_l$'s advanced service, the more information the database $\dbb_l$ knows, and the more accurate the database $\dbb_l$'s information will be.~~~~~~~~


Next we can characterize the accuracy of a database's information explicitly.
Due to the frequency independence assumption, it is reasonable to assume that each channel $k\in\Kset$ will be occupied by an average of $\frac{\N}{\K}$ {\eus}.
Let $\Prob_l$ denote the percentage of {\eus} subscribing to the advanced service of database $\dbb_l$ (called the \emph{market share} of database $\dbb_l$).
%Notice that each {\eu} will
%be ``assigned'' to each channel with an equal probability due
%to the assumption of the frequency independence.
Then, among all  $\frac{\N}{\K}$ {\eus} operating on channel $k$, there are, \emph{on average}, $\frac{\N}{\K}\cdot\Prob_l$ {\eus}  subscribing to the database $\dbb_l $'s advanced service, and $\frac{\N}{\K}\cdot(1-\Prob_1 -\Prob_2)$ {\eus} not subscribing to any advanced service.
That is, $| \Nkset | = \frac{\N}{\K}$, $| \Nkset^{[l]} | = \frac{\N}{\K}\cdot\Prob_l, \forall l\in\{1,2\}$, and $|\Noset | = \frac{\N}{\K}\cdot(1-\Prob_1-\Prob_2)$.\footnotesc{{Note that the above discussion is from the aspect of expectation, and in a particular time period, the realized numbers of {\eus} in different channels may be different.}}
Finally, by the {user-independence} of $\InfEU_{\k,m}$, we can immediately calculate the distributions of $ \InfKnown_{\k}^{[l]}$ and $ \InfUnknown_{\k}^{[l]}$ under any given market share $\Prob_l$ via (\ref{eq:known_inf}) and (\ref{eq:unknown_inf}).

%That is, there are an average $\N\cdot \Prob_1$ {\eus} subscribing to the $\dbb_1$'s advanced service, $\N\cdot \Prob_2$ {\eus} subscribing to the $\dbb_2$'s advanced service, and $\N\cdot (1-\Prob_1 - \Prob_2)$ {\eus} not subscribing to the advanced service.
%%Suppose the {\eu} number $\N$ is very large, and
%Since the {\eus} are independent with each other,  then, from a system perspective, all the {\eus} will be ``assigned'' to all available channels equally (i.e., $|\Nset_k| = \frac{\N}{\K}$).
%That is,
%on every available channel $k$, there are on average $\frac{\N}{\K}\cdot\Prob_{\i} $ {\eus} subscribing to the advanced serve of database $\i$ (whose interference (to any particular {\eu}) can be computed by the database) where $ \i \in \{ 1, 2\}$, and $\frac{\N}{\K}\cdot(1-\Prob_1 - \Prob_2)$ {\eus} not subscribing to the advanced serve (whose interference cannot be computed by the database)\footnotesc{This is because of the diversity of users' locations as well as their
%environments. The good channels for a user may not be good for others.
%Moreover, even if users share the similarity in the environment, they
%are likely to be directed to different channels for the purpose of
%interference avoidance.}.
%Similarly, we assume that the interference from single {\eu} {$\{\InfEU_{\n, \k}\}_{\n \in \Nkset}$}, are iid with a CDF   $F_{\InfEU}(\cdot)$.
%
%
%%We denote these three kinds of interference for \ch~$\k$ as random variable $\InfTV_{\k}$, and $\InfOut_{\k}$. We let random variable $\InfEU_{\n}$ as \eu $\n$'s interference.
%%We denote these three kinds of interference as random variable $\InfTV$, $\InfOut$, and $\InfEU$, respectively.
%%We also assume $\{ \InfTV_{\k} \}_{\k \in \Kset}$, $\{ \InfOut_{\k} \}_{\k \in \Kset}$, and $\{ \InfEU_{\n} \}_{\n \in \Nset}$ are i.i.d. random variables.
%%Let $F_{\InfTV}(\cdot)$, $F_{\InfOut}(\cdot)$, and $F_{\InfEU}(\cdot)$ denote the CDF of above three random variable. And correspondingly, let $f_{\InfTV}(\cdot)$, $f_{\InfOut}(\cdot)$, and $f_{\InfEU}(\cdot)$ denote their probability density function (PDF).
%
%%As we assume the total number of \eus~$\N$ is very large, we can consider \eus~are uniformly assign to each \ch,~i.e., there are ${ \N }/{\K}$ \eus~in each \ch.
%%Hence, the total interference level of \ch~$\k$ is:
%%\begin{equation}\label{eq:total_inf}
%%\begin{aligned}
%%%\textstyle
%%\vspace{2mm}
%%\InfTot_{\k} \triangleq \InfTV_{\k} +\InfOut_{\k}+ \frac{\N}{\K} \cdot \InfEU
%%\vspace{2mm}
%%\end{aligned}
%%\end{equation}
%
%%Since every \eu~needs to report its location to \db, \db~can calculate the TV station's interference to each \eu. Hence, \db~knows the distribution of $\InfTV$.
%%As we assume that advanced \eu~will choose the \ch~with highest ranking, therefore, \db~can also calculate the total interference caused by advanced \eu. We denote $\Prob$ as the percentage of advanced \eus \footnotesc{"percentage of advanced \eus" is used throughout this paper to mean the proportion of \eus~in the market that subscribe to advanced service}~. Then, the number of advanced \eus~is $\N \cdot \Prob$. As we assume $\N$ is very large, we can consider both advanced \eus~and basic \eus~are uniformly assign to each \ch,~i.e., there are $\frac{ \N \cdot \Prob }{\K}$ advanced \eus~and $\frac{ \N \cdot (1-\Prob) }{\K}$ basic \eus~in each \ch.
%
%In summary, for each \ch~$\k$, the interference level known by the \db~$\i$ is
%\begin{equation}\label{eq:known_inf}
%\begin{aligned}
%\textstyle
%\InfKnown^{\i}_{\k} \triangleq \InfTV^{\i}_{\k} + \sum_{n \in \Naiset} \InfEU_{\n, \k}~\i = \{ 1 , 2\}.
%%\sum_{n=1}^{\frac{ \N }{\K}  \cdot \Prob_{\i}} \InfEU_{n},~\i = \{ 1 , 2\}.
%\end{aligned}
%\end{equation}
%The interference level not known by the \db~$\i$ is
%\begin{equation}\label{eq:unknown_inf}
%\begin{aligned}
%\textstyle
%\InfUnknown^{\i}_{\k} \triangleq \InfOut^{\i}_{\k} + \sum_{n \in \Noset} \InfEU_{n, \k} + \sum_{n \in \Najset} \InfEU_{n, \k}~\j \neq \i.
%%\InfUnknown^{\i}_{\k} \triangleq \InfOut^{\i}_{\k} + \sum_{n=1}^{\frac{ \N  }{\K}\cdot (1 - \Prob_{\i} - \Prob_{\j})} \InfEU_{n} + \sum_{n=1}^{\frac{ \N  }{\K}\cdot \Prob_{\j}} \InfEU_{n}~\j \neq \i.
%\end{aligned}
%\end{equation}
%The total interference level  on  \ch~$\k$ is
%\begin{equation}\label{eq:total_inf_new}
%\begin{aligned}
%\textstyle
%\InfTot_{\k} = \InfKnown_{\k} + \InfUnknown_{\k} = \InfTV_{\k} +\InfOut_{\k}+ \sum_{n \in \Nkset} \InfEU_{\n,\k}
%\end{aligned}
%\end{equation}
%where $\Naiset$ denotes the set of {\eus} operating on the channel $k$ and subscribing to the advance service of database $\i$; $\Najset$ denotes the set of {\eus} operating on the channel $k$ and subscribing to the advance service of database $\j \neq \i$; $\Noset$ denotes the set of {\eus} operating on the same channel $k$ and not subscribing to the advance service of both database, and $\Nkset$ denotes the set of {\eus} operating on the same channel $k$. Besides, we have $|\Naiset| = \frac{N}{K}\cdot{\eta_i}$, $|\Najset| = \frac{N}{K}\cdot{\eta_j}$, and $|\Noset| = \frac{N}{K}\cdot( 1 - \eta_1 - \eta_2)$. Moreover, we have $\i, \j \in \{1 ,2 \}$, $\i \neq \j$, $\Nkset = \Naiset \bigcup \Najset \bigcup \Noset$, and $\Naiset \bigcap \Najset \bigcap \Noset = \emptyset$.
%The database knows the precise value of $\InfKnown_{\k}$ on every channel $k$, which will be provided for {\eus} who subscribing to the advanced service.
%It is easy to see that the more {\eus} subscribing to this advanced service, the more accurate the advanced information will be.
%%It is assumed that the \db~knows the realized value of $\InfKnown_{\k}$.
%{
%By the iid assumption on $\InfTV_{\k}$, $\InfEU_{\n,\k}$, and $\InfOut_{\k}$, we can easily find that (i) $\{ \InfKnown_{\k} \}_{ \k\in\Kset }$, are i.i.d., (ii) $\{ \InfUnknown_{\k}\}_{\k\in\Kset}$, are i.i.d., and (iii) $\{ \InfTot_{\k} \}_{ \k\in\Kset }$, are i.i.d..
%Finally, we assume that both the \db~and \eus~knows \emph{a priori} the distributions of $\InfTV_{\k}$, $\InfEU_{\n,\k}$, and $\InfOut_{\k}$, and therefore the distributions of $\InfKnown_{\k}$, $\InfUnknown_{\k}$, and $\InfTot_{\k}$ given the market share $\Prob$.
%}

\textbf{Information Value.}
Now we evaluate the value of database $\dbb_l$'s information to {\eus}, which is
reflected by the {\eu}'s benefit (utility) that can be achieved from this information.

We first consider the expected  utility of a {\eu} when not subscribing to any advanced service (i.e., $\l=0$).
In this case, the {\eu} will randomly select a channel from the available channel list, and its expected utility is
\begin{equation}\label{eq:rate-random-fixed}
\begin{aligned}
\textstyle
\RB   \textstyle \triangleq \ut(\R_0) = \ut\left(\int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z)\right),
%& \textstyle = \ut\left( \Ex_{\InfTot} \big[ \rt \left( \InfTot_{\k} \right) \big] \right)
%\\
%& \textstyle = \ut\left( \int_{z} \rt(z) \cdot f_{\InfTot}(z) \cdot \mathrm{d}z \right).
%\vspace{8mm}
\end{aligned}
\end{equation}
where $\R_0$ is the expected data rate given in (\ref{eq:rkgs}).
%By (\ref{eq:total_inf_new}), the distribution of $\InfTot$ is independent of the percentage of advanced {\eus} $\Prob$. Therefore, the value of $\RB$ is also independent of $\Prob$.
%and for an {\eu} with $\l = \S$, its expected utility is
%\begin{equation}\label{eq:rate-sense-fixed}
%\begin{aligned}
%\RS  & \textstyle  \triangleq \ut\left(\Rks\right) ,
%%=  \ut\left( \Ex_{\InfTotMin} \big[ \rt \left(\InfTotMin \right) \big] \right)
%%\\
%%&\textstyle= \ut\big( \K  \int_z \rt(z) \cdot [ 1 - F_{\InfTot}(z)]^{\K - 1} \cdot f_{\InfTot}(z) \cdot \mathrm{d}z \big),
%%\vspace{8mm}
%\end{aligned}
%\end{equation}
%where $\R^{(\G_i)} $ is the expected data rates defined in (\ref{eq:rkgs}).
Obviously, $\RB$ depends only on the distribution of the total interference $\InfTot_k$, while not on the specific distributions of $\InfKnown_k^{[l]}$ and $\InfUnknown_k^{[l]}$. This implies that the accuracy of the database $\dbb_l$'s information does not affect the utilities of those {\eus} not subscribing to its advanced service.


Then we consider the expected utility of a {\eu} when subscribing to the database $\dbb_l$'s advance service (i.e., $\l\in\{1,2\}$).
In this case, the {\db} $\dbb_l$ returns the interference $\{\InfKnown_{k}^{[l]}\}_{k\in\Kset}$ to the {\eu}, together with the basic information such as the available channel list.
%Notice that the total interference also includes the interference $\{\InfUnknown_{k}\}_{k\in\Kset} $ not provided by the database.
%\db~ranks the  {\chs} in ascending order given {\ch} interference level it known (i.e., $\InfKnown_{1}, \InfKnown_{2}, \ldots, \InfKnown_{\K} $). The ranked interference level are denoted by $\InfKnown_{(1)}, \InfKnown_{(2)}, \ldots, \InfKnown_{(\K)}$ and satisfy $\InfKnown_{(1)} < \ldots< \InfKnown_{(\K)}$.
For a rational {\eu}, it will always choose the channel with the minimum $\InfKnown_{k}^{[l]}$ (since $\{\InfUnknown_{k}^{[l]}\}_{k\in\Kset}$ are iid).
%\footnote{This is because the uncertain interference $\{\InfUnknown_{k}\}_{k\in\Kset} $ are i.i.d.}
Let $\InfKnownMin^{[l]} =  \min\{ \InfKnown_{1}^{[l]},  \ldots, \InfKnown_{K}^{[l]}  \} $ denote the minimum interference indicated by the database $\dbb_l$'s information.
Then, the actual interference experienced by a {\eu} (subscribing to the database $\dbb_l$'s advanced service) can be formulated as the sum of two random variables, denoted by $\InfTot^{[l]} = \InfKnownMin^{[l]} + \InfUnknown$. Accordingly, the {\eu}'s expected data rate and expected utility under the strategy $l\in\{1,2\}$ can be computed by
%Hence, the advanced {\eus} transmit at the {\ch} with lowest $\InfKnown$ and with total interference level $\InfTotA = \InfKnownMin + \InfUnknown$. Therefore, the advanced \eu's expect data rate is
\begin{equation}\label{eq:rate-pay-fixed}
\begin{aligned}
\Rl & \textstyle = \Ex_{\InfTot^{[l]}} \big[ \rt \left(\InfTot^{[l]} \right) \big] = \int_z \rt(z)  \mathrm{d} F_{\InfTot ^{[l]}}(z),
\\
\RA_l & \textstyle  \triangleq \ut\left(\Rl\right) = \ut\left(\int_z \rt(z)  \mathrm{d} F_{\InfTot ^{[l]}}(z)	\right) ,
% \textstyle =  \ut\left(\Ex_{\InfTotA} \big[ \rt \left(\InfTotA \right) \big] \right),
%\\
%&= \Ex_{\InfTotA} \big[ \rt \big( \InfKnownMin + \InfUnknown \big) \big] \\
%&= \K \cdot \int_{\InfTotA} \rt(z) \cdot \big[ \int_{\infty}^{\infty} f_{\InfKnown}(z -y) \cdot [ 1 - F_{\InfKnown}(y)]^{K-1} \cdot f_{\InfUnknown}(y) \mathrm{d}y  \big] \mathrm{d}z
%& \textstyle  = \ut \big( \int_z \rt(z) \cdot f_{\InfTotA}(z) \cdot \mathrm{d}z \big),
%\vspace{8mm}
\end{aligned}
\end{equation}
where
 $F_{\InfTot^{[l]}}(z)$ is the CDF of $\InfTot^{[l]}$.
% , and defined by
%\begin{equation*}\label{eq:min-known-pdf}
%%\begin{aligned}
%\textstyle
%f_{\InfTotA}(z) = \K   \int_y \big[ 1 - F_{\InfKnown}(z - y) \big]^{K-1} \cdot f_{\InfKnown}(z -y) \cdot f_{\InfUnknown}(y) \cdot \mathrm{d}y.
%%\vspace{8mm}
%%\end{aligned}
%\end{equation*}
It is easy to see that both $\Rl$ and $\RA_l$ depend on the distributions of $\InfKnown_k^{[l]}$ and $\InfUnknown_k^{[l]}$, and thus depend on the market share $\Prob_l$.
Thus, we will write $\RA_l$ as $\RA_l(\Prob_l)$.
We can further check that $\RA_l(\Prob_l)$ increases with $\Prob_l$.~~~~
%, because the more {\eus} subscribing to the database $\dbb_i$'s advanced service, the more accurate the database $\dbb_i$'s information, and further the more benefit for the {\eus} subscribing to the database $\dbb_i$'s advanced service.
%For convenience, we assume that $\RA_l(\Prob_l)$ is concave in $\Prob_l$ \rev{\footnote{This is validated by the simulation}}.~~~~~~~~~~~


%By (\ref{eq:rate-random-fixed})--(\ref{eq:rate-pay-fixed}), we can find the following useful properties.
%%, which are very important for the later analysis.
%
%\begin{proposition}
%%[Properties of $\RA, \RB, \RS$]
%\label{prop:ABS}
%~
%\begin{itemize}
%\item
% $\RB$ in (\ref{eq:rate-random-fixed})  does not depend on $\Prob_i$, $i\in\{1,2\}$;
% \item
% $\RA_i(\Prob_i)$ in (\ref{eq:rate-pay-fixed}) monotonously increases with $\Prob_i$;
% \item
% $\RA_i(\Prob_i) \geq \RB $, $\forall \Prob_i \in [0, 1]$;
% \item
%$\RA_i(\Prob_i)  = \RB$, only when $\Prob_i=0$ and meanwhile there is no licensee interference $\{ \InfTV_{\k} \}_{k\in\Kset}$.
%\end{itemize}
%\end{proposition}
%
%
%
%Then we consider the expected data rate of the \eus~who subscribe to the advance service (i.e., $\l=\A_{\i}, \i \in \{ 1, 2 \}$).
%With this advanced service, the \db~$\i$ returns the interference $\{ \InfKnown^{\i}_{k}\}_{k\in\Kset}$ to {\eus}, together with the basic information such as the available channel list.
%Notice that the actual interference also includes the interference part $\{\InfUnknown^{\i}_{k}\}_{k\in\Kset} $ not known by the database $\i$.
%%\db~ranks the \chs~in ascending order given \ch~interference level it known (i.e., $\InfKnown_{1}, \InfKnown_{2}, \ldots, \InfKnown_{\K} $). The ranked interference level are denoted by $\InfKnown_{(1)}, \InfKnown_{(2)}, \ldots, \InfKnown_{(\K)}$ and satisfy $\InfKnown_{(1)} < \ldots< \InfKnown_{(\K)}$.
%For a rational {\eu}, he will always choose the channel with the lowest $\InfKnown^{\i}_{k}$ provided~by~the~database.\footnotesc{This is because the uncertain interference $\{\InfUnknown^{\i}_{k}\}_{k\in\Kset} $ are i.i.d.}
%Let $\InfKnownMin^{\i} =  \min\{ \InfKnown^{\i}_{1},  \ldots, \InfKnown^{\i}_{\k}  \} $ denote the lowest interference provided by the database.
%Then, the actual interference experienced by the {\eu} is $\InfTotA^{\i} = \InfKnownMin^{\i} + \InfUnknown$, and accordingly the expected data rate is
%%Hence, the advanced \eus~transmit at the \ch~with lowest $\InfKnown$ and with total interference level $\InfTotA = \InfKnownMin + \InfUnknown$. Therefore, the advanced \eu's expect data rate is
%\begin{equation}\label{eq:rate-pay-fixed}
%\begin{aligned}
%\ut(\R^{\A_{\i}})  = \RA^{\i} & \textstyle \triangleq \ut( \Ex_{\InfTotA^{\i}} \big[ \rt \big(\InfKnownMin^{\i} + \InfUnknown^{\i} \big) \big] ) \\
%%&= \Ex_{\InfTotA} \big[ \rt \big( \InfKnownMin + \InfUnknown \big) \big] \\
%%&= \K \cdot \int_{\InfTotA} \rt(z) \cdot \big[ \int_{\infty}^{\infty} f_{\InfKnown}(z -y) \cdot [ 1 - F_{\InfKnown}(y)]^{K-1} \cdot f_{\InfUnknown}(y) \mathrm{d}y  \big] \mathrm{d}z
%& \textstyle  = \ut( \int_{\InfTotA^{\i}} \rt(z) \cdot h(z) \cdot \mathrm{d}z ),
%%\vspace{8mm}
%\end{aligned}
%\end{equation}
%where
% $h(\cdot)$ is the pdf of $\InfTotA^{\i}$, defined by
%\begin{equation*}\label{eq:min-known-pdf}
%%\begin{aligned}
%\textstyle
%h(z) = \K \cdot \int f_{\InfKnown^{\i}}(z -y) \cdot \big[ 1 - F_{\InfKnown^{\i}}(z - y) \big]^{K-1} \cdot f_{\InfUnknown^{\i}}(y) \cdot \mathrm{d}y.
%%\vspace{8mm}
%%\end{aligned}
%\end{equation*}
%By (\ref{eq:rate-pay-fixed}), we can see that $\RA^{\i}$ depends on the distributions of $\InfKnown^{\i}_k$ and $\InfUnknown^{\i}_k$, and accordingly depends on the market share $\Prob_{\i}$ (and thus, we will also write $\RA^{\i}$ as $\RA(\Prob_{\i})$).
%We can further check that $\RA(\Prob_{\i})$ increases with $\Prob_{\i}$. This is because the more {\eus} subscribing to the advanced service,  the more accurate the database's information is, and further the more benefit for the {\eus} subscribing to the advanced service. We can also note that if two database $\dbb_1$ and $\dbb_2$ share their market shared information, both of them can obtain more accurate information. However, they compete for the same pool of {\eus}. Sharing the information may lead to the decreasing of their own profit.

%Based on the above, we can find the following useful properties, which are very important for the later analysis.
%\begin{proposition}\label{prop:ABS}
%~
%\begin{itemize}
%\item
% $\RB$ in (\ref{eq:rate-random-fixed}) and $\RS$ in (\ref{eq:rate-sense-fixed}) do not depend on $\Prob$;
% \item
% $\RA(\Prob)$ in (\ref{eq:rate-pay-fixed}) monotonously increases with $\Prob$;
% \item
% $\RB\leq \RA(\Prob) \leq \RS $, $\forall \Prob \in [0, 1]$;
% \item
%$\RA(1)  = \RS$, if no outside interference $\{ \InfOut_{\k} \}_{k\in\Kset}$;
% \item
%$\RA(0)  = \RB$, if no licensee interference $\{ \InfTV_{\k} \}_{k\in\Kset}$.
%\end{itemize}
%\end{proposition}




\textbf{Problem Formulation.}
Suppose that each {\eu} is rational, and will always choose the strategy that maximizes its payoff.
We are interested in the following problems: given the information prices $\{\p_1, \p_2\}$ and initial market shares $\{\Prob^0_1, \Prob^0_2 \}$ of databases, how these market shares dynamically evolve and what is the market equilibrium?

%We will study the oligopoly price competition game between databases $\dbb_1$ and $\dbb_2$.
%In the proposed oligopoly price competition game, each database $\dbb_i$ chooses the price $\p_i$ for its information, aiming at maximizing its revenue
%$$
%\Udb_i = \p_i\cdot \Prob_i \cdot N.
%$$
%%given the distributions of licensee interference $\InfTV_{\k}$, outside interference $\InfOut_{\k}$, and single {\eu} interference $\InfEU_{\n,\k}$.
%Note that the market share $\Prob_i $ of the database $\dbb_i$ depends not only on its own price $\p_i$, but also on the other database $\dbb_j$'s price $\p_j$, and thus can be written as $\Prob_i(\p_1, \p_2)$.
%Moreover, the change of $\Prob_i$ will affect the distributions of $\InfKnown_k^i$ (known by the database $\dbb_i$) and $\InfUnknown_k^i$ (not known by the database $\dbb_i$), which in turn will affect the {\eu}'s utility $\RA_i(\Prob_i)$ achieved from the database $\dbb_i$'s advanced service.

%
%revenue maximization where two database compete by choosing prices, given the distributions of licensee interference $\InfTV_{\k}$, outside interference $\InfOut_{\k}$, and single {\eu} interference $\InfEU_{\n}$.
%For database $\i$, its {revenue} is $\p_{\i} \cdot \Prob_{\i}(\bp) \cdot N$.
%%optimal information pricing plan (i.e., $\p_1$ and $\p_2$) that maximizes the database's
%Notice that the database $\dbb_{\i}$'s market share $\Prob_{\i}(\bp)$ is a function of $\bp = (\p_1, \p_2)$.
%Moreover, the change of $\BProb$ will affect the interference levels $\InfKnown^{\i}_k$ (known by the database) and $\InfUnknown^{\i}_k$ (not known by the database), which in turn will affect the {\eu}'s expected data rate $\RA^{\i}(\BProb)$ achieved from the advanced service, and the {\eu}'s decision.

% (ii)
%By comparing (\ref{eq:rate-random-fixed}), (\ref{eq:rate-sense-fixed}), and (\ref{eq:rate-pay-fixed}), we have $\RB \leq \RA \leq \RS$
%When the random variable $\InfKnown$ is zero, we have $\RA = \RB$. Otherwise, $\RA > \RB$, $\forall \Prob \in [0,1]$. If the value of $\InfUnknown$ is zero, we have $\RA = \RS$. Otherwise, $\RA < \RS$, $\forall \Prob \in [0,1]$.

%We associate interference caused by TV station denoted by $\InfTV$, which is a random variable follows from a continuous distribution with cdf $F_{\InfTV}(\cdot) $ and pdf $f_{\InfTV}(\cdot)$. $\InfOut$ represents the interference cause by other database's {\eus} and is a random variable follows from a continuous distribution with cdf $F_{\InfOut}(\cdot) $ and pdf $f_{\InfOut}(\cdot)$ and represents the interference cause by other database's {\eus}. For particular {\eu}, we assume its receiving interference from each {\eu} in the same network \footnotesc{We assume {\eus} who connect to the same database acting in the same network.} $Y$ is a random variable with cdf $F_{Y}(\cdot) $ and pdf $f_{Y}(\cdot)$.



==> Section_network_effect.tex <==

\section{The Value of Information and the Network Effect}
%If a \eu~chooses operating on TV \ch, it can only operate on one of the available TV \chs from the \ch~set $\Kset = \{ 1,\ldots, \K \}$ at a particular time on the shared basis (i.e., each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques).
%Let $\Kset = \{ 1,\ldots, \K \}$ denote the set of available TV channels in this area. One \eu~can only operate on \emph{one} of the available \chs~at a particular time on the shared basis (i.e., each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques).
%
%Each \eu~makes its choice through the online platform provided by a \db. We assume that a \db~has the available TV \chs~information and provides such information to each querying \eu~in order to let the \eu~operate on \emph{one} of the available \chs~at a particular time. Note that each \ch~is can be used by multiple \eus~ simultaneously using CDMA or CSMA techniques.
%We also assume that the licensed spectrum holders display their licensed spectrum

For each {\eu} $n\in \Nset$, each channel $\k$ is associated with an \emph{interference level}, denoted by  $\InfTot_{\n,\k}$, which reflects the aggregate interference from all other nearby devices (including TV stations
%\footnotesc{{Notice each TV station has the right to transmit on a particular channel within certain coverage area centered around the TV station, and unlicensed users may be allowed to transmit in this coverage \emph{with a strictly constrained power}. Hence, the TV station might generate interference to unlicensed users (whereas the reverse is not allowed).}}
and other {\eus}) operating on this channel.
%For convenience, we also refer to $\InfTot_{\k}$ as the \emph{quality} of channel $k$.
Due to the fast changing of wireless channels and the uncertainty of {\eus}' mobilities and activities, the interference $\InfTot_{\n,\k}$ is a random variable.
For convenience, we assume that
$$
\InfTot_{\n,\k} \mbox{ is \emph{temporal-independence} and \emph{frequency-independence}}.
$$
That is,
(i) the interference $\InfTot_{\n,\k}$ on channel $\k$ is independent identically distributed (iid) at different times, and (ii)
the interferences on different channels, $\InfTot_{\n,\k}, \k\in\Kset$, are also iid at the same time.\footnotesc{Note that the iid assumption is a reasonable approximation of the practical scenario, where all channel quality distributions are the same but the realized instant qualities of different channels are different (e.g., \cite{chang2009channel,jiang2009channel,zhou2011channel}).}
%Under the i.i.d. assumption, we assume that all channel states $\{ \InfTot_{\k} \}_{\k \in \Kset}$ have the same cumulative distribution function (CDF)
As we are talking about a general WSD $n$, \textbf{we will omit the WSD index $n$ in the notations (e.g., write $\InfTot_{\n,\k}$ as $\InfTot_{\k}$), whenever there is no confusion caused.}
Let $F_{\InfTot}(\cdot)$ and $f_{\InfTot}(\cdot)$ denote the cumulative distribution function (CDF) and probability distribution function (PDF) of $\InfTot_{\k}$, $\forall \k\in\Kset$.\footnotesc{In this paper, we will conventionally  use $F_X(\cdot)$ and $f_X(\cdot)$ to denote the CDF and PDF of a random variable $X$, respectively.}~~~~

For convenience, we illustrate the basic service and advanced service by the example in the following table.
In the basic service, the database provides the available channel set (i.e., \{CH1, CH3, CH4, CH6\}) to a particular \eu. In the advanced service, the database provides the interference levels on available channels (i.e., \{$\InfTot_1$, $\InfTot_3$, $\InfTot_4$, $\InfTot_6$\}) to the \eu, in addition to the available channel set.

\begin{table}[h]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Channel ID} & \textbf{CH1}& \textbf{CH2}& \textbf{CH3} & \textbf{CH4} & \textbf{CH5} & \textbf{CH6}
\\
\hline
Availability & Yes & No & Yes & Yes & No & Yes
\\
\hline
Interference Level & $\InfTot_1$ &  - & $\InfTot_3$ & $\InfTot_4$ &  - & $\InfTot_6$
\\
\hline
\end{tabular}
\end{table}


\textbf{Interference Level (Information).}
{For a particular {\eu}}, its experienced interference $\InfTot_{\k}$ on a channel $k$ is the aggregate interference from all other (nearby) devices operating on channel $k$,
and usually consists of the following three components:
\begin{enumerate}
\item
$\InfTV_{\k}$: the interference from licensed TV stations;
\item
$\InfEU_{\k,m}$: the interference from another {\eu} $m$ operating on the same channel $k$;
\item
$\InfOut_{\k}$: any other interference from outside systems.
\end{enumerate}
%Here $\InfEU_{\n,\k}$ denotes the interference from an {\eu} $\n$ operating on channel $\k$, and
The total interference on channel $k$ is
$
\InfTot_{\k} = \InfTV_k + \InfEU_k + \InfOut_k
$, where  $\InfEU_k  \triangleq \sum_{m \in \Nkset} \InfEU_{\k,m}$ is the total interference from all other {\eus} operating on channel $k$ (denoted by $\Nkset$).
Similar to $\InfTot_{\k}$, we assume that  $ \InfTV_k , \InfEU_k , \InfEU_{\k,m}$, and $ \InfOut_k$ are random variables with \emph{temporal-independence} (i.e., iid across time) and \emph{frequency-independence} (i.e., iid across frequency).
We further assume that $\InfEU_{\k,m}$ is \emph{user-independence}, i.e., $\InfEU_{\k,m}, m\in \Nkset$, are iid.
%Similarly, we assume that $\{ \InfTV_k \}_{\k \in \Kset}$ are i.i.d., with the CDF $F_{\InfTV}(\cdot)$, and
%$\{ \InfOut_k \}_{\k \in \Kset}$, are i.i.d., with the CDF $F_{\InfOut}(\cdot)$.
%Let $F_{\InfTV}(\cdot)$, $F_{\InfEU}(\cdot)$, and $F_{\InfOut}(\cdot)$ denote the CDFs of $ \InfTV_k , \InfEU_{\n,\k}$, and $\InfOut_k $, respectively.
{It is important to note that \textbf{different {\eus} may experience different interferences $\InfTV_k$ (from TV stations), $ \InfEU_{\k,m} $ (from another WSD), and $ \InfOut_k$ (from outside systems) on a channel $k$, as we have omitted the \eu~index $n$ for all these notations for clarity.}}

Next we discuss these interferences in more details.

\begin{itemize}
\item
Each database is able to compute the interference $\InfTV_k$ from TV stations to every {\eu} (on channel $k$), as it knows the locations and channel occupancies of all TV stations.~~~~
%\footnotesc{Here we consider the long-term average interference, not the instantaneous interference. The same applies to {\eu} and outside interference.}

\item
Each database cannot compute the interference
$\InfOut_k$ from outside systems, due to the lack of outside interference source information.
%\footnotesc{Such outside interference may come from WSDs interacting with other databases, different wireless systems operating on the same or nearby frequency bands, etc.}
Thus, the interference $\InfOut_{\k}$ will \emph{not} be included in a database's information sold to {\eus}.~~~~~~~~
%This reduces the accuracy of information.

\item
Each database may or may not be able to compute the interference $\InfEU_{\k,m}$ from another {\eu} $m$, depending on whether {\eu} $m$ subscribes to the database's advanced service.
Specifically, if {\eu} $m$ subscribes to the advanced service, the database can predict its channel selection (since the {\eu} is fully rational and will always choose the channel with the lowest interference level indicated by the database at the time of subscription), and thus can compute its interference to any other \eu.
However, if {\eu} $m$ does not subscribe to the advanced service, the database cannot predict its channel selection, and thus cannot compute its interference to other \eus.~~~~
\end{itemize}


For convenience, we denote $\Nkset^{[l]},l\in\{1,2\}$, as the set of {\eus} operating on channel $k$ and subscribing to the database $\dbb_l$'s advance service (i.e., those choosing the strategy $\l \in\{1,2\}$), and $\Noset$ as the set of {\eus} operating on channel $k$ and \emph{not} subscribing to any advance service (i.e., those choosing the strategy $\l = 0$).
That is, $\Nkset^{[1]} \bigcup \Nkset^{[2]} \bigcup \Noset = \Nkset $.
Then, for a particular WSD, its experienced interference (on channel $k$) \textbf{known by database $\dbb_l$} is
% (and thus will be included in the database $\dbb_i$'s advanced service to this WSD) is
\begin{equation}\label{eq:known_inf}
\begin{aligned}
\textstyle
\InfKnown_{\k}^{[l]} \triangleq \InfTV_{\k} + \sum_{m \in \Nkset^{[l]}} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from TV licensees and all {\eus} (operating on channel $k$)  subscribing to the database $\dbb_l$'s advanced service.
The WSD's experienced interference (on channel $k$) \textbf{\emph{not} known by database $\dbb_l$} is
% (and thus will not be included in the database $\dbb_i$'s advanced information) is
\begin{equation}\label{eq:unknown_inf}
\begin{aligned}
\textstyle
\InfUnknown_{\k}^{[l]}  \triangleq \InfOut_{\k} +\sum_{m \in \Noset} \InfEU_{\k,m} + \sum_{m \in \Nkset^{[i]},i\neq l} \InfEU_{\k,m},
\end{aligned}
\end{equation}
which contains the interference from outside systems and all {\eus} (operating on channel $k$) not subscribing to the database $\dbb_l$'s advanced service.
Obviously, both $\InfUnknown_{\k}^{[l]}$ and $\InfKnown_{\k}^{[l]}$ are also random variables with temporal- and frequency-independence.
Accordingly, the total interference on {\ch} $\k$ for a WSD can be written as
%\begin{equation}\label{eq:total_inf_new}
%\begin{aligned}
$\textstyle
\InfTot_{\k} = \InfKnown_{\k}^{[l]} + \InfUnknown_{\k}^{[l]}.$~~~~~~
% = \InfTV_{\k} +\InfOut_{\k}+ \sum_{n \in \Nkset} \InfEU_{\n,\k}.
%\end{aligned}
%\end{equation}

\textbf{Since the database $\dbb_l$ knows only $\InfKnown_{\k}^{[l]}$, it will provide this information (instead of the total interference $\InfTot_k$) as the {advanced service} to a subscribing {\eu}.}
%to its advanced service.
It is easy to see that the more {\eus} subscribing to the database $\dbb_l$'s advanced service, the more information the database $\dbb_l$ knows, and the more accurate the database $\dbb_l$'s information will be.~~~~~~~~


Next we can characterize the accuracy of a database's information explicitly.
Due to the frequency independence assumption, it is reasonable to assume that each channel $k\in\Kset$ will be occupied by an average of $\frac{\N}{\K}$ {\eus}.
Let $\Prob_l$ denote the percentage of {\eus} subscribing to the advanced service of database $\dbb_l$ (called the \emph{market share} of database $\dbb_l$).
%Notice that each {\eu} will
%be ``assigned'' to each channel with an equal probability due
%to the assumption of the frequency independence.
Then, among all  $\frac{\N}{\K}$ {\eus} operating on channel $k$, there are, \emph{on average}, $\frac{\N}{\K}\cdot\Prob_l$ {\eus}  subscribing to the database $\dbb_l $'s advanced service, and $\frac{\N}{\K}\cdot(1-\Prob_1 -\Prob_2)$ {\eus} not subscribing to any advanced service.
That is, $| \Nkset | = \frac{\N}{\K}$, $| \Nkset^{[l]} | = \frac{\N}{\K}\cdot\Prob_l, \forall l\in\{1,2\}$, and $|\Noset | = \frac{\N}{\K}\cdot(1-\Prob_1-\Prob_2)$.\footnotesc{{Note that the above discussion is from the aspect of expectation, and in a particular time period, the realized numbers of {\eus} in different channels may be different.}}
Finally, by the {user-independence} of $\InfEU_{\k,m}$, we can immediately calculate the distributions of $ \InfKnown_{\k}^{[l]}$ and $ \InfUnknown_{\k}^{[l]}$ under any given market share $\Prob_l$ via (\ref{eq:known_inf}) and (\ref{eq:unknown_inf}).

%That is, there are an average $\N\cdot \Prob_1$ {\eus} subscribing to the $\dbb_1$'s advanced service, $\N\cdot \Prob_2$ {\eus} subscribing to the $\dbb_2$'s advanced service, and $\N\cdot (1-\Prob_1 - \Prob_2)$ {\eus} not subscribing to the advanced service.
%%Suppose the {\eu} number $\N$ is very large, and
%Since the {\eus} are independent with each other,  then, from a system perspective, all the {\eus} will be ``assigned'' to all available channels equally (i.e., $|\Nset_k| = \frac{\N}{\K}$).
%That is,
%on every available channel $k$, there are on average $\frac{\N}{\K}\cdot\Prob_{\i} $ {\eus} subscribing to the advanced serve of database $\i$ (whose interference (to any particular {\eu}) can be computed by the database) where $ \i \in \{ 1, 2\}$, and $\frac{\N}{\K}\cdot(1-\Prob_1 - \Prob_2)$ {\eus} not subscribing to the advanced serve (whose interference cannot be computed by the database)\footnotesc{This is because of the diversity of users' locations as well as their
%environments. The good channels for a user may not be good for others.
%Moreover, even if users share the similarity in the environment, they
%are likely to be directed to different channels for the purpose of
%interference avoidance.}.
%Similarly, we assume that the interference from single {\eu} {$\{\InfEU_{\n, \k}\}_{\n \in \Nkset}$}, are iid with a CDF   $F_{\InfEU}(\cdot)$.
%
%
%%We denote these three kinds of interference for \ch~$\k$ as random variable $\InfTV_{\k}$, and $\InfOut_{\k}$. We let random variable $\InfEU_{\n}$ as \eu $\n$'s interference.
%%We denote these three kinds of interference as random variable $\InfTV$, $\InfOut$, and $\InfEU$, respectively.
%%We also assume $\{ \InfTV_{\k} \}_{\k \in \Kset}$, $\{ \InfOut_{\k} \}_{\k \in \Kset}$, and $\{ \InfEU_{\n} \}_{\n \in \Nset}$ are i.i.d. random variables.
%%Let $F_{\InfTV}(\cdot)$, $F_{\InfOut}(\cdot)$, and $F_{\InfEU}(\cdot)$ denote the CDF of above three random variable. And correspondingly, let $f_{\InfTV}(\cdot)$, $f_{\InfOut}(\cdot)$, and $f_{\InfEU}(\cdot)$ denote their probability density function (PDF).
%
%%As we assume the total number of \eus~$\N$ is very large, we can consider \eus~are uniformly assign to each \ch,~i.e., there are ${ \N }/{\K}$ \eus~in each \ch.
%%Hence, the total interference level of \ch~$\k$ is:
%%\begin{equation}\label{eq:total_inf}
%%\begin{aligned}
%%%\textstyle
%%\vspace{2mm}
%%\InfTot_{\k} \triangleq \InfTV_{\k} +\InfOut_{\k}+ \frac{\N}{\K} \cdot \InfEU
%%\vspace{2mm}
%%\end{aligned}
%%\end{equation}
%
%%Since every \eu~needs to report its location to \db, \db~can calculate the TV station's interference to each \eu. Hence, \db~knows the distribution of $\InfTV$.
%%As we assume that advanced \eu~will choose the \ch~with highest ranking, therefore, \db~can also calculate the total interference caused by advanced \eu. We denote $\Prob$ as the percentage of advanced \eus \footnotesc{"percentage of advanced \eus" is used throughout this paper to mean the proportion of \eus~in the market that subscribe to advanced service}~. Then, the number of advanced \eus~is $\N \cdot \Prob$. As we assume $\N$ is very large, we can consider both advanced \eus~and basic \eus~are uniformly assign to each \ch,~i.e., there are $\frac{ \N \cdot \Prob }{\K}$ advanced \eus~and $\frac{ \N \cdot (1-\Prob) }{\K}$ basic \eus~in each \ch.
%
%In summary, for each \ch~$\k$, the interference level known by the \db~$\i$ is
%\begin{equation}\label{eq:known_inf}
%\begin{aligned}
%\textstyle
%\InfKnown^{\i}_{\k} \triangleq \InfTV^{\i}_{\k} + \sum_{n \in \Naiset} \InfEU_{\n, \k}~\i = \{ 1 , 2\}.
%%\sum_{n=1}^{\frac{ \N }{\K}  \cdot \Prob_{\i}} \InfEU_{n},~\i = \{ 1 , 2\}.
%\end{aligned}
%\end{equation}
%The interference level not known by the \db~$\i$ is
%\begin{equation}\label{eq:unknown_inf}
%\begin{aligned}
%\textstyle
%\InfUnknown^{\i}_{\k} \triangleq \InfOut^{\i}_{\k} + \sum_{n \in \Noset} \InfEU_{n, \k} + \sum_{n \in \Najset} \InfEU_{n, \k}~\j \neq \i.
%%\InfUnknown^{\i}_{\k} \triangleq \InfOut^{\i}_{\k} + \sum_{n=1}^{\frac{ \N  }{\K}\cdot (1 - \Prob_{\i} - \Prob_{\j})} \InfEU_{n} + \sum_{n=1}^{\frac{ \N  }{\K}\cdot \Prob_{\j}} \InfEU_{n}~\j \neq \i.
%\end{aligned}
%\end{equation}
%The total interference level  on  \ch~$\k$ is
%\begin{equation}\label{eq:total_inf_new}
%\begin{aligned}
%\textstyle
%\InfTot_{\k} = \InfKnown_{\k} + \InfUnknown_{\k} = \InfTV_{\k} +\InfOut_{\k}+ \sum_{n \in \Nkset} \InfEU_{\n,\k}
%\end{aligned}
%\end{equation}
%where $\Naiset$ denotes the set of {\eus} operating on the channel $k$ and subscribing to the advance service of database $\i$; $\Najset$ denotes the set of {\eus} operating on the channel $k$ and subscribing to the advance service of database $\j \neq \i$; $\Noset$ denotes the set of {\eus} operating on the same channel $k$ and not subscribing to the advance service of both database, and $\Nkset$ denotes the set of {\eus} operating on the same channel $k$. Besides, we have $|\Naiset| = \frac{N}{K}\cdot{\eta_i}$, $|\Najset| = \frac{N}{K}\cdot{\eta_j}$, and $|\Noset| = \frac{N}{K}\cdot( 1 - \eta_1 - \eta_2)$. Moreover, we have $\i, \j \in \{1 ,2 \}$, $\i \neq \j$, $\Nkset = \Naiset \bigcup \Najset \bigcup \Noset$, and $\Naiset \bigcap \Najset \bigcap \Noset = \emptyset$.
%The database knows the precise value of $\InfKnown_{\k}$ on every channel $k$, which will be provided for {\eus} who subscribing to the advanced service.
%It is easy to see that the more {\eus} subscribing to this advanced service, the more accurate the advanced information will be.
%%It is assumed that the \db~knows the realized value of $\InfKnown_{\k}$.
%{
%By the iid assumption on $\InfTV_{\k}$, $\InfEU_{\n,\k}$, and $\InfOut_{\k}$, we can easily find that (i) $\{ \InfKnown_{\k} \}_{ \k\in\Kset }$, are i.i.d., (ii) $\{ \InfUnknown_{\k}\}_{\k\in\Kset}$, are i.i.d., and (iii) $\{ \InfTot_{\k} \}_{ \k\in\Kset }$, are i.i.d..
%Finally, we assume that both the \db~and \eus~knows \emph{a priori} the distributions of $\InfTV_{\k}$, $\InfEU_{\n,\k}$, and $\InfOut_{\k}$, and therefore the distributions of $\InfKnown_{\k}$, $\InfUnknown_{\k}$, and $\InfTot_{\k}$ given the market share $\Prob$.
%}

\textbf{Information Value.}
Now we evaluate the value of database $\dbb_l$'s information to {\eus}, which is
reflected by the {\eu}'s benefit (utility) that can be achieved from this information.

We first consider the expected  utility of a {\eu} when not subscribing to any advanced service (i.e., $\l=0$).
In this case, the {\eu} will randomly select a channel from the available channel list, and its expected utility is
\begin{equation}\label{eq:rate-random-fixed}
\begin{aligned}
\textstyle
\RB   \textstyle \triangleq \ut(\R_0) = \ut\left(\int_{z} \rt(z) \mathrm{d} F_{\InfTot}(z)\right),
%& \textstyle = \ut\left( \Ex_{\InfTot} \big[ \rt \left( \InfTot_{\k} \right) \big] \right)
%\\
%& \textstyle = \ut\left( \int_{z} \rt(z) \cdot f_{\InfTot}(z) \cdot \mathrm{d}z \right).
%\vspace{8mm}
\end{aligned}
\end{equation}
where $\R_0$ is the expected data rate given in (\ref{eq:rkgs}).
%By (\ref{eq:total_inf_new}), the distribution of $\InfTot$ is independent of the percentage of advanced {\eus} $\Prob$. Therefore, the value of $\RB$ is also independent of $\Prob$.
%and for an {\eu} with $\l = \S$, its expected utility is
%\begin{equation}\label{eq:rate-sense-fixed}
%\begin{aligned}
%\RS  & \textstyle  \triangleq \ut\left(\Rks\right) ,
%%=  \ut\left( \Ex_{\InfTotMin} \big[ \rt \left(\InfTotMin \right) \big] \right)
%%\\
%%&\textstyle= \ut\big( \K  \int_z \rt(z) \cdot [ 1 - F_{\InfTot}(z)]^{\K - 1} \cdot f_{\InfTot}(z) \cdot \mathrm{d}z \big),
%%\vspace{8mm}
%\end{aligned}
%\end{equation}
%where $\R^{(\G_i)} $ is the expected data rates defined in (\ref{eq:rkgs}).
Obviously, $\RB$ depends only on the distribution of the total interference $\InfTot_k$, while not on the specific distributions of $\InfKnown_k^{[l]}$ and $\InfUnknown_k^{[l]}$. This implies that the accuracy of the database $\dbb_l$'s information does not affect the utilities of those {\eus} not subscribing to its advanced service.


Then we consider the expected utility of a {\eu} when subscribing to the database $\dbb_l$'s advance service (i.e., $\l\in\{1,2\}$).
In this case, the {\db} $\dbb_l$ returns the interference $\{\InfKnown_{k}^{[l]}\}_{k\in\Kset}$ to the {\eu}, together with the basic information such as the available channel list.
%Notice that the total interference also includes the interference $\{\InfUnknown_{k}\}_{k\in\Kset} $ not provided by the database.
%\db~ranks the  {\chs} in ascending order given {\ch} interference level it known (i.e., $\InfKnown_{1}, \InfKnown_{2}, \ldots, \InfKnown_{\K} $). The ranked interference level are denoted by $\InfKnown_{(1)}, \InfKnown_{(2)}, \ldots, \InfKnown_{(\K)}$ and satisfy $\InfKnown_{(1)} < \ldots< \InfKnown_{(\K)}$.
For a rational {\eu}, it will always choose the channel with the minimum $\InfKnown_{k}^{[l]}$ (since $\{\InfUnknown_{k}^{[l]}\}_{k\in\Kset}$ are iid).
%\footnote{This is because the uncertain interference $\{\InfUnknown_{k}\}_{k\in\Kset} $ are i.i.d.}
Let $\InfKnownMin^{[l]} =  \min\{ \InfKnown_{1}^{[l]},  \ldots, \InfKnown_{K}^{[l]}  \} $ denote the minimum interference indicated by the database $\dbb_l$'s information.
Then, the actual interference experienced by a {\eu} (subscribing to the database $\dbb_l$'s advanced service) can be formulated as the sum of two random variables, denoted by $\InfTot^{[l]} = \InfKnownMin^{[l]} + \InfUnknown$. Accordingly, the {\eu}'s expected data rate and expected utility under the strategy $l\in\{1,2\}$ can be computed by
%Hence, the advanced {\eus} transmit at the {\ch} with lowest $\InfKnown$ and with total interference level $\InfTotA = \InfKnownMin + \InfUnknown$. Therefore, the advanced \eu's expect data rate is
\begin{equation}\label{eq:rate-pay-fixed}
\begin{aligned}
\Rl & \textstyle = \Ex_{\InfTot^{[l]}} \big[ \rt \left(\InfTot^{[l]} \right) \big] = \int_z \rt(z)  \mathrm{d} F_{\InfTot ^{[l]}}(z),
\\
\RA_l & \textstyle  \triangleq \ut\left(\Rl\right) = \ut\left(\int_z \rt(z)  \mathrm{d} F_{\InfTot ^{[l]}}(z)	\right) ,
% \textstyle =  \ut\left(\Ex_{\InfTotA} \big[ \rt \left(\InfTotA \right) \big] \right),
%\\
%&= \Ex_{\InfTotA} \big[ \rt \big( \InfKnownMin + \InfUnknown \big) \big] \\
%&= \K \cdot \int_{\InfTotA} \rt(z) \cdot \big[ \int_{\infty}^{\infty} f_{\InfKnown}(z -y) \cdot [ 1 - F_{\InfKnown}(y)]^{K-1} \cdot f_{\InfUnknown}(y) \mathrm{d}y  \big] \mathrm{d}z
%& \textstyle  = \ut \big( \int_z \rt(z) \cdot f_{\InfTotA}(z) \cdot \mathrm{d}z \big),
%\vspace{8mm}
\end{aligned}
\end{equation}
where
 $F_{\InfTot^{[l]}}(z)$ is the CDF of $\InfTot^{[l]}$.
% , and defined by
%\begin{equation*}\label{eq:min-known-pdf}
%%\begin{aligned}
%\textstyle
%f_{\InfTotA}(z) = \K   \int_y \big[ 1 - F_{\InfKnown}(z - y) \big]^{K-1} \cdot f_{\InfKnown}(z -y) \cdot f_{\InfUnknown}(y) \cdot \mathrm{d}y.
%%\vspace{8mm}
%%\end{aligned}
%\end{equation*}
It is easy to see that both $\Rl$ and $\RA_l$ depend on the distributions of $\InfKnown_k^{[l]}$ and $\InfUnknown_k^{[l]}$, and thus depend on the market share $\Prob_l$.
Thus, we will write $\RA_l$ as $\RA_l(\Prob_l)$.
We can further check that $\RA_l(\Prob_l)$ increases with $\Prob_l$.~~~~
%, because the more {\eus} subscribing to the database $\dbb_i$'s advanced service, the more accurate the database $\dbb_i$'s information, and further the more benefit for the {\eus} subscribing to the database $\dbb_i$'s advanced service.
%For convenience, we assume that $\RA_l(\Prob_l)$ is concave in $\Prob_l$ \rev{\footnote{This is validated by the simulation}}.~~~~~~~~~~~


%By (\ref{eq:rate-random-fixed})--(\ref{eq:rate-pay-fixed}), we can find the following useful properties.
%%, which are very important for the later analysis.
%
%\begin{proposition}
%%[Properties of $\RA, \RB, \RS$]
%\label{prop:ABS}
%~
%\begin{itemize}
%\item
% $\RB$ in (\ref{eq:rate-random-fixed})  does not depend on $\Prob_i$, $i\in\{1,2\}$;
% \item
% $\RA_i(\Prob_i)$ in (\ref{eq:rate-pay-fixed}) monotonously increases with $\Prob_i$;
% \item
% $\RA_i(\Prob_i) \geq \RB $, $\forall \Prob_i \in [0, 1]$;
% \item
%$\RA_i(\Prob_i)  = \RB$, only when $\Prob_i=0$ and meanwhile there is no licensee interference $\{ \InfTV_{\k} \}_{k\in\Kset}$.
%\end{itemize}
%\end{proposition}
%
%
%
%Then we consider the expected data rate of the \eus~who subscribe to the advance service (i.e., $\l=\A_{\i}, \i \in \{ 1, 2 \}$).
%With this advanced service, the \db~$\i$ returns the interference $\{ \InfKnown^{\i}_{k}\}_{k\in\Kset}$ to {\eus}, together with the basic information such as the available channel list.
%Notice that the actual interference also includes the interference part $\{\InfUnknown^{\i}_{k}\}_{k\in\Kset} $ not known by the database $\i$.
%%\db~ranks the \chs~in ascending order given \ch~interference level it known (i.e., $\InfKnown_{1}, \InfKnown_{2}, \ldots, \InfKnown_{\K} $). The ranked interference level are denoted by $\InfKnown_{(1)}, \InfKnown_{(2)}, \ldots, \InfKnown_{(\K)}$ and satisfy $\InfKnown_{(1)} < \ldots< \InfKnown_{(\K)}$.
%For a rational {\eu}, he will always choose the channel with the lowest $\InfKnown^{\i}_{k}$ provided~by~the~database.\footnotesc{This is because the uncertain interference $\{\InfUnknown^{\i}_{k}\}_{k\in\Kset} $ are i.i.d.}
%Let $\InfKnownMin^{\i} =  \min\{ \InfKnown^{\i}_{1},  \ldots, \InfKnown^{\i}_{\k}  \} $ denote the lowest interference provided by the database.
%Then, the actual interference experienced by the {\eu} is $\InfTotA^{\i} = \InfKnownMin^{\i} + \InfUnknown$, and accordingly the expected data rate is
%%Hence, the advanced \eus~transmit at the \ch~with lowest $\InfKnown$ and with total interference level $\InfTotA = \InfKnownMin + \InfUnknown$. Therefore, the advanced \eu's expect data rate is
%\begin{equation}\label{eq:rate-pay-fixed}
%\begin{aligned}
%\ut(\R^{\A_{\i}})  = \RA^{\i} & \textstyle \triangleq \ut( \Ex_{\InfTotA^{\i}} \big[ \rt \big(\InfKnownMin^{\i} + \InfUnknown^{\i} \big) \big] ) \\
%%&= \Ex_{\InfTotA} \big[ \rt \big( \InfKnownMin + \InfUnknown \big) \big] \\
%%&= \K \cdot \int_{\InfTotA} \rt(z) \cdot \big[ \int_{\infty}^{\infty} f_{\InfKnown}(z -y) \cdot [ 1 - F_{\InfKnown}(y)]^{K-1} \cdot f_{\InfUnknown}(y) \mathrm{d}y  \big] \mathrm{d}z
%& \textstyle  = \ut( \int_{\InfTotA^{\i}} \rt(z) \cdot h(z) \cdot \mathrm{d}z ),
%%\vspace{8mm}
%\end{aligned}
%\end{equation}
%where
% $h(\cdot)$ is the pdf of $\InfTotA^{\i}$, defined by
%\begin{equation*}\label{eq:min-known-pdf}
%%\begin{aligned}
%\textstyle
%h(z) = \K \cdot \int f_{\InfKnown^{\i}}(z -y) \cdot \big[ 1 - F_{\InfKnown^{\i}}(z - y) \big]^{K-1} \cdot f_{\InfUnknown^{\i}}(y) \cdot \mathrm{d}y.
%%\vspace{8mm}
%%\end{aligned}
%\end{equation*}
%By (\ref{eq:rate-pay-fixed}), we can see that $\RA^{\i}$ depends on the distributions of $\InfKnown^{\i}_k$ and $\InfUnknown^{\i}_k$, and accordingly depends on the market share $\Prob_{\i}$ (and thus, we will also write $\RA^{\i}$ as $\RA(\Prob_{\i})$).
%We can further check that $\RA(\Prob_{\i})$ increases with $\Prob_{\i}$. This is because the more {\eus} subscribing to the advanced service,  the more accurate the database's information is, and further the more benefit for the {\eus} subscribing to the advanced service. We can also note that if two database $\dbb_1$ and $\dbb_2$ share their market shared information, both of them can obtain more accurate information. However, they compete for the same pool of {\eus}. Sharing the information may lead to the decreasing of their own profit.

%Based on the above, we can find the following useful properties, which are very important for the later analysis.
%\begin{proposition}\label{prop:ABS}
%~
%\begin{itemize}
%\item
% $\RB$ in (\ref{eq:rate-random-fixed}) and $\RS$ in (\ref{eq:rate-sense-fixed}) do not depend on $\Prob$;
% \item
% $\RA(\Prob)$ in (\ref{eq:rate-pay-fixed}) monotonously increases with $\Prob$;
% \item
% $\RB\leq \RA(\Prob) \leq \RS $, $\forall \Prob \in [0, 1]$;
% \item
%$\RA(1)  = \RS$, if no outside interference $\{ \InfOut_{\k} \}_{k\in\Kset}$;
% \item
%$\RA(0)  = \RB$, if no licensee interference $\{ \InfTV_{\k} \}_{k\in\Kset}$.
%\end{itemize}
%\end{proposition}




\textbf{Problem Formulation.}
Suppose that each {\eu} is rational, and will always choose the strategy that maximizes its payoff.
We are interested in the following problems: given the information prices $\{\p_1, \p_2\}$ and initial market shares $\{\Prob^0_1, \Prob^0_2 \}$ of databases, how these market shares dynamically evolve and what is the market equilibrium?

%We will study the oligopoly price competition game between databases $\dbb_1$ and $\dbb_2$.
%In the proposed oligopoly price competition game, each database $\dbb_i$ chooses the price $\p_i$ for its information, aiming at maximizing its revenue
%$$
%\Udb_i = \p_i\cdot \Prob_i \cdot N.
%$$
%%given the distributions of licensee interference $\InfTV_{\k}$, outside interference $\InfOut_{\k}$, and single {\eu} interference $\InfEU_{\n,\k}$.
%Note that the market share $\Prob_i $ of the database $\dbb_i$ depends not only on its own price $\p_i$, but also on the other database $\dbb_j$'s price $\p_j$, and thus can be written as $\Prob_i(\p_1, \p_2)$.
%Moreover, the change of $\Prob_i$ will affect the distributions of $\InfKnown_k^i$ (known by the database $\dbb_i$) and $\InfUnknown_k^i$ (not known by the database $\dbb_i$), which in turn will affect the {\eu}'s utility $\RA_i(\Prob_i)$ achieved from the database $\dbb_i$'s advanced service.

%
%revenue maximization where two database compete by choosing prices, given the distributions of licensee interference $\InfTV_{\k}$, outside interference $\InfOut_{\k}$, and single {\eu} interference $\InfEU_{\n}$.
%For database $\i$, its {revenue} is $\p_{\i} \cdot \Prob_{\i}(\bp) \cdot N$.
%%optimal information pricing plan (i.e., $\p_1$ and $\p_2$) that maximizes the database's
%Notice that the database $\dbb_{\i}$'s market share $\Prob_{\i}(\bp)$ is a function of $\bp = (\p_1, \p_2)$.
%Moreover, the change of $\BProb$ will affect the interference levels $\InfKnown^{\i}_k$ (known by the database) and $\InfUnknown^{\i}_k$ (not known by the database), which in turn will affect the {\eu}'s expected data rate $\RA^{\i}(\BProb)$ achieved from the advanced service, and the {\eu}'s decision.

% (ii)
%By comparing (\ref{eq:rate-random-fixed}), (\ref{eq:rate-sense-fixed}), and (\ref{eq:rate-pay-fixed}), we have $\RB \leq \RA \leq \RS$
%When the random variable $\InfKnown$ is zero, we have $\RA = \RB$. Otherwise, $\RA > \RB$, $\forall \Prob \in [0,1]$. If the value of $\InfUnknown$ is zero, we have $\RA = \RS$. Otherwise, $\RA < \RS$, $\forall \Prob \in [0,1]$.

%We associate interference caused by TV station denoted by $\InfTV$, which is a random variable follows from a continuous distribution with cdf $F_{\InfTV}(\cdot) $ and pdf $f_{\InfTV}(\cdot)$. $\InfOut$ represents the interference cause by other database's {\eus} and is a random variable follows from a continuous distribution with cdf $F_{\InfOut}(\cdot) $ and pdf $f_{\InfOut}(\cdot)$ and represents the interference cause by other database's {\eus}. For particular {\eu}, we assume its receiving interference from each {\eu} in the same network \footnotesc{We assume {\eus} who connect to the same database acting in the same network.} $Y$ is a random variable with cdf $F_{Y}(\cdot) $ and pdf $f_{Y}(\cdot)$.


